On regularity of maximal distance minimizers in Euclidean Space

We study the properties of sets $\Sigma$ which are the solutions of the maximal distance minimizer problem, i.e. of sets having the minimal length (one-dimensional Hausdorff measure) over the class of closed connected sets $\Sigma \subset \mathbb{R}^n$ satisfying the inequality \[ max_{y \in M} dist(y,\Sigma) \leq r \] for a given compact set $M \subset \mathbb{R}^n$ and some given $r > 0$. Such sets can be considered as the shortest networks of radiating Wi-Fi cables arriving to each customer (for the set $M$ of customers) at a distance at most $r$. In this paper we prove that any maximal distance minimizer $\Sigma \subset \mathbb{R}^n$ has at most $3$ tangent rays at each point and the angle between any two tangent rays at the same point is at least $2\pi/3$. Moreover, in the plane (for $n=2$) we show that the number of points with three tangent rays is finite and every maximal distance minimizer is a finite union of simple curves with one-sided tangents continuous from the corresponding side. All the results are proved for the more general class of local minimizers, i.e. sets which are optimal under a perturbation of a neighbourhood of their arbitrary point.

==> parts/lemma_tree.tex <==
\begin{lemma}
Let $x \in E_\Sigma$ be a non-isolated energetic point. Let $\Sigma_0$ be a closed connected component of $\Sigma \setminus \{x\}$. Let $\varepsilon>0$ with $\sharp ( \Sigma \cap \partial B_\varepsilon(x) ) = \oord_x\Sigma$ and $\sharp ( \Sigma_0 \cap \partial B_\varepsilon(x) ) = 1$ be sufficiently small. Let $F\in \Sigma_0\cap B_{\varepsilon}(x)$ be a branching point and let $\Sigma_1\ni F$ be such a connected component of $\Sigma \setminus F$ that $\eta \defeq \dist (\Sigma_1, \partial B_{\varepsilon}(x) \cup \{x\})>0$.

Then there exists such $\gamma=o_\varepsilon(1)$ and such finite graph $G$ that
\begin{enumerate}
    \item all vertices $V(G)$ belong to $\Sigma_1$;
    \item for every edge and both vertices the angle between edge and one-sided tangent at the vertex is not greater than $30\gamma$;\label{second}
    \item for every two vertices path between them in $\Sigma$ and in $T$ contains the same set of vertices; 
    \item for every vertex its degree as a vertex of the graph is equal to its order as a point of the minimizer: $deg_v T=\oord_{v}\Sigma$.  
%$T$ doesn't contain loops; ОТСУТСТВИЕ ЦИКЛОВ ИЛИ ЧТО-ТО ДРУГОЕ
%    \item all leaves of $T$ are terminal points of of $\Sigma_0$ and all branching points of $T$ are the branching points of $\Sigma_0$.          МОЖНО ПРО ЛЮБЫЕ СТЕПЕНИ
\end{enumerate}
\label{tree}
\end{lemma}
\begin{remark}
$G$ is a finite tree. Moreover, if $A,B,C,D$ are such vertices of $T$ that $D$ belongs to every path from $i$ to $j\neq i$ where $i,j \in \{A,B,C\}$ then $D\in V(T)$. 
\end{remark}
\begin{proof}
Fix $\gamma,c=o_\varepsilon(1)$. 
For $\bar x$ define \textit{comfort zone} as such $\delta(\bar x)>0$ that there exists such $\bar \delta \in [8\delta(\bar x),9\delta(\bar x)]$ that \begin{enumerate}
    \item $\oord_{\bar x}\Sigma_1=\sharp(B_{\delta}(\bar x)\cap \Sigma_1)=\sharp(B_{\bar \delta(\bar x)}(\bar x)\cap \Sigma_1)$;
    \item for every positive $\delta'\leq \bar \delta$ there exists such connected $S=S(\bar x, \delta')\ni \bar{x}$ that $F_M(\Sigma \setminus B_{\delta'}(\bar x)\cup S) \leq F_M(\Sigma)$ and $\H(S)\leq c\delta'$;МОЖНО СИЛЬНЕЕ AS $F_M(\Sigma \setminus B_{\delta'}(\bar x)\cup S) =o(\delta')$\label{ququ}
    \item for every positive $\delta'\leq \bar \delta$ there exists $\oord_{\bar x}(\Sigma_1)$ tangent rays $[\bar x, a_i)_{i=1}^{\oord_{\bar x}\Sigma_1}$ that for every $t\in \Sigma_1\cap B_{\delta'}(\bar x)\setminus \{ \bar x\}$ the inequality $\angle t\bar x a_i\leq \gamma$ holds for some $i\in \{1,\ldots,\oord_x\Sigma_1\}$.
\end{enumerate}
As $\Sigma_1$ is a compact set, there exists a minimal by inclusion finite collection $\{x_i\}_{i\in I}\subset \Sigma_1$ such that $\Sigma_1 \subset \bigcup_{i \in I} B_{\delta(x_i)}(x_i)$.
Define a graph $T$ on the set of vertices $V(T) \defeq \{x_i\}_{i \in I}$ as follows: let $(x_a, x_b) \in E(T)$, i.e. let $x_a$ and $x_b$ be adjacent, if and only if there is no other $x_i$ on the path $\Sigma_1(x_a, x_b)$.
Note that if $x_a$,$x_b$ and $x_c$ are such points of $\Sigma_1$ that each path in $\Sigma_1$ from $x_i$ to $x_j$ (where different indices $i,j$ belong to $\{a,b,c\}$) contains the same branching point $F\notin \{x_a,x_b,x_c\}$, then there is such an index $l\in I$ that $F=x_l$. Note that $T$ is tree and all leaves of $T$ has an order $1$ in the set $\Sigma_1$.
\textbf{Note that all conditions on $G$ except~\ref{second} holds for $T$ by the construction}.

Let $U\in V(T)$ be ``bad'' i.e. such that the second condition doesn't hold i.e. $\angle (t_u,[uv])>10 \gamma$ where $t_U$ is the nearest tangent ray of $\Sigma$ at $U$, and $[UV]\in E(T)$. Thus %$\delta(V)=o(\delta(U))$ (depends on ...), particularly,
$\delta(U)<\frac{\delta(V)}{8}$. 
Let $U$ be an arbitrary first bad vertex at the path in $T$ from $F$.
We will consider $B_{2\delta(V)}(V)$ and remove some vertices and incident them edges such a way that the first ``bad'' vertex become farer on the path from $F$ through $U$ in $\Sigma$.

When the algorithm stops two conditions hold for each edge $UV$:
\begin{enumerate}
    \item $|UV|\leq 2(\delta(U)+\delta(V))$
    \item $\angle(t_U),(UV).\angle(t_V,(UV))\leq 10\gamma$ for some tangent rays $t_U$, $t_V$ of $\Sigma$ at points $U$ and $V$ accordingly.
\end{enumerate}

Let us denote by \textit{case A} situation when vertex  $U$ belongs to the path from $F$ to $V$ and by \textit{case B} the opposite case. 
Thus the following cases are possible:
\begin{enumerate}
   
    
    %There are two cases: \begin{enumerate}
        %\item 
%\textbf{        $U$ (and hence $Y$) belongs to the path from $F$ to $V$ in $\Sigma$.}

%Point $Y$ can not be ``bad'' vertex as $V$ was the first.
%радиус удвоился
        %\item \textbf{$V$ belongs to the path from $F$ to $U$ in $\Sigma$ (hence $V$ belongs to the path from $F$ to $Y$ in $\Sigma$).}
%Vertex $Y$ can be a ``bad'' vertex.
%радиус удвоился      
 %   \end{enumerate}
    \item \textbf{There exists $k>1$ and a set of consecutive adjacent vertices $\{A_i\}_{i=1}^{i=k} \subset V(T)\cap B_{2\delta(A_0)}(A_0)$ with $A_0\defeq V$, $A_1 \defeq U$ such that 
    \[
    (\Sigma_{VU}\cap B_{\frac{3}{2}\delta(V)}(V)) \subset \bigcup_{i=0}^k B_{2\delta(A_i)}(A_i),
    \]
    where $\Sigma_{UV}$ is a connected component of $\Sigma \setminus V$ containing $U$.}
    Clearly for every $i$ the inequality $\delta(A_i)\leq 3\delta(A_0)$ holds.
    %Then in \textit{case B} we can just 
    %delete from $V(T)$ all inner vertices and edges of path from $A_0$ to $A_k$ and all edges and vertices belonging to resulting connected components, which doesn't content $A_k$ or $A_0$ and add to $E(T)$ the edge $[A_0A_k]$. %любой другой i тоже ок, может надо другой
    There are two possible situation %in \textit{Case A}:
    \begin{enumerate}
        \item \textbf{for every $j\leq k$ the inequality $\angle ( t_{A_j},t_{A_0})\geq 9\gamma$ for every tangent rays of $\Sigma$ at $A_j$.}
        
        Due to construction conditions there are  $\angle (t_{A_0},[A_0A_{j}])\leq \gamma$.
        
        Note that in every ball $B_{\delta(A_j)}(A_j)$ with $j\geq 1$ the difference
        \[
        \H(\Sigma \cap B_{\delta(A_j)}(A_j))-\H(Pr_{t_{A_0}}\Sigma \cap B_{\delta(A_j)}(A_j)) \geq 2\delta(A_j)(1-\cos (8\gamma))=4\delta(A_j)\sin^2(4\gamma)\]
         where $Pr_{t_{A_j}}()$ means the projection to the tangent line $t_{A_j}$.
        Note also that
        \[
        \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))\geq \sum_{j=1}^k\frac{\H(\Sigma \cap B_{\delta(A_j)}(A_j))}{4}
        \]
        where
        $\Sigma_{UV}$ is a connected component of $\Sigma \setminus V$  containing $U$ and \[
        B_{2\delta(A_0),\delta(A_0)}(A_0):=B_{2\delta(A_0)}(A_0)\setminus B_{\delta(A_0)}(A_0).
        \]
        Hence
           \[ \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))-\H(Pr_{t_{A_0}}\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0) \geq \sin^24\gamma \sum_{j=1}^k\delta(A_j)\geq \frac{\delta(A_0)\sin^24\gamma}{4}.\]
        %\[
        %\H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))\geq
        %\]
        By the other hand 
        \[
        \H(\Sigma_{UV}\cap B_{2\delta(A_0)}(A_0)\setminus B_{\delta(A_0)}(A_0))=\delta(A_0)+o(\delta(A_0))
        \]and
        \[ \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))-\H(Pr_{t_{A_0}}\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0) \leq \delta(A_0)(1-\cos \gamma)=2\delta(A_0)\sin^2\frac{\gamma}{2}.\]
        So we got a contradiction for $\gamma<0,2$.
        
        
        
        %thus $\angle (t_{A_0},t_{A_{j}})\geq 2\gamma$ for every $j\leq k$ and hence $\angle (t_{A_0},[A_{j-1}A_{j}])\geq \gamma$
      %  for every $j$. % On the other hand in \textit{case A} the inequality \[\angle (t_{A_j}[A_j,A_{j-1}]), \angle (t_{A_j}[A_j,A_{j-1}])\leq \gamma\] holds for $j>1$.
     %But this is impossible, otherwise we can pick $\bar A$ such that $|3/2\delta(A_0)-|A_0\bar A||=o(\delta(A_0))$ and delete in $\Sigma$ path between $A_0$ and $\bar A$ (we also delete all connected components doesn't contain $A_0$ or $\bar{A}$) and add the segment $[A_0\bar A]$ and a connected set $S\ni A_0$ from Lemma... instead of it. The resulting set is better than $\Sigma$ as the length of the deleted set was at least $\frac{3|\delta(A_0)|}{2\sin \gamma}+o(\delta(A_0))$ and the length of the added set is $\frac{3|\delta(A_0)|}{2}+o(\delta(A_0))$. 
       % So we get a contradiction.
%                \[
 %       \sharp (\Sigma \cap B_{|A_0A|(A_0)})=\oord_{A_0}(\Sigma).
  %      \]
   %     Thus
        
        \item \textbf{ there exists such $1<j\leq k$ that $\angle (t_{A_j},t_{A_0})<9\gamma$ where $t_{A_j}$ is a tangent ray of $\Sigma$ at $A_j$.}     
        Due to construction 
        \[
        \angle (t_{A_j},(A_0A_j))<10\gamma. 
        \]
        We delete from $V(T)$ all inner vertices of the path between $A_0$ and $A_j$ (and all edges and vertices belonging to resulting connected components, which don't content $A_0$ or $A_j$) and add to $E(T)$ the edge $[A_0A_j]$.
        
        Note that $|A_jA_0| \leq 2\delta(A_0)$. 
        %(the vertex $A_j$ was not ``bad'' as $U$ was the first bad one). %тут утроился угол 
    \end{enumerate}
     \item \textbf{There exists such a point $Y \in V(T)$ that $U$ belongs to the path in $T$ from $V$ to $Y$, and $\delta(Y)+\frac{3}{2}\delta(V)>\dist(V,Y)\geq 2\delta(V) $.}
    
    Thus $2\delta(Y)\geq \delta(V)$ and thus $\angle(t_Y,(YV))<\gamma<10\gamma$
    
    If $\angle(t_V,(YV))<10\gamma$
    (particularly in case $\delta(Y)\leq 8\delta(V)$) we delete from $V(T)$ all inner vertices of the path between $Y$ and $V$ (and all edges and vertices belonging to resulting connected components, which doesn't content $Y$ or $V$) and add to $E(T)$ the edge $[YV]$. 
    
    Otherwise we also delete from $T$ the same vertices and edges, also add to $E(T)$ the edge $[YV]$ and repeat the algorithm for $V$ as $U$ and $Y$ as $V$ ($V:=Y$ and $U:=V$). When this process stops we will have vertices that corresponds to both conditions.
    
    
    %Note that in \textit{case A} point $Y$ can not be ``bad'' vertex as $U$ was the first, and in \textit{case B} it can but the first ``bad'' vertex is later than before the reconstruction of the tree.
\end{enumerate}
\end{proof}

==> parts/per.tex <==
\section{Остальные локальные свойства минимайзеров}
\label{per}


Использованные в статье методы позволяют получить большое количество утверждений относительно гладкости и локальной структуры $\Sigma$. %В частности,

%\subsection{Еще несколько результатов}

%\begin{remark}
%А обозначениях теоремы~\ref{mainT1} можно считать, что каждая инъективная кривая имеет на конце непрерывную касательную. Иными словами, односторонние касательные ко внутренним точкам кривой сходятся к касательной в концевой точке.
%\end{remark}

\begin{theorem2}
Пусть $\Sigma$ --- минимайзер максимального расстояния для плоского компактного множества $M$.  Тогда
\begin{enumerate}
\item в окрестности произвольной точки $x\in \Sigma$ множество $\Sigma$ совпадает с одной, двумя или тремя дугами с концами в $x$, имеющими в $x$ непрерывную касательную %(соответствующие им функции имеют в $x$ непрерывную первую производную).   
Также в каждой из точек каждой из дуг есть односторонняя касательная, односторонние касательные непрерывно сходятся к касательной к дуге в точке $x$.
Каждая из дуг является графиком функции, имеющей в точке $x$ непрерывную производную (за абсциссу считаем касательную). 
%Для краткости будем называть такие функ
\label{f}
\item в достаточно малой окрестности $B_{\varepsilon}(x)$ произвольной точки $x\in \Sigma$ выполняется
 \[
  \oord_x\Sigma \cdot \varepsilon \leq \H(\Sigma \cap B_\varepsilon(x)) = \oord_x \Sigma \cdot \varepsilon +o(\varepsilon).
 \]
 Заметим, что это уточняет константы регулярности по Альфорсу (см. свойства минимайзеров п.~\ref{j});
 \label{len1}
\item для произвольной точки $x\in \Sigma$ выполняется $\oord_x\Sigma=\oordball_x\Sigma$; 
\label{oo}
\item множество $\Sigma$ в окрестности произвольной $x \in G_\Sigma$ является графиком некоторой функции %(для краткости будем называть такую функцию "соответствующей"). 
Если точка $x \in G_\Sigma$ имеет два различных касательных луча, угол между которыми меньше $\pi$, то $\Sigma$
%(как функция) 
локально нестрого выпукла в окрестности точки $x$ (выпукла внутрь меньшего угла). В таком случае соответствующая функция нестрого выпукла, то есть, в частности,
%$\Sigma$ в окрестности $x$ является графиком нестрого выпуклой функции, то есть, в частности, функции, которая 
%Это, в частности означает, что соответствующая ей функция 
почти всюду имеет вторую производную;
\label{conv_}
\item если (содержащаяся в $\Sigma$) инъективная кривая с концом в точке $x$ не является нестрого выпуклой в её окрестности, то 
\label{nevv}
\begin{enumerate}
\item если она имеет кривизну, то кривизна по модулю не превосходит $1/r$ (если соответствующая данной кривой функция имеет в точке $x$ вторую производную, то она по модулю не превосходит $1/r$);
\item её односторонние касательные сходятся к односторонней касательной в точке $x$ (соответствующая данной кривой функция имеет непрерывную первую производную в точке $x$);
\label{ggg}
\item если существует другая инъективная кривая с концом в $x$, то  ее кривизна, в случае наличия, по модулю не превосходит $1/r$, а её односторонние касательные сходятся к односторонней касательной в точке $x$. При этом односторонние касательные к обеим инъективным кривым образуют прямую (то есть, функция, соответствующая $\Sigma$, имеет непрерывную производную в $x$); 
\item в достаточно малой окрестности $B_{\varepsilon}(x)$  выполняется
 \[
\oord_x\Sigma \cdot \varepsilon  \leq \H(\Sigma \cap B_\varepsilon(x)) \leq \oord_x\Sigma \cdot \varepsilon +O(\varepsilon^2).
 \]
 \label{len2}
\end{enumerate}
\end{enumerate}
\label{persp}
\end{theorem2}
\begin{proof}

Докажем пункт~\ref{f}. Из доказательства Теоремы~\ref{mainT1}  следует, что
каждая такая дуга либо является отрезком, либо содержится в псевдоконусе с вершиной в $x$ и энергетическим ребром в качестве оси. В первом случае утверждение пункта очевидно, а во втором следует из леммы~\ref{zapred}.
%\end{proof}
%леммы~\ref{eva} ы~\ref{uggi}
Покажем верность пункта~\ref{len1}. Множество $\Sigma \setminus \{x\}$ имеет $\oord_x \Sigma \leq 3$ компонент связности. Каждая из компонент связности, ввиду Теоремы~\ref{mainT1} имеет в точке $x$ касательную, а значит ввиду замечания~\ref{len0}, в достаточно малом шаре $B_\varepsilon(x)$ имеет длину $\varepsilon+ o(\varepsilon)$. 

Таким образом
\[
\H(\Sigma \cap B_\varepsilon(x)) =\oord_x \Sigma \varepsilon +o(\varepsilon).
\]
 Неравенство $\H(\Sigma \cap B_\varepsilon(x)) $ напрямую следует из неравенства коплощади

Покажем верность пункта~\ref{oo}. Предположим противное, то есть, ввиду замечания~\ref{rem_ord}, что $\oordball_x\Sigma >\oord_x\Sigma $.
В таком случае для достаточно малого $\varepsilon$
\[
\H(\Sigma \cap B_\varepsilon(x)) \geq \oordball_x \Sigma \varepsilon \geq (\oord_x \Sigma +1) \varepsilon,
\]
что противоречит утверждению пункта~\ref{len1}.

Докажем пункт~\ref{conv_}. Утверждение интересно только для $x\in E_\Sigma$. В таком случае хотя бы одна из двух касательных является энергетическим ребром, при этом ребро направлено в одну сторону. Рассмотрим дугу $\breve{sx}$, являющуюся замыканием компоненты связности $\Sigma \cap B_\varepsilon(x) \setminus \{x\}$ для достаточно малого $\varepsilon$, для которой данное энергетическое ребро является касательной в точке $x$. Не умаляя общности, будем полагать это ребро совпадающим с отрицательной частью оси абсцисс и будем полагать его направленным вверх. Будем также полагать, что для всех энергетических точек, принадлежащих $\breve{sx}$, соответствующие им точки находятся в верхней полуплоскости (это возможно ввиду показанного в лемме~\ref{Losiu}). В таком случае не существует двух точек $z_1, z_2 \in \breve{]sx[} $ таких, что поддуга $\breve{sx}$, их соединяющая, находится ниже соединяющего их отрезка: в противном случае замена дуги на отрезок уменьшило бы длину, без ущерба для связности и энергии. Несложно заметить, что данное свойство влечет нестрогую выпуклость вверх дуги $\breve{sx}$. Также мы показали, что $\breve{sx}$ можно рассматривать как график нестрого выпуклой функции.

Перейдем к пункту~\ref{nevv}: как было показано выше точка $x$ должна принадлежать множеству $E_\Sigma$, причем иметь энергетическое ребро, направленное в две стороны. В таком случае найдутся такие точки $y_1$, $y_2$, что прямая $(y_1y_2)$ перпендикулярна энергетическому ребру, \[|y_1x|=r=|xy_2|\] и \[B_r(y_1) \cap \Sigma =\emptyset = B_r(y_2)\cap \Sigma.\]
Отсюда тривиально следуют все утверждения пункта.
%\begin{remark}
%Доказательство  пунктов~\ref{len1} и~\ref{len2} можно было бы провести и аналитически, сопоставив кривой график функции $f$, точке $x$ начало координат, а касательной к кривой в точке $x$ --- ось абсцисс. Тогда $f(0)=0=f'(0)$. В случае~\ref{len2} кривую также пришлось бы сгладить, после чего заметить ограниченность модуля второй производной гладкой функции, приближающей $f$, числом $1/r$. 
%\end{remark}

\end{proof}
%Доказательства Теоремы~\ref{persp} 
%можно найти в разделе~\ref{prf}, 
%и объяснение, как методами данной статьи получать другие локальные утверждения можно найти в разделе~\ref{per}.
%Доказаны также некоторые еще утверждения про выпуклость %множества $\Sigma$ (см Леммой~\ref{main_ld}).


На самом деле, мы доказали даже более сильный результат, поскольку в доказательствах Теорем~\ref{mainT1} и~\ref{persp}  использовались только локальные аргументы, и поэтому его можно провести и для определенного ниже локального минимайзера.

\begin{definition}
Для заданного компактного множества $M \subset \R^2$ и числа $r>0$ локальным минимайзером функционала максимального расстояния будем называть такое связное замкнутое множество $\Sigma \subset \R^2$, что $F_M(\Sigma)\leq r$ и существует такое $\varepsilon>0$, что для произвольного замкнутого связного $\Sigma'$ такого, что $F_M(\Sigma')\leq r$ и $\diam \Sigma \triangle  \Sigma' < \varepsilon$ выполняется $\H(\Sigma)\leq \H(\Sigma')$.
\end{definition}

\begin{theorem2}
Пусть $\Sigma$ --- локальный минимайзер максимального расстояния.  Тогда выполняются все утверждения Теорем~\ref{mainT1} и~\ref{persp}.
%\begin{itemize}
%\item[(i)] множество $\Sigma$ является объединением конечного числа инъективных кривых;
%\item[(ii)] угол между любыми двумя касательными лучами в произвольной точке $x \in \Sigma$ не меньше $2 \pi/3$.
%\end{itemize}
%\label{mainT2}
\end{theorem2}

%\begin{corollary}
%Из Теоремы~\ref{mainT1} следует конечность числа точек порядка $3$ в (локальном) минимайзере максимального расстояния.
%\end{corollary}






%Покажем  верность Теоремы~\ref{persp}.


Поговорим о том, как получать иные утверждения о локальном поведении $\Sigma$. Оно интересует нас только в окрестностях точек из множества $E_\Sigma$. Ясно, что точки $E_\Sigma$ бывают следующих типов:
%\begin{enumerate}
%\item точки ветвления $x\in S_\Sigma$ степени $3$. Таких точек конечное число, поэтому при исследовании окрестностей точек $x\in %E_\Sigma$ можно считать, что их не существует.
%\item точки $x\in S_\Sigma$ степени $2$. Касательная в этих точках не меняется.
%\item точки $x\in X_\Sigma$ степени два такие, что существуют две окружности с центрами в $y_1,y_2$ такие, что $|y_1y_2|=2r$ и %$B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. В этом случае в точке $x$ касательная не меняется.
%\item Более интересные точки:
\begin{itemize}
%\item [(a)] точки $x\in X_\Sigma$ степени два такие, что в них $\Sigma$ имеет два разных отрезка с углом, не равным $\pi$; 
\item [(i)] точки $x\in E_\Sigma$ такие, что не существует двух окружностей с центрами в $y_1,y_2$ таких, что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ в окрестности точки $x$ (нестрого) выпукла. % (однако хотя бы одна окружность $B_r(y)$, такая что $B_r(y)\cap\Sigma=\emptyset$ существует и ее расположение задает направление выпуклости). 
А значит, имеет субградиент, а также почти всюду выпукла и являются графиком функции, которая почти всюду %(но не обязательно в $x$)
имеет производную, которая монотонна;
\item [(ii)] точки $x\in E_\Sigma$ такие, что существуют две окружности с центрами в $y_1,y_2$, такие что $|y_1y_2|=2r$ и $B_r(y_1)\cap \Sigma=\emptyset=B_r(y_2)\cap \Sigma$. Тогда $\Sigma$ является графиком функции, которая имеет непрерывную производную в точке $x$. А если она имеет вторую производную, то та ограничена по модулю величиной $1/r$. 
\end{itemize}
%\end{enumerate}
%При этом точки типа (ii) являются пределом либо точек степени (ii), либо точек типа (i) или (a), где пустые окружности расположены по разную сторону от кривой. При этом выпуклость может меняться только в точках типа (ii), либо (в некотором смысле) в таких точках типа (i), что одна из кривых --- прямолинейный отрезок.

Если какая-то дуга минимайзера (c концом в $x$) целиком состоит из точек типа (i), то она наследует свойства некоторого подмножества множества $M$: утверждается, что множество $M$ тогда должно иметь кривую (или счетный набор кривых), полученную из данной дуги отступлением по внешней (если считать дугу границей выпуклой фигуры) нормали на $r$ во всех точках, где нормаль единственна (то есть в почти всех точках дуги). В частности, если дуга была непрерывно дифференцируемой, то ей соответствует дуга множества $M$. Причем данная дуга $\Sigma$ тогда должна быть дважды дифференцируемой, соответствующая ей дуга множества $M$ также должна быть дважды дифференцируемой, причем её вторая производная должна не превосходить $1/r$. Если она строго меньше $1/r$, то есть минимальный радиус кривизны дуги $M$ больше $r$, то тогда минимальный радиус кривизны дуги $\Sigma$ в точности равен разности между минимальным радиусом кривизны дуги $M$ и числом $r$. Доказательство данного факта мы приводить не будем, оно является достаточно очевидным следствием основного свойства энергетических точек. 

Если какая-то дуга целиком состоит из точек типа (ii), то она является непрерывно дифференцируемой. Тогда множество $M$ содержит две дуги полученных из данной дуги $\Sigma$ отступами по обеим нормалям на $r$. Несложно заметить, что тогда исходная дуга является дважды дифференцируемой и значит её вторая производная по модулю ограничена величиной $1/r$. При этом радиусы кривизны кривых $M$ отличаются от её радиусов кривизны в каждой точке на $r$.

Таким образом, получается что точки всех видов обладают рядом полезных свойств, комбинируя которые можно получать новые свойства $\Sigma$ или отвечать на вопрос, может ли то или иное множество быть минимайзером (отвечать отрицательно или конструктивно строить множество $M$, для которого данное множество может быть минимайзером). В частности --- графики элементарных функций, поскольку они (кроме графиков константы) обязаны состоять только из точек типа (i) и (ii).

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2\sin(\frac{1}{x})$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Но производная функции $f$ не является непрерывной в нуле и значит график данной функции не может быть минимайзером. 
\end{proof}

\begin{example}
Может ли кривая, являющаяся графиком функции $f(x)= x^2 \sin \left (\frac{1}{\sqrt{x}} \right)$ в окрестности нуля быть минимайзером для некоторого множества $M$?
\end{example}
\begin{proof}
Заметим, что точка $0$ --- точка типа (ii). Теперь производная $f$ непрерывна в нуле. Поскольку для каждой точки $x\neq 0$ вторая производная существует, непрерывна и ее значение по модулю стремится к бесконечности при приближении к нулю и, значит, можно считать, что она больше, чем $1/r$. Тогда каждая точка, кроме $0$ может быть только типа (i). Но знак второй производной все время меняется и, значит, существует стремящаяся к нулю последовательность точек, в которых кривая меняет выпуклость. Ввиду отсутствия прямолинейных отрезков получили противоречие.
\end{proof}
%а выпуклость может меняться?



%Покажем верность правых частей в неравенствах пунктов~\ref{len1} и~\ref{len2}. Для этого достаточно показать, что %длина каждой из кривой


%Осталось доказать пункты~\ref{len1} и~\ref{len2}. Левые части следуют из неравенства ко-площади Предположим, это не так и длина какой-то из кривых
%ой еще про орд равно ордболл


%точки первого и второго типа
%пример: рассказ почему x^2\sin(\sqrt{x}) не подходит, хотя казалось бы а ой нет она же гладкая вне нуля и значит вт произв дб ограничены а они нет

==> parts/poka_vikinula.tex <==

\begin{definition}
We define the ``wind rose'' as six rays from the origin, with an angle $ \pi / 3 $ between any two adjacent ones, equipped with weights (real numbers) that have the following property: the weight on each ray is the sum of the weights of the rays adjacent to it. (From this, in particular, it follows that the weights on opposite (forming a straight line) rays add up to zero.)
\label{roza_v}
\end{definition}
An example is shown in Figure~\ref{fig:roza1}. A similar construction, but for physical reasons, appears in~\cite{gilbert1968steiner}.
%тут неверное вне плоскости!
\begin{remark}
A full Steiner tree consists of segments belonging to the set of three straight lines with pairwise angles $ \pi / 3 $. Let $ T $ be an arbitrary full Steiner tree. Take an arbitrary wind rose, consisting of rays, parallel to the segments of $ T $, and assign to each end vertex of $ T $ the weight of the ray of this wind rose, co-directed with the segment entering this vertex. Then the sum of numbers over all vertices of $ T $ will be zero.
\label{main_rose_property}
\end{remark}

\begin{remark}
Remark~\ref{main_rose_property} is also true for a local Steiner tree as well as for a full Steiner forest and a local Steiner forest (in the case of forests, multiple wind roses may be required to assign weights to).
\end{remark}


\begin{lemma}
Let $ S $ be a full Steiner forest and  let $ l $ be an arbitrary hyperplane such that no nontrivial ending component of $ S $ is contained in $ l $. By ending component of $S$ we understand such connected subgraph $T$, that $S\setminus T$ has less or equal connected components than $S$.

Then
\[
\sharp(\partial S \cap l) \leq 2\sharp(\partial S \setminus l),
\]
where $\partial S$ is a vertex set of $S$ 
%В частности, бесконечность левой части неравенства влечет неограниченность правой.
\label{St_l_c}
\end{lemma}

\begin{proof}%[Доказательство Леммы~\ref{St_l_c}:]
Let $ S $ have a finite number of vertices. Let $ l^{+} $, $ l^{-} $ be open half-spaces bounded by $ l $. It is easy to see that it is sufficient to separately prove the inequalities for $ \overline {S \cap l^{+}} $, $ \overline {S \cap l^{-}} $. Moreover, it suffices to prove the assertion for one connected component of these sets. Thus, we will prove the assertion for the closure of an arbitrary Steiner tree lying in an open half-space bounded by $ l $.
We place the center of the wind rose in the same open half-plane, choose a wind rose such that all those and only those rays that intersect $ l $ have a positive weight: obviously, such a wind rose exists, since $ l $ intersect $ 2 $ or $ 3 $ in a row going ray. In the first case, we will equip them with weights $ 1, 2, 1 $, in the second $ 1, 1 $. Then the rest of the rays will have weights $ -1, -2, -1 $ or $ 0, -1, -1, 0 $. Let's assign weights to the leaf vertices in the same way as it was done in Remark~\ref{main_rose_property}. Then the sum over the endpoints of $ l $ is at least $ \sharp (S \cap l) $. Due to Remark~\ref{main_rose_property} the sum over all endpoints must be zero, so endpoints not belonging to $ l $ must be at least $ \frac{\sharp (S \cap l)}{2} $.
Let $ S $ have an infinite number of vertices (but still, by the general statement of Steiner problem, is contained in a compact and has a finite length). Assume the statement opposite to the lemma, that is, that $ \sharp (S \cap l) = \infty $, and $ \sharp (\partial S \setminus l) $, on the contrary, is finite. It suffices to prove the statement for each of the half-planes $ l^{+} $ and $ l^{-} $. Without loss of generality, there is a connected component $ S \cap l^{+} $ such that its closure $ T $ has an infinite number of vertices on $ l $. Let $ l'$ be parallel to $ l $ and contained in $ l^{+} $. We will move the straight line $ l'$ inside this half-plane, parallel to $ l $, and denote by $ S (l') $ the Steiner forest, which is the intersection of $ T $ and the half-plane bounded by $ l'$ and not containing $ l $. %As $\H(T)<\infty$ for almost every such lines $\sharp(T\cap l')<\infty$. But if every 
For an arbitrarily large $ N $, there is $ l_0 $ such that $ N <\sharp (l_0 \cap T) <\infty $. Let's choose this $ l_0 $ for $ N = 3 \sharp (\partial T \setminus l) $. This contradicts the already proven statement for $ S (l_0) $.

\end{proof}

\begin{corollary}
Let $ T $ be a full (that is, having no vertices of degree $ 2 $) Steiner tree, $ l $ an arbitrary line such that $ T \not \subset l $. Then
\[  
\sharp(\partial T \cap l)\leq 2\sharp(\partial T \setminus l).
\]
%
\label{St_l}
\end{corollary}


\hline
And 
\[
0\leq (y_i-z_i)-(y_i-\hat{z_i})\leq c\delta^2
\]
for $i \in J$.
Then $\sum_{i\in J}(y_i-z_i)\leq \sqrt r$ and
\[
0\leq \sum (y_i-z_i)^2_{i\in J}-\sum(y_i-\hat{z_i})^2_{i\in J}=\sum_{i\in J}((y_i-z_i)-(y_i-\hat{z_i}))((y_i-z_i)+(y_i-\hat{z_i})) \leq c\delta^2 \sum_{i\in J} (2y_i-z_i-\hat{z_i})\leq 2cr\delta^2(1+c\delta^2).
\]
Id est
\[
\sum_{i\in J}(y_i-z_i)^2 - 2cr\delta^2 \leq \sum(y_i-\hat{z_i})^2_{i\in J}\leq \sum_{i\in J}(y_i-z_i)^2
\]




\[
\sum (y_i-z_i)^2-\sum(y_i-\hat{z_i})^2=\sum_{i\in J}((y_i-z_i)-(y_i-\hat{z_i}))((y_i-z_i)+(y_i-\hat{z_i})) -\sum_{i\in I}(y_i-\hat{z_i})^2\leq
\]
\[
\leq c\delta^2 \sum_{i\in J} (2y_i-z_i-\hat{z_i})-|I|\delta^4\leq 2rc\delta^2+o(\delta^2) .
\]
So 
\[
\sum(y_i-\hat{z_i})^2 \leq \sqrt{ r^2+ 2rc\delta^2}\leq r+2rn\delta^2c.
\]
fr
%Let us construct a union of segments for each flat of $I^m$. Without loss of generality let it be a flat $x_1=\delta$. Then let us consider a point $z_1^+\defeq (r+\delta,0,\ldots,0)$. Then for every vertex of this flat $A_i=(\delta,\pm \delta \ldots \pm \delta)$ there exists point $B_i$ such that $B_i^{1,+} \in[A_i;z_1^+]$ and $|B_i;z_1^+|=r$. Clearly, in view of Pythagorean theorem, $|A_iB_i|=o(\delta)$. Analogously for other flats. Then \[S_i\defeq \bigcup_{j\in \{1;\ldots;m\},s\in \{+,-\} : |A_iz_j^{s}|=r }[A_i;B_i^{j,s}]\] for $i\in\{1, \ldots,2^m\}$. And \[S_0 \defeq \bigcup_{i\in\{1, \ldots,2^m\}}[(0,\ldots,0),A_i].\]


Length inequality is clearly holds. Let $z$ be such point that $\dist (z,I^m)\leq r$. Let $z'$ be the projection from $z$ to $\partial I^m$.


%Then for every vertex $A^{\pm,\ldots, \pm}=(\delta,\pm \delta \ldots \pm \delta)$ there exists point $B^{\pm,\ldots, \pm}$ such that $B^{\pm,\ldots, \pm}\in [A^{\pm,\ldots, \pm},z_1^+]$ and $\H([B^{\pm,\ldots, \pm},z_1^+])=r$. Clearly, in view of Pythagorean theorem, $|A^{\pm,\ldots, \pm},B^{\pm,\ldots, \pm}|=o(\delta)$


\begin{enumerate}
\item Let $t$ be a branching point and let $C$ be such a point that $[tC]$ is a maximal segment in $\Sigma$ and the angle $\angle ((tC], a)=\pi/3-\angle ([t\bar x),(x \bar x])$.%проверить 
Thus $C$ can not be an energetic point of the energetic hyper-space $a$ of order $1$. Then the following cases are possible:Я ТУТ
\begin{enumerate}
    \item $C$ is an energetic point of the energetic hyper-space $a$ of order $2$. By Corollary~\ref{sm_an} $ \angle ((tC], (ax]) \leq \pi/6+\alpha/100$. 
    Hence $\angle ((tC], (ax])$ is equal to $\pi/6$ within $\alpha/50$.
    \item $C$ is an energetic point of the energetic ray $(bx]$
    \begin{enumerate}
        \item $C$ is an energetic point of the energetic ray $(bx]$ of order $1$.
        
        If $ C $ were an energetic point of ray  $ (bx] $ of degree $ 1 $, then there would be a contradiction with the fact that $ [\bar x t] $ lies on the path from $ \bar x $ to $ x $: polyline $ [ \bar x t] \cup [tC] $ and four empty balls of radius $ r $ (empty balls touching the points $ \bar x $ and $ C $ with centers at the corresponding points, as well as two empty balls, tangent to the energetic rays $ (ax] $ and $ (bx] $ centered at the limit points of the points corresponding to the energetic points of the rays) entail the absence of a path from $ \bar x $ to $ x $ in $ \Sigma'$. So we get a contradiction.
        
        \item $C$ is an energetic point of the energetic ray $(bx]$ of order $2$.
        
        Let point $ C $ be an energetic point of ray  $ b $ of degree $ 2 $, then $ \angle ((tC], (bx]) \leq \pi / 6 + \alpha / 100 $. Let $ [tD] $ be the third maximal segment incident to the branching point $ t $. Note that 
         $ \angle ([Dt), (bx])>2\pi/3$. Consider two paths inside $ U $: the path starting from $ t-\bar x $ and the path starting from $ t-D $: we will show that both of them have to contain the single point from $\partial U \cap \Sigma'$, which is impossible: 
        Let the first path does not contain any energetic points of ray  $ (bx] $, so the direction of the tangent along the path changes only at the branching points and energetic points of ray  $ (ax] $ of degree $ 2 $. We require that at the branching points the path continues not by the segment that is $\alpha/50$-almost perpendicular to $ (ax] $.  Then this path does not contain any energetic points of degree $ 1 $ of ray $ (ax]$ and all the angles between $ (ax) $ and the one-sided tangent to $ \Sigma $ along the path do not exceed $ \pi / 6 + \alpha / 100 $. Clearly this path can not end by a limit point, because by Remark otherwise $\bar x$ has two-orientated energetic ray, which is impossible for sufficiently small $\rho_1>0$ as $(ax]$ and $(bx]$ are one-orientated (in what follows we will omit this reasoning). Thus, this path cannot end with an energetic point of degree $ 1 $ and  point $ x $, but then the path inevitably passes through a single point $ \Sigma'\cap \partial U $. Similar reasoning is true for some path starting with $ t-D $ under the assumption that it does not contain energetic points $ (ax] $.
        
 Thus, it is impossible that at the same time the path starting from $ t-\bar x$ does not contain energetic points of the energetic ray $ (bx] $, and the path starting from $ t-D $ does not contain energetic points of ray $ (ax] $. But if the path, starting with $ t - \bar x $, contains an energetic point $ (bx] $, then the second path is bounded by the first path and empty balls of radius $ r $, that is, it does not contain the energetic points of ray  $ (ax] $ and of the boundary $\partial U$, which is impossible. Similarly, the situation is impossible when the path starting with $ t-D $ contains an energetic point of ray  $ (ax] $.       

        
        \end{enumerate}
    \item  $C$   is a branching point %Thus, point $ C $ can only be a branching point. 

 In this case, the path starting from the segments $ [\bar x t] $ and $ [tC] $ and continuing with turns in the same direction can end only if $ C $ is connected by a segment with the energetic point of the energetic ray $ (ax] $ of order $ 1 $ , we denote it by $ x^a_2 $ (this point can not be of order $2$ as $\angle ((Cx^a_2],(ax]) \geq 2\pi/3 - \angle([t\bar x)(ax]) \geq \pi/2-\alpha/50>\pi/6+\alpha/100$. Then the angle $ \angle ((Cx^a_2), (ax)) $ is equal to $ \pi / 2 $ up to $ \alpha / 100 $. In this case, considering the quadrilateral bounded by the lines $ (ax) $, $ (\bar x t), (tC), (Cx^a_2) $, we get 
$\angle  ([t\bar x)(ax])=2\pi/3-\angle ((Cx^a_2),(ax))$,
which, up to $ \alpha / 100 $, is equal to $ \pi / 6 $ (see Fig.~\ref{norm11}).
            \end{enumerate}
Thus, in any case $ \angle ((\bar xt], (ax]) $ is equal to $ \pi / 6 $ up to $ \alpha / 50 $. Let $ [tD] $ be the remaining maximum segment with the end at point $ t $. Then $ \angle ((tD), (ax)) $ is equal to $ \pi / 2 $ within $ \alpha / 50 $, then either $ [tD) $ and $ (bx ] $ do not intersect (if $ \alpha + \angle ((tD), (ax))> \pi $), or $ \angle ((tD], (bx]) $ equals $ \pi / 2- \alpha $ up to $ \alpha / 50 $. In this case, point $ D $ cannot be an energetic point of ray  $ (bx] $ of order $1$. point $D$ also can not be a energetic point of order $2$ or a branching point as in these cases there are two paths in $ \Sigma'$ (a path starting with $ t-\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%: a point of degree $ 1 $ due to Lemma~\ref{alm}, and a point of degree $ 2 $ due to the fact that in this case there are two paths in $ \Sigma'$ (a path starting with $ t\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%Thus, point $ D $ can only be a branching point. However, in this case too, there is a path starting with $ t-D $ that cannot coexist with some path starting with $ t-\bar x $.

This contradicts the assumption that $ t $ is a branching point.
\item Let $t$ be an energetic point of the energetic ray $(bx]$.
Note that
\[
\angle((\bar x t],(bx])= \angle (( \bar x t],(b x]) + \alpha \leq \pi/6+\alpha/100,
\]
in view of Lemma~\ref{alm} and Corollary~\ref{sm_an}, since $t$ can only be an energetic point of ray  $ (bx] $ of degree $ 2 $ belonging to set $ X_\Sigma $. The previous item entails that the maximum segment on the path to $\Sigma $ from $t$ to $ x $ ends with an energetic point of the energetic ray $ (ax] $, we denote it by $ x^a_2 $. This point is of order $2$ and $\angle((tx^a_2),(ax))>\alpha/50$ thus the previous item entails the existence in $\Sigma'$ a polyline $\bar x -t-x^a_2-x^b_2$, where $x^b_2$ is an energetic point of order $2$ of the energetic ray $(bx]$ such that the segment $[x^a_2x^b_2]$ is a maximal segment in a path from $x^a_2$ to $x$ in $\Sigma$. But then the previous item entails the existence in $\Sigma'$ a polyline $\bar x -t-x^a_2-x^b_2-x^a_3$, where $x^a_3$ is an energetic point of order $2$ of the energetic ray $(ax]$ such that the segment $[x^b_2x^a_3]$ is a maximal segment in a path from $x^a_2$ to $x$ and so on, so there exists an infinite polyline with alternating energetic points of two energetic rays as the vertices. Wherein at every step the angle between a segment of polyline and the energetic ray increases by  $\alpha$ within $\alpha/100$ (see Fig.~\ref{norm2}):
$\angle((x^a_kx_k^b],(bx])= \angle ((x_k^bx_k^a], (xx_k^a]) + \alpha $ within $\alpha/100$ and $\angle((x^b_kx^a_{k+1}],(ax])= \angle ((xx^b_k],(x_{k+1}^ax^b_k])+\alpha \geq \angle ((x^a_kx^b_k],(bx])+ \alpha -\alpha/100= \angle ((x_k^bx_k^a], (xx_k^a]) + 2\alpha-\alpha/100$ within $\alpha/100$
for every $k\in \N$ if $x^a_1 \defeq x$ and $x^b_1 \defeq t$.
Thus, there exists a number $ k $ such that $ \angle ((x ^ i_kx ^ j_k), (jx))> \pi / 6 + \alpha / 50 $, where $ \{i, j \} = \{a, b \} $, but then point $ x^k_j $ cannot be an energetic point of degree $ 2 $ of ray  $ (jx] $. The resulting contradiction completes the proof of the step.
\end{enumerate}


%Из утверждения автоматически следует утверждение для любого шара с центром в $x$, содержащегося в $U$, а значит найдется такое $\rho_1>0$ (например, $\rho_1 \defeq \rho_4$), что для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap \overline {B_{\rho_1}(x)} \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.
And now we are finally ready to prove the following lemma, in which it is stated that no connected component of the $ \Sigma \setminus \{ x \}$ can contain infinite sequences of energy points of two different energetic rays converging to $ x $.
\begin{lemma}
Let $\Sigma$ be the a minimizer, $a$ and $b$ be two different energetic hyper-planes with vertices at $x$ and hyper-cusps $Q^{a,x}_\rho \in \mathbb{Q}^{a,x}_\rho$ and $Q^{b,x}_\rho \in \mathbb{Q} ^{b,x}_\rho$ be such that $G_\Sigma \cap \overline{B_\rho(x)} \subset  Q^{a,x}_\rho \cup Q^{b,x}_\rho$ for some $\rho>0$. Let $\Sigma'$ be the connected component of $\Sigma \setminus \{x\}$ containing an infinite sequence of points from set $G_\Sigma \cap  Q^{a,x}_\rho$, converging to $x$. Then there exists such $\rho_3>0$, that 
\[
\Sigma' \cap G_\Sigma \cap  Q^{b,x}_\rho \cap \overline {B_{\rho_3}(x)} = \{x\}.
\]
\label{eva}
\end{lemma}

The sketch of the proof is as follows: suppose the opposite, let $ \Sigma '$ contain an infinite sequence of points from set $G_\Sigma \cap  Q^{b,x}_\rho$, converging to $x$. Then
\begin{enumerate}
\item[Step 1.] There exists such $\rho_1>0$, that $\Sigma' \cap \overline {B_{\rho_1}(x)} \setminus \{ x\}$ doesn't contain the points from $X_\Sigma$ with order $2$ except the ones with incident segments $o_\rho(1)$-almost parallel to the closest energetic hyper-plane $i\in \{a,b\}$.
\item[Step 2.] %There exists such $\rho_2>0$, that $\Sigma' \cap \overline {B_{\rho_2}(x)}\setminus \{ x\}$ doesn't contain any energetic points with order $2$ 
There exists such $\rho_2>0$, that $\Sigma' \cap \overline {B_{\rho_2}(x)}\setminus \{ x\}$ has a tangent line in each energetic points. %with order $2$ 
\item[Step 3.] The angle $\angle (a,b)$ can be only $\pi/3$, $2 \pi/3$ or $\pi$.
\item[Step 4.] Obtaining a contradiction in each of the three possible cases.% by remark~\label{vector}.
\end{enumerate}
\begin{proof}
In view of the assumption that there are two different energetic hyper-planes, we can assume that each of the energetic hyper-planes is one-orientated.
Let's denote the value of the internal angle between the hyper-planes by $ \alpha$ (id est the angle doesn't contain any points corresponding to $\Sigma \cap B_{\rho}(x)$): $ \alpha \defeq \angle (a,b]) < \pi $. 
\textcolor{red}{Let also $y^a,y^b \in M$ be such points corresponding to $x$ that $(y^ax)\perp a$ and $(y^bx)\perp b$. }%Such points exists due to!
It is possible, without loss of generality, to consider $ \rho_1 \leq \rho $ such that the statements of Lemma~\ref{alm} for $ c \defeq \alpha / 100 $ hold and that for every point $z \in Q^{i,x}_{\rho} \cap \overline{B_{\rho_1}(x)}$ inequality $|\angle zxy^i-\pi/2 |\leq \alpha/100$ holds, where $i=a,b$. We also get such a small $\rho_1$ that all points corresponding to the same energetic hyper-planes (excluding $x$) are located at the same semi-space with respect to the energetic hyper-planes (It is possible due to item~\ref{1115} of Lemma~\ref{Losiu}) and for every energetic point $\bar x \in \overline{B_{\rho_1}(x)}$ the inequality $\angle (y(\bar x)\bar x],(y^ix]$, where $i\in {a,b}$ is the nearest to $\bar x$ energetic hyper-plane. 
In the proof we still use the formulation ``the values \ldots are equal to within $ \bar c $ '', which mean that the absolute value of the difference between the values does not exceed $ \bar c $.
Let area $U \ni x$ be such that $U \subset B_{\rho_1}(x)$ and $\sharp (\partial U \cap \Sigma)=\oord_x\Sigma$. Then $\sharp (\partial U \cap \Sigma')=1$, and hence for each point $\bar x \in \Sigma' \cap U \setminus{x}$ there exists only one path to $\partial U$, and the path from $\bar x$ to $x$ is contained in $U \subset B_\rho(x)$. 
\begin{itemize}

\item{Step 1.} For any point $ \bar {x} \in G_\Sigma \cap \Sigma'\cap U \setminus \{x \} $ with $\oord_x\Sigma =2$, the tangent rays to $ \bar x $ are $\alpha/10$-almost parallel to the nearest energetic hyper-plane $i$.

Assume the contrary: let there exists such an energetic point 
$\bar x \in B_{\rho_1}(x) \setminus \{x\}$ with order $2$ that it has a tangent ray with angle with the closest to $\bar x$ energetic hyper-plane greater then $\alpha/10$. Thus by item~\ref{AB} Lemma~\ref{alm} point $\bar x$ belongs to $X_\Sigma$ and hence there exists nontrivial segments $[s\bar x], [t\bar x] \subset \Sigma$. Without loss of generality let $[\bar x t]$ be the maximal segment in the path from $\bar x$ to $x$. Thus, by Corollary~\ref{sm_an}, as $\bar x \in Q^{i,x}_{\rho_1}$, $\angle ((t\bar x], (y(\bar x),\bar x])-\pi/2  \leq \pi/6 +\alpha/100$. %Thus, by Corollary~\ref{sm_an}, as $\bar x \in Q^{i,x}_{\rho_1}$, $\angle ((t\bar x],i)  \leq \pi/6 +\alpha/100$. 
So
\begin{equation}
\alpha/10 <\angle ((t\bar x],( x y(\bar x)])-\pi/2\leq \pi/6 +\alpha/50.
\label{hu}
\end{equation}
Without loss of generality let $i \defeq a$. Point $t$ can not be an energetic point of the energetic hyper-plane $a$ as $a$ is one-orientated and due to choice of $U$.
% Lemma~\ref{alm} and Corollaries~\ref{sm_an} and~\ref{notv}%проверить.
It also can not coincide with $x$ due to definition of $Q^{a,x}_{\rho_1}\ni x$. Thus point $t$ can be an energetic point of order $2$ of the another energetic hyper-plane $b$ or it can have order $3$.

 
 \input{pictures/trash/norm1}
\input{pictures/trash/norm2}
\input{pictures/trash/norm11}

\begin{enumerate}
\item Let $t$ be of order $3$ and let $C\neq \bar x$ be such a point that $[tC]$ is a maximal segment in $\Sigma$ and the sign sign$(\angle y(\bar x)\bar x t)=$sign $(\angle \bar x t C)$. Then 
$\angle ((tC],(y^ax))> \pi/6-\alpha/50$ and
%$\angle ((tC], a)=\pi/3-\angle ([t\bar x),(x \bar x])$.%проверить 
thus $C$ can not be an energetic point of the energetic hyper-space $a$ of order $1$. Then the following cases are possible:
\begin{enumerate}
    \item $C$ is an energetic point of the energetic hyper-space $a$ of order $2$. Clearly, up to $\alpha/50$ 
    \[
    \angle ((tC],(y^ax))=\angle ((t\bar x],(y(\bar x) \bar x))-\frac{\pi}{3}\in [\frac{\pi}{6}+\frac{\alpha}{10},\frac{\pi}{3}]
    \]
    At the same time, by Corollary~\ref{sm_an}, $ |\angle ((tC], (y^ax))-\pi/2| \leq \pi/6+\alpha/100$. 
    Hence $\angle ((tC], a)$ is equal to $\pi/6$ within $\alpha/50$.
    %\item $C$ is an energetic point of the energetic hyper-plane $b$.Я ТУТ
    %\begin{enumerate}
        \item $C$ is an energetic point of energetic hyper-plane $b$ of order $1$.
        Let $[tz]$ be the last maximal segment of $\Sigma$ incident to $t$. Thus $[tz)$ has 
        angles with normals $[xy^a)$ and $[xy^b)$ greater than $\pi/2$ and angles with hyper-planes $a$ and $b$ greater than $\pi/6-\alpha/50$. Thus $z$ can not be an energetic point of order $1$ or $2$ and hence there exists maximal segments $[zz_1]$ and $[zz_2]$ such that all three segments incident to $z$ lay in the same plane and have pairwise angles equal to $2\pi/3$. Clearly for $i\in\{1;2\}b$ the angles of $[zz_i)$ has  with normals $[xy^a)$ and $[xy^b)$ are greater than $2\pi/3$.% and angles with hyper-planes $a$ and $b$ greater than $\pi/6-\alpha/50$.. 
        And so on, we can iterate this process and get an infinite path which can not finish at $\partial U$ due to choice of $U$ or by energetic point !ТУТ НАДО НА ЧТО-ТО СОСЛАТЬСЯ, ТИПА ТОГО ЧТО У ПРЕДЕЛЬНОЙ ТОЧКИ ОБЯЗАТЕЛЬНО ДОЛЖЕН БЫТЬ ТАКАЯ ОКРЕСТНОСТЬ ИЛИ ШАР ЧТО ПЕРЕСЕЧЕНИЯ В ТОЧКАХ НА ПРАВИЛЬНЫХ УГЛАХ
        
        ИЛИ НА ТО ЧТО ИЗ-ЗА ОРИЕНТАЦИИ ГИПЕРПЛОСКОСТИ в ОДНУ СТОРОНУ НЕ МОЖЕТ БЫТЬ ПРЕДЕЛА 
        
        %as the path, consisting of two iterating directions, will have a tangent RAY at the limit point, and this tangent RAY HAVE angles with hyper-planes $a$ and $b$ greater than $\pi/6-\alpha/50$                           
        
        \item $C$ is an energetic point of order $2$ of the energetic hyper-plane $b$.
        
        Let point $ C $ be an energetic point of  hyper-plane $ b $ of degree $ 2 $, then 
        \[
        -\frac{\alpha}{50}< \angle((tC],(y^bx])-\frac{\pi}{2}<\frac{\pi}{6}+\frac{\alpha}{50}.
        \]
        Let $ [tD] $ be the third maximal segment incident to the branching point $ t $. Note that 
         $ \angle ([Dt), (bx])>2\pi/3$. Consider two paths inside $ U $: the path starting from $ t-\bar x $ and the path starting from $ t-D $: we will show that both of them have to contain the single point from $\partial U \cap \Sigma'$, which is impossible: 
        Let the first path does not contain any energetic points of ray  $ (bx] $, so the direction of the tangent along the path changes only at the branching points and energetic points of ray  $ (ax] $ of degree $ 2 $. We require that at the branching points the path continues not by the segment that is $\alpha/50$-almost perpendicular to $ (ax] $.  Then this path does not contain any energetic points of degree $ 1 $ of ray $ (ax]$ and all the angles between $ (ax) $ and the one-sided tangent to $ \Sigma $ along the path do not exceed $ \pi / 6 + \alpha / 100 $. Clearly this path can not end by a limit point, because by Remark otherwise $\bar x$ has two-orientated energetic ray, which is impossible for sufficiently small $\rho_1>0$ as $(ax]$ and $(bx]$ are one-orientated (in what follows we will omit this reasoning). Thus, this path cannot end with an energetic point of degree $ 1 $ and  point $ x $, but then the path inevitably passes through a single point $ \Sigma'\cap \partial U $. Similar reasoning is true for some path starting with $ t-D $ under the assumption that it does not contain energetic points $ (ax] $.
        
 Thus, it is impossible that at the same time the path starting from $ t-\bar x$ does not contain energetic points of the energetic ray $ (bx] $, and the path starting from $ t-D $ does not contain energetic points of ray $ (ax] $. But if the path, starting with $ t - \bar x $, contains an energetic point $ (bx] $, then the second path is bounded by the first path and empty balls of radius $ r $, that is, it does not contain the energetic points of ray  $ (ax] $ and of the boundary $\partial U$, which is impossible. Similarly, the situation is impossible when the path starting with $ t-D $ contains an energetic point of ray  $ (ax] $.       

        
       % \end{enumerate}
    \item  $C$   is of order $3$% a branching point %Thus, point $ C $ can only be a branching point. 
    ПРОВЕРИТЬ ЧТО ЭТО В ТОЧНОСТИ ЗНАЧИТ БРАНЧИНГ(

 In this case, the path starting from the segments $ [\bar x t] $ and $ [tC] $ and continuing with turns in the same direction can end only if $ C $ is connected by a segment with the energetic point of the energetic ray $ (ax] $ of order $ 1 $ , we denote it by $ x^a_2 $ (this point can not be of order $2$ as $\angle ((Cx^a_2],(ax]) \geq 2\pi/3 - \angle([t\bar x)(ax]) \geq \pi/2-\alpha/50>\pi/6+\alpha/100$. Then the angle $ \angle ((Cx^a_2), (ax)) $ is equal to $ \pi / 2 $ up to $ \alpha / 100 $. In this case, considering the quadrilateral bounded by the lines $ (ax) $, $ (\bar x t), (tC), (Cx^a_2) $, we get 
$\angle  ([t\bar x)(ax])=2\pi/3-\angle ((Cx^a_2),(ax))$,
which, up to $ \alpha / 100 $, is equal to $ \pi / 6 $ (see Fig.~\ref{norm11}).
            \end{enumerate}
Thus, in any case $ \angle ((\bar xt], (ax]) $ is equal to $ \pi / 6 $ up to $ \alpha / 50 $. Let $ [tD] $ be the remaining maximum segment with the end at point $ t $. Then $ \angle ((tD), (ax)) $ is equal to $ \pi / 2 $ within $ \alpha / 50 $, then either $ [tD) $ and $ (bx ] $ do not intersect (if $ \alpha + \angle ((tD), (ax))> \pi $), or $ \angle ((tD], (bx]) $ equals $ \pi / 2- \alpha $ up to $ \alpha / 50 $. In this case, point $ D $ cannot be an energetic point of ray  $ (bx] $ of order $1$. point $D$ also can not be a energetic point of order $2$ or a branching point as in these cases there are two paths in $ \Sigma'$ (a path starting with $ t-\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%: a point of degree $ 1 $ due to Lemma~\ref{alm}, and a point of degree $ 2 $ due to the fact that in this case there are two paths in $ \Sigma'$ (a path starting with $ t\bar x $ and a path starting with $ t-D $) that cannot coexist (the proof is similar to that discussed above).
%Thus, point $ D $ can only be a branching point. However, in this case too, there is a path starting with $ t-D $ that cannot coexist with some path starting with $ t-\bar x $.

This contradicts the assumption that $ t $ is a branching point.
\item Let $t$ be an energetic point of the energetic ray $(bx]$.
Note that
\[
\angle((\bar x t],(bx])= \angle (( \bar x t],(b x]) + \alpha \leq \pi/6+\alpha/100,
\]
in view of Lemma~\ref{alm} and Corollary~\ref{sm_an}, since $t$ can only be an energetic point of ray  $ (bx] $ of degree $ 2 $ belonging to set $ X_\Sigma $. The previous item entails that the maximum segment on the path to $\Sigma $ from $t$ to $ x $ ends with an energetic point of the energetic ray $ (ax] $, we denote it by $ x^a_2 $. This point is of order $2$ and $\angle((tx^a_2),(ax))>\alpha/50$ thus the previous item entails the existence in $\Sigma'$ a polyline $\bar x -t-x^a_2-x^b_2$, where $x^b_2$ is an energetic point of order $2$ of the energetic ray $(bx]$ such that the segment $[x^a_2x^b_2]$ is a maximal segment in a path from $x^a_2$ to $x$ in $\Sigma$. But then the previous item entails the existence in $\Sigma'$ a polyline $\bar x -t-x^a_2-x^b_2-x^a_3$, where $x^a_3$ is an energetic point of order $2$ of the energetic ray $(ax]$ such that the segment $[x^b_2x^a_3]$ is a maximal segment in a path from $x^a_2$ to $x$ and so on, so there exists an infinite polyline with alternating energetic points of two energetic rays as the vertices. Wherein at every step the angle between a segment of polyline and the energetic ray increases by  $\alpha$ within $\alpha/100$ (see Fig.~\ref{norm2}):
$\angle((x^a_kx_k^b],(bx])= \angle ((x_k^bx_k^a], (xx_k^a]) + \alpha $ within $\alpha/100$ and $\angle((x^b_kx^a_{k+1}],(ax])= \angle ((xx^b_k],(x_{k+1}^ax^b_k])+\alpha \geq \angle ((x^a_kx^b_k],(bx])+ \alpha -\alpha/100= \angle ((x_k^bx_k^a], (xx_k^a]) + 2\alpha-\alpha/100$ within $\alpha/100$
for every $k\in \N$ if $x^a_1 \defeq x$ and $x^b_1 \defeq t$.
Thus, there exists a number $ k $ such that $ \angle ((x ^ i_kx ^ j_k), (jx))> \pi / 6 + \alpha / 50 $, where $ \{i, j \} = \{a, b \} $, but then point $ x^k_j $ cannot be an energetic point of degree $ 2 $ of ray  $ (jx] $. The resulting contradiction completes the proof of the step.
\end{enumerate}


%Из утверждения автоматически следует утверждение для любого шара с центром в $x$, содержащегося в $U$, а значит найдется такое $\rho_1>0$ (например, $\rho_1 \defeq \rho_4$), что для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap \overline {B_{\rho_1}(x)} \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.

\item[Step 2.] Every energetic point of $\Sigma' \cap U \setminus \{x\}$ belongs to set $X_\Sigma$ and has the order $1$.
\begin{proof}
Assume the contrary: due to item~\ref{__1} of Lemma~\ref{alm} and step 1 it means that there exists such $\bar x \in \Sigma' \cap U \setminus \{x\}$ of order $2$ that it belongs to $E_\Sigma$ (and hence by Lemma~\ref{alm} and Corollary~\ref{notv} there exist one-sided tangents at $\bar x$ $\alpha/100$-almost parallel to $(ix]$, the closest energetic ray to $\bar x$) or to $X_\Sigma$ with both incident segments $\alpha/10$-almost parallel to $(ix]$. 

Consider the path from $\bar x$ to $x$. This path is contained in $U$ by definition of $U$ and its points by Remark~\ref{remA} can not be a limit point of the branching points. НАДО ПЕРЕДЕЛАТЬ ЧЕГО-ТО Thus if this path contains some branching points one can pick the first branching point $C_0$. Then, in view of compactness of $E_\Sigma$, we can take the last energetic point $B$ from the path from $\bar x$ to $C_0$  (it may coincide with $\bar x$). Thus the path from $B$ to $C_0$ has to be a segment and, due to Lemma~\ref{alm}, Corollary~\ref{notv} and step 1, this segment is contained in a line, $\alpha/100$-almost parallel to $(jx]$, energetic ray closest to $B$ for $j\in \{a,b\}$. Without loss of generality let $j=a$. Consider the maximal segment $[C_0C_1]\subset \Sigma'$, such that $\angle((ax](C_0C_1])$ is equal to $\frac{\pi}{3}$ within $\alpha/100$. Hence, by Lemma~\ref{alm} and Corollary~\ref{sm_an} $C_1$ can not be an energetic point and thus it has to be a branching point. Then let $[C_1C_2] \subset \Sigma'$ be such a maximal segment that it is not contained in a almost parallel to $(ax)$ line and hence $\angle((ax](C_1C_2])$ is equal to $\frac{2\pi}{3}$ within $\alpha/100$. Thus $C_2$ has to be a branching point. But then the path, beginning by $C_0-C_1-C_2-\ldots$ and continuing by the alternating turns (id est the injective polyline $\bigcup_{j=0} [C_j C_{j+1}]$, with $\angle((ax](C_{j}C_{j+1}])=\pi-\angle((ax](C_{j-1}C_{j}])$) can not ends.

If the path from $ \overline{x} $ to $ x $ does not contain any branching points, then the arc $ \breve{]\overline{x} x[} $ will also have no energetic points of the energetic ray $ (bx] $: otherwise, let $ x_b $ be the first such point; and let $ x_a $ be the last energetic point of ray  $ (ax] $ from this arc before $x_b$ ($x_a \in Q^{a,x}_{\rho_1}$ and $x_b \in Q^{b,x}_{\rho_1}$ are the different points because $Q^{a,x}_{\rho_1}\cap Q^{b,x}_{\rho_1} =\{x\}$). In this case, the arc $ \breve{x_a x_b} $ is a segment, contained in a line almost parallel to both energetic-rays, which is impossible:
\[
\angle ((x_a x_b), (ax)) \leq \alpha/10
\]
and
\[
\angle ((x_a x_b), (bx)) \leq \alpha/10
\]
entails
\[
\alpha=\angle((ax],(bx]) =\angle((ax),(bx))\leq \alpha/5,
\]
which is impossible for $\alpha>0$. 

Thus the path from $\bar x$ to $x$ doesn't contain any energetic points of the energetic ray $(bx]$ or any branching points, id est in each point of the path the tangent ray of $\Sigma'$ is $\alpha/10$ almost parallel to $(ax]$. Then there exists such open area $U_0 \subset B_{|\bar x x|}(x)$, that $x \in U_0$, $\sharp (\partial U \cap \Sigma ) = \oord_x \Sigma$. Then $U_0 \cap \Sigma' \subset \breve{\overline{x}x}$ doesn't contain any energetic points of ray  $(bx]$. So we get a contradiction with a definition of $\Sigma'$ for $\rho_2 \defeq \rho_1$.

%для $\rho_2 \defeq \rho_4$.
%Из утверждения автоматически следует утверждение для любого шара с центром в $x$, содержащегося в $U$, то есть найдется такое $\rho_2>0$ (например, $\rho_2 \defeq \rho_4$), что любая точка $\bar{x} \in G_\Sigma \cap  \Sigma' \cap \overline{B_{\rho_2}(x)} \setminus \{ x\}$ принадлежит множеству $X_\Sigma$ и имеет порядок $1$.
\end{proof}

\item [Step 3]
Let $ U_1 \ni x $ be an open area of sufficiently small diameter (so that $ \Sigma'\cap (U \setminus U_1) $ contains sufficiently many energetic points of both energetic rays: for example at least three energetic points of each energetic ray) such that $ U_1 \subset U $, $ \sharp (\partial U_1 \cap \Sigma) = \oord_x \Sigma $.
In view of the previous steps, $\overline{\Sigma'\cap (U \setminus U_1)} $ is a locally minimal tree (with a finite number of vertices) without vertices of degree $ 2 $. Then there exist three lines with pairwise angles $ \pi / 3 $ such that each segment of $ \overline{\Sigma'\cap (U \setminus U_1)} $ is parallel to one of them.
Each endpoint of the Steiner tree $ \overline{\Sigma'\cap (U \setminus U_1)} $, except two points of $ (\partial U \cup \partial U_1) \cap \Sigma' $, lies on a segment belonging to the line $\alpha/100$-almost perpendicular to one of the rays. Therefore, since set $ \Sigma'\cap (U \setminus U_1) $ contains the energetic points of both rays, the angle $ \alpha = \angle axb \leq \pi$ can only be $\frac{\pi}{3}$, $\frac{2\pi}{3}$ or $\pi$ within $\alpha/100$.
%\end{enumerate}

\item[ Step 4]
\input{pictures/trash/roza1}
\input{pictures/trash/roza2}
\input{pictures/trash/roza3}
Let us construct the wind rose with the center inside the internal angle $\angle axb$ and the lines, containing perpendiculars to both energetic rays $(ax]$ and $(bx]$. We put the weights depending on angle $\angle axb$:
\begin{itemize}
\item If $\alpha = \frac{\pi}{3}$ then put $1$ at both rays directed towards to $(ax]$ and $(bx]$ and perpendicular to it (see Fig.~\ref{fig:roza1}). Thus there are weights $-1$ at the complementary rays, and weights $2$ and $-2$ at the last line.
 \item If $\alpha = \frac{2\pi}{3}$ then put $1$ at the ray, perpendicular to $(ax]$ and directed towards to it, and put $2$ at the ray, perpendicular to $(bx]$ and directed towards to it (see Fig.~\ref{fig:roza2}). Thus there are weights $-1$ and $-2$ at the complementary rays, and weights $1$ and $-1$ at the last line.
 \item If $\alpha = \pi$ we put $1$ at the ray directed towards to $(ab)$  and perpendicular to it, and weights $-1$ and $0$ at the remaining ones (see Fig.~\ref{fig:roza3}). Thus there are weights $-1$, $1$ and $0$ at the complementary rays.
 \end{itemize}
 
 Now, as in Remark~\ref{main_rose_property}, we assign to each terminal vertex of tree  $\overline{\Sigma \cap U}$ the weight of the ray of the corresponding wind rose, co-directed with the segment entering this vertex.
 
 
 
% We now associate a tree $\overline{\Sigma \cap U}$ with a directed graph (one segment can be associate to two edges if there are only two vertices at the graph) with weights, where the weight of each edge is equal to the weight of the edge of wind rose, $\alpha/100$-almost co-directional to it.
 
 %Выберем также $\rho_1<\rho_4$ так, чтобы $\sharp(\Sigma \cap \partial(B_{\rho_1}(x)))\leq 3$, а количество энергетических точек $\Sigma' \cap B_{\rho_4}(x)\setminus B_{\rho_1}(x)$ было достаточно велико.
 
By Remark~\ref{main_rose_property}, sum of all weights of $\Sigma' \cap (U \setminus U_1)$ is equal to $0$. On the other hand, sum is positive, as there are arbitrarily many positive terms, and at most two negative. So we get a contradiction.

\end{itemize}

\end{proof}

As $\Sigma_1$ is a compact set, there exists a minimal by inclusion finite collection $\{x_i\}_{i\in I}\subset \Sigma_1$ such that $\Sigma_1 \subset \bigcup_{i \in I} B_{\delta(x_i)}(x_i)$.
%If there is no other $x_i$ on path in $\Sigma_1$ from $x_a$ to $x_b$ we will say that these vertices are adjacent. \textcolor{blue}{расписать поподробнее, почему в этом случае весь путь лежит в объединении их шариков}
%\textcolor{red}{Consider the subpartition $\{x_i,s_i,t_i\}_{i\in I}$ of the partition $\{x_i\}_{i\in I}$ such that 
%there exists such a finite partition $\{x_i,s_i,t_i\}_{i\in I}$ of $\Sigma_1$ that for adjacent vertices of the tree $x_a,x_b,x_c$ points lay in $\Sigma_1$ in the order $x_a,s_a,t_a, x_b, s_b, t_b, x_c$ and the following equalities are true: $|x_at_a|=\bar{\varepsilon}(x_a)$, $|s_ax_b|=\bar{\varepsilon}(x_b)=|x_bt_b|$, $|s_bx_c|=\bar{\varepsilon}(x_C)$ and $|s_it_i|=o(\min_{i\in I}\bar{\varepsilon}(x_i))$, $\bar{\varepsilon}(x_i)\leq \varepsilon(x_i)$ for every $i \in I$ and $\oord_{\bar x}\Sigma_1 = \sharp ( \Sigma_1 \cap \partial B_{\bar{\varepsilon}(\bar x)}(\bar x) )$.The subpartition exists as we can construct it by such a way: } 
This collection contains $F$ because $\delta(x_i) < d(x_i) / 2$, so $F \notin B_{\delta(x_i)}(x_i)$ for every $i \in I$. Define a graph $T$ on the set of vertices $V(T) \defeq \{x_i\}_{i \in I}$ as follows: let $(x_a, x_b) \in E(T)$, i.e. let $x_a$ and $x_b$ be adjacent, if and only if there is no other $x_i$ on the path $\Sigma_1(x_a, x_b)$.
\textcolor{red}{Note that for every $i\in I$ set $B_\varepsilon(x_i)\cap \Sigma_1$ is connected and there is no such $j\neq i\in I$ that $B_{\varepsilon_i}(x_i) \cap \Sigma_1 \subset B_{\varepsilon_j}(x_j) \cap \Sigma_1$ ой извини не заметила что это там ниже уже написано (надо бы перенести до утверждения про отсутствие циклов)}
\textcolor{blue}{добавить обозначение для пути между вершинами куда-нибудь} Note that $T$ is a tree because $\Sigma_1$ is connected and does not contain cycles. \textcolor{blue}{на самом деле этих аргументов недостаточно, надо нормально объяснить}
\textcolor{red}{Assume $T$ contains a cycle. Thus there exists two adjacent vertices $x_A$ and $x_B$ with other, except the edge, path between them in $T$. That path should contain a vertex, let us denote it by $x_C$. But, as $\Sigma_1$ doesn't contain any cycles, the paths $\Sigma_1(x_A, x_C)$ and $\Sigma_1(x_B, x_C)$ intersects not only by point $x_C$, but also by some nontrivial arc. Thus there exists a branching point $D\in \Sigma_1(]x_A, x_C[) \cap \Sigma_1(]x_B, x_C[)$. As $x_A$ and $x_B$ are adjacent points, $D$ is not a vertex of $T$. Let $x_E$ be a first vertex of $T$ in the path of $\Sigma_1$ from $D$ to $x_C$. Clearly, by conditions on the number of points $\Sigma_1$ at the boundaries $\partial B_{\delta(x_i)}(x_i)$ and the condition of not-containing, that  $D\notin \bigcup_{i\in \{A,B,E\}}B_{\delta(x_i)(x_i)}$ and also $D\notin B_{\delta(x_j)}(x_j)$ for any other $j\in I$ due to connectivity condition. So $D\notin \bigcup_{i\in I}B_{\delta(x_i)}(x_i)$ and we get a contradiction}
Note that for each $i \in I$ the set $\Sigma_1^i \defeq \Sigma_1 \cap B_{\delta(x_i)}(x_i)$ is connected, $\sharp ( \partial \Sigma_1^i ) = \oord_{x_i} \Sigma_1$ and $\Sigma_1^i \not\subset \bigcup_{j \in I \setminus \{i\}} \Sigma_1^j$. It follows that if $\Sigma_1^a \cap \Sigma_1^b \neq \emptyset$, then $\Sigma_1(x_a, x_b)$
\textcolor{red}{is contained in $B_{\delta(x_a)}(x_a)\cup B_{\delta(x_b)}(x_b)$. Otherwise there exists point $z\in \Sigma_1(x_a, x_b)\setminus B_{\delta(x_a)}(x_a)\cup B_{\delta(x_b)}(x_b)$ and $c\in I$ such that $z\in B_{\delta(x_c)}(x_c)$. But then $\Sigma_1(z,x_c)\subset B_{\delta(x_c)}(x_c)$ and, as $\oord_{x_C}\Sigma_1(z,x_c)=1$ for $j\in \{a,b\}$ there holds $\Sigma_1\cap B_{\delta(x_j)}(x_j)\subset B_{\delta(x_c)}(x_c)$, so we get a contradiction.}

\textcolor{red}{Note also that for every adjacent vertices $x_a,x_b$ the angles $\angle sx_ax_b, sx_bx_a\leq 2\gamma$ for every $s\in \Sigma_1(x_ax_b)$. Without loss of generality let $\delta(x_b)\geq \delta(x_a)$ so $\angle sx_bx_a\leq \gamma$ by definition of $\delta(\cdot)$. Assume $\angle sx_ax_b>2\gamma$, then
\[
\H(\Sigma_1(x_ax_b))\geq |x_as|+|sx_b|\geq :(( 
\]
все сломалось в случае если $sx_b$ сильно больше $sx_a$ а угол $sx_bx_a$ очень маленький 
and thus
\[
\Sigma \setminus S_1(x_ax_b)\cup [x_ax_*b]\cup S^*(x_a,\delta(x_a))\cup S^*(x_b,\delta(x_b))
\]
is better than $\Sigma$, so we get a contradiction. ИДЕЯ ПОЧИНКИ: сказать что этих отвратительных ситуаций очень мало (то есть суммарная длина сигмы в них -- ошка от не в них), и они не могут сильно помешать. Но у нас там сложение направлений, так что непонятно(}


==> parts/thoughts.tex <==
Какие задачи вообще интересно ставить и решать?

Не задача "является ли $\Sigma$ чьим-то минимайзером  и чьим, если является", а что-то похожее?

Компьютерная проверка этого? (с вероятностным ответом нет, и приближенным ответом да)
(Вообще дискретная задачка. Непрерывность заменяется на минимальное расстояние от точки до множества остальных точек.)

Например, найти минимальное такое $M$, что $\Sigma$ его минимайзер. Если минимальное по включению, то там будут криволинейные дуги понятно какой кривизны и точки. Возможно надо просить связность $M$ и минимальность по длине. Как связаны две этих минимальности?

Построить такую последовательность множеств, где каждый предыдущий -- минимайзер для следующего (при одинаковых $r$), причем следующий минимальный.
Верно ли что можно убрать k членов заменив r на (k+1)r?

что там для подковы?кажется, тоже подкова? если бы не было связности, а вместо минимальности по длине  была бы минимальность по включению, была бы дуга окружности и конечный набор точек. А если попросить цикличность (как в коммивояжере?), получится ли окружность?

Или пучок при $t\in[0;1]$ смотрим на минимайзеры или обратные минимайзеры для $tr$.

_______
какие-то сжимающие отображения, воздействующие на оба множества? СИММЕТРИЗАЦИЯ НЕ УДОВЛЕТВОРЯЕТ!
образ минимайзера по-прежнему удовлетворяет условиям обсуживания, но может перестать удовлетворять локальным условиям, то есть перестать быть минимайзером. Это наверное дает какие-то утверждения про симметричность (и другую устойчивость к сжимающим преобразованиям) М при симметричности Сигма.


Если верно что :
Пусть у x энергетические гиперплоскости ориентированы в однеу сторону. Тогда у него есть такая окрестность в которой все эн точки такие и в частности не являются пределом точек ветвления.

Кстати хорошо бы написать следствие сразу:
что либо не больше двух касательных плоскостей, либо не предел тв ??? что-то не так

==> parts/trash.tex <==
% \begin{lemma}
% Let $\Sigma$ be a minimizer for a compact set $M \subset \mathbb{R}^2$ and $r>0$. And let $x \in \Sigma \cap G_\Sigma$. Then for every $c>0$ there exists such $(\Sigma,x)$-nice $\rho>0$ that for every $\bar x \in \Sigma' \cap B_\rho(x)$ where $\Sigma'$ is an arbitrary connected component of $\Sigma \setminus x$ and $(ax]$ is the unique tangent ray of $\Sigma'$ at the point $x$ and $\{y_1,y_2\}$ are such a points that $r=|y_1x|=|y_2x|$, $x\in (y_1y_2)$ and $(y_1y_2) \perp (ax)$ 
% there holds
% \begin{enumerate}
% \item if $\oord_{\bar x}\Sigma=1$, then $\bar x \in X_\Sigma$ and hence there exists non-degenerate segment $[s\bar{x}] \subset \Sigma$ and the following inequality is true:  \[\angle((s\bar{x})(ax))>\pi/2-c.\] 
% In the other words
%  \[
%  \angle ([s\bar{x}), [xy))<c.
%  \]
%  for $y\in\{y_1,y_2\}$ be a limit point of the points corresponding to the sequence of energetic points of $\Sigma'$ converging to $x$.
%  In other words the segment $[s\bar x]$ is $o_{|\bar xx|}(1)-$almost perpendicular to $(ax)$.
% \label{__1}
%     \item  if $\bar x \in X_\Sigma$ and  $\oord_{\bar x} \Sigma=2$, then the angle of incidence is almost equal to the angle of reflection:
% \[|\angle((s\bar{x}], (ax))-\angle( (ax),(t\bar{x}])|<c\mbox{, for disjoint non-degenerate segments } [s\bar{x}[, [t\bar{x}[ \subset \Sigma;\]
% \label{__2}
% \item if $\bar {x} \in E_\Sigma$, then there exists such $\varepsilon>0$ that $B_\varepsilon(\bar x) \cap \Sigma$ is contained in the union of two cusps (and each cusp is not empty) with axes $(m\bar{x}]$ and $(n\bar{x}]$, almost parallel to $(ax)$, id est $|\angle((m\bar{x}],(ax))|<c$ and $|\angle((n\bar{x}],(ax))|<c$. 
% \label{__3}
% \end{enumerate}
% \label{alm}
% \end{lemma}
% \begin{proof}
% This lemma is particular case of~\ref{napr}.
% \end{proof}

% \begin{proposition}
% For an arbitrary $x \in E_\Sigma$ and $\bar c>0$ there exists such $\rho>0$, that if $\Sigma \cap B_\rho(x)$ contains a polyline $L_1-L_2-L_3-L_4-L_5$, the nodes of which are energetic points of the same energetic ray $(ix]$ and all its internal points are of order $2$, then $\angle((L_jL_{j+1}),(ix)) \leq \bar c$ for every $j=1, \dots, 4$ (see Fig.~\ref{fig:dvapo}).  
% \label{brrrr}
% \end{proposition}
% \begin{proof}
% Let $\rho>0$ be such small that conditions of Lemma~\ref{alm} for $c=\bar c/10$ holds. Assume the contrary to the desired statement: id est $\angle((L_jL_{j+1}),(ix) > \bar c$ for some $j\in\{1,\dots,4\}$. Due to  Lemma~\ref{alm} points $L_1$,\ldots, $L_5$ belong to $X_\Sigma$ and inequality $\angle((L_jL_{j+1}),(ix))> \bar{c}/2$ holds for every $j=1,2,3,4$. By Remark~\ref{rem_cc}, for sufficiently small $\rho>0$ $\angle ((L_{j-1}L_{j}],(L_{j+1},L_j]) \leq \pi-\bar c/2$ for $j \in \{2,3,4\}$, so points of $M$ corresponding to $L_j$ with odd and even indices located at the different semi-plane with respect to $(ix)$. %Really, from Remark~\ref{rem_cc} we have $|\angle((ix), (L_jy(L_j))-\pi/2|<\bar c/10$ for every $j\in 1, \ldots, 5$, 
% Note that the ratio between the lengths of the sides of polyline is linear. Really, by law of sines and inequality $\angle L_{j-1}L_jL_{j+1}\geq 2\pi/3$ we get
% \[
% \frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}=\frac{\sin \angle L_{j-1}L_{j+1}L_j}{\sin \angle L_jL_{j-1}L_{j+1}}\geq \frac{\sin (c/2+o_\rho(1))}{\sin (\pi/3)}\geq \frac{\bar c}{3}.
% \]
% On the other hand
% \[
% \frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}=\frac{\sin \angle L_{j-1}L_{j+1}L_j}{\sin \angle L_jL_{j-1}L_{j+1}}\leq \frac{\sin \frac{\pi}{3}}{\sin (\bar c/2+o_\rho(1))}\leq \frac{3}{\bar c}.
% \]
% Thus we get \[\frac{\bar c}{3} \leq \frac{|L_{j-1}L_j|}{|L_jL_{j+1}|}\leq \frac{3}{\bar c}\]
% for every $j\in \{2,3,4\}$.
%  Then the replacement polyline $L_1-L_2-L_3-L_4-L_5$ with polyline $L_1-L_2-L_4-L_5$ reduces the length by amount, linearly dependent on  $|L_1L_2|$:
%  \begin{multline*}
%  |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
%  > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
%  \frac{|L_3L_4|(1- \cos \frac{\bar{c}}{2})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{\bar{c}^4}{24(1+\frac{3}{\bar{c}})}|L_1L_2|.
% \end{multline*}
% Let $A'$ be a figure bounded by $[L_1,L_5]$, $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. The boundary of $A'$ is the union $[L_1L_5] \cup \breve{L_1C} \cup \breve{L_5C}$ where $C$ is a point of intersection $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. Note that $\dist(C,(L_1L_5))=o(|L_1L_5|)=o(|L_1L_2|)=o(\rho)$. Thus there exists a set $S=S_1\cup S_5$ such that $\H(S) = o(|L_1L_2|)$, $L_j\in S_j$ and $S_j$ is connected for $j\in \{1;5\}$. And we also will impose some condition on the energy of $S$. Let $L_j'$ be such point that $L_1'$,$C$ and $L_5'$ lie on the same line parallel to $(L_1L_5)$ and $(L_jL_j')\perp (L_1L_5)$ for $j\in \{1;5\}$. And let $C'$ be such point that $|CC'|=r$,$(CC')\perp (L_1L_5)$ and $[CC')\cap (L_1L_5)=\emptyset$. Now let $L_j''\defeq \partial B_r(C')\cap [L_i'C']$ for $i\in \{1;5\}$. Then $S\defeq [L_1L_1']\cup [L_1'L_1'']\cup [L_5L_5']\cup [L_5'L_5'']$. Thus $\H(S)=o(|L_1L_2|)=o(\rho)$. 
% It is easy to see that the connected set  
% \[
% S \cup [L_1L_2] \cup [L_2L_4]\cup [L_4L_5]
% \]
% for sufficiently small $\rho>0$ has strictly smaller length and not greater energy than $\Sigma$, so we get a contradiction with optimality of $\Sigma$.
% \end{proof}

% \item \label{plane:itema} \textit{Let $\bar x \in (\Sigma' \setminus \{x\}) \cap B_\varepsilon(x) \cap \E_\Sigma$ be a non-isolated energetic point.
% Then $\oord_{\bar x} \Sigma' = 2$, and every one-sided tangent $(\bar a\bar x]$ of $\Sigma'$ at $\bar x$ is $o_{|\bar xx|}(1)$-parallel to $(ax)$.}

% One can find sequences $x_k \rightarrow \bar x$ and $y(x_k)$ satisfying conditions of item~\ref{alm-orth:item1} of Proposition~\ref{prop:alm-orth}; let $(\bar a\bar x]$ be the one-sided tangent to the closed connected component containing $x_k$, and let $y(x_k) \rightarrow y(\bar x)$.
% Then $\vv{\bar xy(\bar x)}$ is orthogonal to $\vv{\bar a\bar x}$.
% On the other hand, due to item~\ref{alm-orth:item2} of Proposition~\ref{prop:alm-orth}, $\vv{\bar xy(\bar x)}$ is $o_{|\bar xx|}(1)$-orthogonal to $\vv{ax}$.
% It follows that $(\bar a\bar x)$ is $o_{|\bar xx|}(1)$-parallel to $(ax)$.

% Recall that, due to Lemma~\ref{napr}, $\vv{s}(\bar x) \in N(\bar x)$.
% Then, in view of item~\ref{alm-orth:item2} of Proposition~\ref{prop:alm-orth} and the definition of $N(\bar x)$, vector $\vv{s(\bar x)}$ is either of zero length or is $o_{|\bar xx|}(1)$-orthogonal to $\vv{ax}$.
% Then $\oord_{\bar x} \Sigma' > 1$, so $\oord_{\bar x} \Sigma' = 2$ (it cannot be equal to $3$ since a branching point is always non-energetic in $\mathbb{R}^2$).

% Finally, the second one-sided tangent $(\bar b\bar x]$ is also $o_{|\bar xx|}(1)$-parallel to $(ax)$ because $\vv{s(\bar x)} = \frac{\vv{\bar a\bar x}}{|\bar a\bar x|} + \frac{\vv{\bar b\bar x}}{|\bar b\bar x|}$ is either zero or $o_{|\bar xx|}(1)$-orthogonal to $\vv{ax}$.

% Note that there exists $\bar{y}=y(\bar x)$ is such that $(\bar y\bar x)$ are perpendicular to $(\bar a\bar x)$ or $(\bar b\bar x)$. On the other hand $\bar y\bar x$ should be almost perpendicular to $(ax)$.

%Assume the contrary.
%Then there exists $x_k\in E_\Sigma$ converging to $x$ with 

% First, let us show that the last condition follows from the first two.
% Note that $t_i$ is non-energetic for $i > 1$, otherwise, if $y(t_i)$ is its energetic point, in view of~\ref{plane:itemb}, we would have $\angle( \vv{t_it_{i - 1}}, \vv{t_iy(t_i)} ) \leq \pi / 3 + o_\varepsilon(1)$.
% Then, if $\varepsilon$ is small enough, $[t_{i - 1}t_i] \subset \Sigma$ intersects $B_r(y(t_i))$, which contradicts the definition of an energetic point.
% So $t_i$ is non-energetic for $i > 1$, then, due to Remark~\ref{rem:non-energ}, $\oord_{t_i} \Sigma \neq 1$.
% On the other hand, $\oord_{t_i} \Sigma \neq 2$, since $t_i$ cannot be a non-energetic point of order 2.

% Next we describe the construction of the sequence $t_i$.

%Assume the contrary. Let $\bar x \in E_\Sigma \cap \Sigma_i$ for any $i$. Then let us consider a path $p$ from a terminal point $T \in \Sigma_i \setminus b_i$ to $\bar x$. Without loss of generality let $\bar x$ be the first point of $E_\Sigma$ at this path. Then for every $\rho>0$ the path $p$ outside $B_\rho(x)$ is a finite union of segments. Clearly all segments has an angle greater then $\pi/7$ with $(ax)$ and hence an angle greater then $\pi/8$ with $(\bar a \bar x)$ where $(\bar a \bar x)$ is a tangent ray of $\Sigma$ at $\bar x$. Here we have a contradiction with a length of the minimizer in a small ball around $\bar x$.
%\textcolor{red}{надо ввести определение и в ремарке про него писать а не про шт дерево: for every point $S$ is a locally minimal tree for a finite set $A \subset S$ if $S$ is connected and for every $x\in S\setminus A$ there exists such $\varepsilon>0$ that $S \cap B_\varepsilon(x)$ is a regular tripod or a segment with center at $x$.}

%\textbf{Step 2}
% Thus for every $b_i$ one of its one-sided tangents is almost perpendicular to $(ax]$.
% \begin{proof}
% sum of $s()$ %belonging to a cone with a bisector 
% \end{proof}

% \item \label{plane:itemd} \textit{There exists $\rho = \rho(x) > 0$ such that for any $(\Sigma, x)$-nice $0 < \varepsilon < \rho$ the point $x$ is the only non-isolated energetic point on the path $\Sigma(x'_\varepsilon, x)$: $\Sigma(x'_\varepsilon, x) \cap \E_\Sigma = \{x\}$.}

% Let $\varepsilon$ be $(\Sigma, x)$-nice and satisfy $\varepsilon < \rho$, where $\rho$ is from~\ref{plane:branch-seg}.
% Assume that the claim is false, then there exists a point $\bar x \in \Sigma(x'_\varepsilon, x) \cap \E_\Sigma$, $\bar x \neq x$.
% Recall that $\Sigma(x'_\varepsilon, x)$ contains an infinite sequence of branching points converging to $x$; let us consider a path $\Sigma(b, \bar x)$ from one of these branching points to $\bar x$.
% Without loss of generality, we can assume that $\bar x$ is the only non-isolated energetic point on this path.
% Let $(\bar a \bar x]$ be the one-sided tangent of $\Sigma$ at $\bar x$ tangent to a connected component containing the path $\Sigma(b, \bar x)$.
% The path $\Sigma(b, \bar x)$ is a union of a (possibly, infinite) set of segments.
% Due to~\ref{plane:branch-seg}, all these segments have an angle with $(ax)$ greater then $\pi / 7$,
% % \alextodo{хочется задавать последовательность $b_j$ так, чтобы все точки ветвления на пути лежали в ней; ещё тут, видимо, надо ссылаться на Prop.~\ref{brrrr}?}\yanatodo{не очень поняла но вдруг там другие точки сгущения точек ветвления еще есть, тогда все не получится}
% and hence, due to Lemma~\ref{lm:ord2parallel}, an angle greater then $\pi / 8$ with $(\bar a \bar x)$, if $\varepsilon$ is small enough.
% This contradicts either Lemma~\ref{lm:seqseg} (if the set of segments is infinite), or the definition of a one-sided tangent (if it is finite).
% \item \textit{Proposition~\ref{brrrr} implies that every one-sided tangents to inner points of the path  in $\Sigma'$ from $\partial B_\varepsilon(x)$ to $x$ have an angle with $(ax]$ greater than $\pi/7$. The contradiction with a length of the closed connected component in a small ball around $x$.}

% \begin{lemma}
% Let $x \in \E_\Sigma$ and let there exist such a  cusp $Q\in \mathbb{Q}^{a,x}_\varepsilon$ that $Q^{a,x}_\varepsilon \cap \Sigma$ is an arc. Then for each $c>0$ there exists such $\varepsilon=\varepsilon(c)>0$ that every one-sided tangent at the points of set $Q^{a,x}_\varepsilon \cap B_{\varepsilon(c)}(x) \cap \Sigma$ has an angle not greater than $2c$ with a line $(ax)$.
% \label{zapred2}
% \end{lemma}
% \begin{proof}
% Assume the contrary, id est there exists a sequence of points with one-sided tangents having an angle with $(ax)$ greater than $2c$, converging to $x$. Without loss of generality assume $c<\pi/2$. By the step (a) of the proof Theorem~\ref{thm:plane} for sufficiently small $\varepsilon$ this sequence consists only on the points of $X_\Sigma \sqcup S_\Sigma$. As there is no branching points, the direction of tangents doesn't change at points of $S_\Sigma$, that is there is a sequence of points from $ X_\Sigma $ converging to $ x $ such that at least one of the two segments incident to the point has an angle with $ (ax) $ greater than $ 2c $. Let $L_1$ be such a point and let $\varepsilon$ be chosen not greater than $\rho$ for $c/5$ in Lemma~\ref{alm}. By item~\ref{__2} of Lemma~\ref{alm} both segments incident to $L_1$ has an angle with $(ax)$ greater than $9/5c$. Then the segment lying on the path from $L_1$ to $x$ should end with point $L_2\in X_\Sigma $. But the segment leaving $ L_2 $ must have an angle with $ (ax) $ greater than $ 8/5c $ and end with point $ L_3 \in X_\Sigma $. Thus for any arbitrarily small $ \bar \varepsilon$ there exists a broken line $ L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar \varepsilon} (x) $ such that all angles $ \angle ((L_jL_{j + 1}), (ax))> c $ for $j = 1,2,3,4 $. This is a contradiction with Proposition~\ref{brrrr}.
% \end{proof}

% Suppose the opposite:
% \[
% k \defeq \oordball_x \Gamma  < n \defeq \oord_x \Gamma. 
% \]
% By the definition of $\oord$, there exists $\rho > 0$ such that for any open set $U \ni x$ with $\diam U < \rho$ the inequality
% \[
% \sharp (\Gamma \cap \partial U) \geq n
% \]
% holds.
% Thus for each $\varepsilon < \frac{\rho}{2}$ we have
% \[
%  \sharp (\Gamma \cap \partial B_{\varepsilon}(x)) \geq n.
% \]
% On the other hand, in view of the definition of $\oordball$, there exists such $\delta < \frac{\rho}{2}$ that 
% \[
%  \sharp (\Gamma \cap \partial B_{\rho}(x)) = k < n.
% \]
% We got a contradiction.

% The symbol $\widehat{~~}$, unless otherwise stated, denotes the order sensitive angle belonging to $(-\pi, \pi]$ for rays and points, and to $[-\pi/2, \pi/2]$ for lines, where the counterclockwise direction is positive.
%order insensitive
%НАДО ОПРЕДЕЛИТЬ УГОЛ МЕЖДУ ЛУЧОМ/прямой и нормалью
% For a hyper-plane these symbols mean $\pi/2$ minus an angle with a line containing a normal to the hyper-plane.% (the normal can be a ray or containing its a line).

%The angle between the rays, unless otherwise stated, will be assumed to be positive and not exceeding $ \pi $, which uniquely determines its value.  %The angle between three points, unless otherwise stated, belongs to $(-\pi,\pi]$. 
%следить по тексту

% Then $[BC]$, $]BC]$ and $]BC[$ denote closed, semi-closed and open interval, accordingly, $[BC)$ and $(BC)$ represent the ray starting at $B$ and containing $C$, and the line containing these points, accordingly.

% \item Throughout the paper, unless stated otherwise, $\Sigma$ denotes a minimizer for a compact set $M \subset \mathbb{R}^n$ and a fixed constant $r > 0$.
% \yanatodo{мне кажется лучше написать $\Sigma(M,r)$ и добавить что будем писат $\Sigma$ там где понятно какие (M,r)}
% \alextodo{я в итоге решил во всех утверждениях писать явно, что такое $\Sigma$; есть ещё такой момент: кажется, часто надо требовать, чтобы $r$ было достаточно мало}
% \yanatodo{точно мало? как-то подозрительно( можно требовать невырожденности решения разве что: чтобы длина минимайзера была не 0, но и то если иначе никак. Вообще вроде мы гордимся тем что M и r любые( }
% \alextodo{я про невырожденность, да, типа $\diam M > 2r$ наверное достаточно везде должно быть}

% Sometimes, instead of $ \angle x_kxa \rightarrow 0 $, it will be more convenient for us to write $ (x_k x] \rightarrow (a x] $.

% \begin{definition}
% We will say that the line $ (ax) $ is the \textit{tangent line} of the set $ \Gamma \subset \mathbb{R}^n $  at the point $ x\in \Gamma $ if any sequence of points $ x_k \in \Gamma \setminus \{x\} $ such that $ x_k \rightarrow x $ satisfies $\angle ((x_kx),(ax)) \rightarrow 0$. 
% \end{definition}

% \begin{definition}
% We say that a ray $ (ax] $ is the \textit{energetic ray} of the set $ \Sigma $ with a vertex at the point $ x\in \Sigma $ if there exists a non-stabilized sequence of energetic points $ x_k \in \G_\Sigma $ such that $ x_k \rightarrow x $ and $ \angle x_kxa \rightarrow 0 $.
% \textcolor{green}{убери, если не нужно}
% \end{definition}


%\begin{remark}
%A point $x \in \Sigma$ belongs to the set of non-isolated energetic points $\E_\Sigma$ iff there exists an energetic ray with vertex at $x$.
%\end{remark}

% and there has to exist a regular tripod with center in a branching point, tangent to the minimizer).

% Note that an energetic point cannot be a branching point in $\mathbb{R}^2$, but it is possible in $R^n$ when $n > 2$.

%that have this property. \textcolor{red}{ой а там ведь еще не отрезки могут быть} 
%So  for each non-energetic point $x$ there exists such $\rho_1>0$ that $\overline{B_\rho(x) \cap \Sigma}$ is a Steiner tree.

% \begin{remark}
% Let $\Gamma \subset \mathbb{R}^n$ be a closed connected set of a finite length.
% If there exists a tangent line of $\Gamma$ at the point $x \in \Gamma$, then there also exists a one-sided tangent of $\Gamma$ at $x$, but not vice versa.
% \end{remark}

% \begin{definition}
% We will write $f(\rho)=o_\rho(1)$ if and only if $f(\rho)\rightarrow 0$ as $\rho \rightarrow 0$. \textcolor{blue}{мб перенести в начало главы или туда, где в первый раз используется}
% \end{definition}

% \begin{definition}
% We will say that a closed simply connected set $Q \subset \mathbb{R}^n$ is a cusp with the axis $(ax]$ if $(ax] \subset Q$ and for any $\varepsilon > 0$, denoting $Q_{\leq \varepsilon} \defeq Q \cap \overline{B_\varepsilon(x)}$ and $Q_\varepsilon \defeq Q \cap \partial B_\varepsilon(x)$,
% conditions $Q_{\leq \varepsilon} \subset \conv (\{x\}, Q_\varepsilon)$ and $\diam Q_\varepsilon = o(\varepsilon)$ hold.
% \end{definition}

% \begin{definition}
% For a given ray $(ax]$ and $\rho>0$ we will denote by a set of \textit{cusps}  $\mathbb{Q}_{\rho}^{a,x}$ the set consisting of all closed simply connected sets $Q$ with the following properties: 
% \begin{itemize}
%     \item $Q \subset \overline{B_{\rho}(x)}$;
%      \item for any $0<\rho'\leq \rho$ and any $2$-dimensional plane $\alpha \ni x$ the set $Q \cap \partial B_{\rho'}(x)\cap \alpha$ is connected; %an arc, i.e. an injective image of the segment %(actually it is sufficient to state this property only for $\rho'=\rho$), a point or an emptyset;
%     \item for any $z\in \partial Q \setminus \partial B_\rho(x)$ the following statement holds: $[xz] \cap Q=\{x\} \cup \{z\}$;
%     \item the intersection $(ax] \cap \overline{B_{\rho}(x)} \subset Q$ is a segment;
%     \item an arbitrary sequence of points $z_k \in Q$ converging to $x$ satisfies $\angle z_k x a \rightarrow 0$.
% \end{itemize}
% The ray $(ax]$ will be called the \textit{axis of the cusp $Q$}.
% \end{definition}


% \begin{lemma} Let the set $\Gamma \subset \mathbb{R}^n$ have a tangent line $(ax)$ at the point $x \in \Gamma$ with the property that any sequence of points $ x_k \in \Gamma \setminus \{x\}$ such that  $ x_k \rightarrow x $ satisfies $(x_kx] \rightarrow (ax]$. %such that $ x_k \rightarrow x $ satisfies $ \angle x_kxa \rightarrow 0 $ \textcolor{red}{кажется, это свойство это просто определение tangent line}. 
% Then there exists a cusp $Q$ with the axis $(ax]$ and $\rho > 0$ such that for every $0 < \varepsilon < \rho$ the inclusion $(\Gamma \cap \overline{B_\varepsilon(x)}) \subset (\Int Q \cup \{x\})$ holds.
% \alextodo{а нам важно, что $\Gamma$ на границу $Q$ не выходит? если нет, то я бы справа просто $Q$ написал}
% %\label{kas} 
% \label{con}
% \end{lemma}
% \begin{proof}
% There exists a strictly decreasing sequence $\varepsilon_k \rightarrow 0$ and a non-strictly decreasing sequence $\gamma_k \rightarrow 0$ such that any $z \in \Gamma \cap B_{\varepsilon_k}(x)$ satisfies $\angle zxa < \gamma_k$.
% Denote 
% \[
% Q(\varepsilon, \gamma) \defeq \{z \in \mathbb{R}^n \ \big | \ |zx| \leq \varepsilon,\ \angle zxa \leq \gamma\},
% \]
% and let $\gamma_0 = \gamma_1$, $\varepsilon_0 = \infty$.
% Then the set
% \[
% Q \defeq \bigcup_{k=0}^{\infty} \left(Q(\varepsilon_k,\gamma_k) \setminus B_{\varepsilon_{k+1}}(x) \right)
% \]
% is a cusp with the axis $(ax]$ and has the desired properties.
% \end{proof}

%\begin{remark}
%As far as all arguments are local all statements of this work are true not only for maximal distance minimizers but also for local minimizers. 
%\label{lcl}
%\end{remark}


% It is known (see~\cite{kuratowski2014topology}) that, as $\Sigma$ has a finite length, the following lemma holds:

% \begin{lemma}\label{ord_arcs}
% Let $\Sigma$ be a minimizer for a compact set $M \subset \mathbb{R}^n$ and $r > 0$, and let $ x \in \Sigma $ be a point of order $ n $: $\oord_x \Sigma = n$.
% Then there exists $\rho = \rho(x) > 0$ such that for any $0 < \varepsilon < \rho$ the set $\Sigma \cap B_\varepsilon (x)$ contains $n$ arcs with one end at $\partial B_\varepsilon(x)$ and another end at $x$ with pairwise intersections only at point $x$.
% \end{lemma}
% \jiocbtodo{надо как-то выделить, что пересечение попарное, а не общее}

% In this work we prove that in planar case the set $\Sigma \cap B_\varepsilon (x)$ coincides with these arcs.

% %\subsection{The main theorem}

% \begin{theorem}\label{mainT1}
% Let $\Sigma$ be a minimizer for a compact set $M \subset \mathbb{R}^n$ and $r > 0$.
% %and in each vertex at most $3$ arcs are incident.
% %И В КАЖДОЙ ТОЧКЕ НЕ БОЛЬШЕ ТРЕХ КАС ЛУЧЕЙ  И УГОЛ ОК
% Then there are at most three tangent rays at any point of $\Sigma$ and the pairwise angles between the tangent rays are at least $2\pi / 3$.
% Moreover, if $n = 2$, then $\Sigma$ is a union of a finite number of arcs with continuous one-sided tangents.
% \end{theorem}
% \begin{proof}
% See Corollary~\ref{cor:struct}, Theorem~\ref{thm:plane} and Lemma~\ref{zapred2}.% and Corollary~\ref{main}.
% \end{proof}

% \begin{definition}
% Let $M \subset \mathbb{R}^n$ be a compact set and let $r > 0$.
% A connected set $\Sigma \subset \mathbb{R}^n$ is called a local minimizer if $M \subset \overline{B_r(\Sigma)}$ and there exists $\varepsilon > 0$ such that for any connected set $\Sigma'$ satisfying $M \subset \overline{B_r(\Sigma')}$ and $\diam (\Sigma \triangle \Sigma') \leq \varepsilon$ the inequality $\H(\Sigma) \leq \H(\Sigma')$ holds, where $\triangle$ is the symmetric difference.
% \end{definition}

% Our proof does not use global arguments, so the following statement is also true.
% \alextodo{мб везде рассуждать про local minimizer, а основную теорему сделать следствием}

% \begin{theorem}
% Let $\Sigma \subset \mathbb{R}^n$ be a local minimizer for a compact set $M \subset \mathbb{R}^n$ and $r > 0$. Then $\Sigma$ has the same properties as in Theorem~\ref{mainT1}.
% \end{theorem}

% \alextodo{предлагаю всё с начала секции до этого момента перенести во введение}

% We now turn to the statements used in the proof of the theorem.

%\subsection{Lemmas}

% \begin{lemma}
% Let $r > 0$. For $m \leq n$, a sufficiently small $\delta > 0$, and the $m$-dimensional cube $I^m = [-\delta; \delta]^m \times \{0\}^{n - m}$ there exists a connected set $S \subset \mathbb{R}^n$ containing the origin point such that $\overline{B_{r}(I^m)} \subset \overline {B_r(S)}$ and $\H(S) = c\delta + o(\delta)$, where $c$ depends only on $n$ and $m$.
% \label{cube}
% \end{lemma}

% \begin{proof}
% Define $S$ as the union of $2^n$ segments connecting the origin point with each point from the set $V \defeq \{\pm(\delta + c'\delta^2)\}^m \times \{\pm c'\delta^2\}^{n - m}$, where $c' \defeq \frac{n\sqrt{n}}{r}$.
% Clearly, $S$ is connected, it contains the origin point and $\H(S) = c\delta + o(\delta)$, where $c = 2^n \sqrt{m}$.

% Let $y \in \overline{B_{r}(I^m)}$ and let $z$ be the closest to $y$ point of $I^m$. Due to symmetry, we can assume that $y_i \geq z_i \geq 0$ for each $i$. Let the index $i$ belong to the set $J$ if $y_i - z_i \leq c'\delta^2$, and to the set $K$ if $y_i - z_i > c'\delta^2$. Denoting $|yz| = l \leq r$, we have
% \begin{equation}
%     l^2 = \sum_{i=1}^n(y_i-z_i)^2=\sum_{i\in K}(y_i-z_i)^2+o(\delta^2).
%     \label{2z}
% \end{equation}

% Define $\hat{z}_i \defeq \delta + c'\delta^2$ for $i \leq m$, and $\hat{z}_i \defeq c'\delta^2$ for $i > m$. By definition, $\hat{z} \in V \subset S$. Note that $|\hat{z}_i - y_i| \leq \delta + c'\delta^2$ for $i \in J$, and $\hat{z}_i - z_i = c'\delta^2$ for $i \in K$. It follows that
% \[
%  \sum_{i=1}^n (y_i-\hat{z_i})^2 \leq |J|\delta^2 + o(\delta^2) + \sum_{i\in K} (y_i-z_i-c'\delta^2)^2 = |J|\delta^2+l^2+o(\delta^2)-2c'\delta^2\sum_{i\in K}(y_i-z_i).
% \]
% The last equality follows from~\eqref{2z}. Equality~\eqref{2z} also implies that there exists $i \in K$ such that $(y_i - z_i)^2 \geq \frac{l^2}{n}+o(\delta^2)$, so $y_i-z_i \geq \frac{l}{\sqrt{n}}+o(\delta^2)$. %(\textcolor{red}{добавила в каком-то виде $o(\delta^2)$}).
% Then
% \[
% \sum_{i=1}^n (y_i-\hat{z_i})^2\leq l^2+\delta^2\left(|J|-2c' \frac{l}{\sqrt{n}}\right)+o(\delta^2) \leq l^2 + \frac{r - 2l}{r} \delta^2 n + o(\delta^2).
% \]
% If $l > r / 2$, then
% \[
% l^2 + \frac{r - 2l}{r} \delta^2 n + o(\delta^2) \leq l^2 \leq r^2.
% \]
% Otherwise, assuming $\delta < \frac{r}{2\sqrt{n}}$, we have
% \[
% l^2 + \frac{r - 2l}{r} \delta^2 n + o(\delta^2) \leq \frac{r^2}{4} + \frac{r^2}{4} + o(\delta^2) \leq r^2.
% \]
% Either way, $y\in \overline{B_r(S)}$, and the statement is proved.
% \end{proof}

% \begin{corollary}
% There exists $c = c(n) > 0$ such that for any sufficiently small $\varepsilon > 0$ and any $x \in \mathbb{R}^n$ there exists a connected set $S(x, \varepsilon) \ni x$ satisfying $\H( S(x, \varepsilon) )=c\varepsilon + o(\varepsilon)$ and
% \[
% \F_M(\Sigma \setminus B_\varepsilon(x)\cup S(x, \varepsilon) )\leq \F_M(\Sigma).
% \]
% \label{ball}
% \end{corollary}
% % \begin{proof}
% % Just let $S$ be as in Lemma~\ref{cube} for the $n$-dimensional cube with the center at $x$ and sides of length $2\delta$.
% % \end{proof}


% %\begin{corollary}
% %Let $r>0$ and let $x \in \mathbb{R}^n$. Then for sufficiently small $\delta>0$ There exists such sets $S_0$, $S_1$,\ldots $S_{2^n}$ that $\overline{B_{r+\delta}(x)} \subset \overline {B_r(\bigcup_{i=1}^{2^n} S_i)}$ and
% %\begin{itemize}
% %\item $S_i$ is connected for every $i\in 0,1,\ldots 2^n$, set $\bigcup_{i=0}^{2^n} S_i$ is also connected;
% %\item $\partial B_{\delta}(x) \cap S_i \neq \emptyset$ for every $i=1,2 \ldots 2^n$;
% %\item $\H(\bigcup_{i=1}^{2^n} S_i)=o(\delta)$, $\H(S_0)=c(n)\delta$, where $c(n)\leq % 2^{m}\sqrt{m}$, and $S_0 \ni x$.
% %\end{itemize}
% %Let us define $S^{x,\delta}\defeq \bigcup_{i=0}^{2^n} S_i$. $\H(S^{x,\delta})\leq 2^{m}\sqrt{m}+o(\delta)$.
% %\label{ball}
% %\end{corollary}

% \begin{remark}
% Let $r > 0$. There exists $\delta = o(\varepsilon)$ such that for any segment $[uv] \subset \mathbb{R}^n$ of length $\varepsilon > 0$ one has $\overline {B_r([uv])} \subset \overline{B_{r + \delta}(u)} \cup \overline{B_{r + \delta}(v)}$.
% \label{twocubes}
% \end{remark}
% \begin{proof}
% Consider an arbitrary point $z \in \overline{B_r([uv])}$ and let $a \defeq \dist(z, (uv)) \leq r$. Then
% \[
% \dist(z, \{u, v\}) \leq \sqrt{ a^2 + \max \left( r^2 - a^2, \left( \frac\varepsilon 2 \right)^2 \right) } \leq \sqrt{ r^2 + \frac{\varepsilon^2}{4} }.
% \]
% Thus there exists $\delta = o(\varepsilon)$ such that
% \[
% \dist \left( \overline{B_r([uv])}, \{u, v\} \right) \leq \sqrt{ r^2 + \frac{\varepsilon^2}{4} } \leq r + \delta.
% \]
% \end{proof}

% \begin{lemma}
% \label{cuspfortangent}
% Let $r > 0$, let $\Gamma \subset \mathbb{R}^n$ be a closed connected set of a finite length, and let $x \in \Gamma$.
% Let every connected component of $\Gamma \setminus \{x\}$ have the same one-sided tangent $(ax]$ at $x$, i.e. for any sequence of points $x_k \in \Gamma \setminus \{x\}$ if $x_k \rightarrow x$, then $(x_kx] \rightarrow (ax]$.
% Then for any $(\Gamma, x)$-nice $\varepsilon > 0$ there exist connected sets $T^x \ni x$ and $T^\partial \supset (\Gamma \cap \partial B_\varepsilon(x)) \cup ((ax] \cap \partial B_\varepsilon(x))$ satisfying
% \[
% \H(T^x \cup T^\partial) = o(\varepsilon) \quad\text{and}\quad \overline{B_r(\Gamma \cap B_\varepsilon(x))} \subset \overline{B_r(T^x \cup T^\partial)}.
% \]
% \end{lemma}
% \begin{proof}
% There exists $\gamma = o(\varepsilon)$ such that for any point $z \in (\Gamma \setminus \{x\}) \cap B_\varepsilon(x)$ the inequality $\angle zxa \leq \gamma$ holds.
% Let
% \[
% Q \defeq \{z \in \partial B_\varepsilon(x) \ \big | \ \angle zxa \leq \gamma \},\quad \xi \defeq \diam Q,
% \]
% and note that $\xi = o(\varepsilon)$ and $( \Gamma \cap B_\varepsilon(x) ) \subset \conv(\{x\} \cup Q)$.
% Let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$ and let $\St(P)$ be a Steiner tree on the set $P \defeq \{\bar x\} \cup ( \Gamma \cap \partial B_\varepsilon(x) )$.
% Note that $\sharp P = \oordball_x \Gamma + 1$ and $P \subset Q$, so $\H(\St(P)) \leq \sharp P \cdot \xi = o(\varepsilon)$.

% The claim follows from Lemma~\ref{cube} by taking $T^x \defeq S(x, \delta)$ and $T^\partial \defeq S(\bar x, \xi + \delta) \cup \St(P)$, where $\delta = o(\varepsilon)$ is from Remark~\ref{twocubes}. Indeed,
% \[
% ( \Gamma \cap B_\varepsilon(x) ) \subset \conv(\{x\}, Q) = \bigcup_{z \in Q} [xz],
% \]
% so
% \[
% \overline{B_r(\Gamma \cap B_\varepsilon(x))} \subset \bigcup_{z \in Q} \overline{B_r([xz])} \subset (\overline{B_{r + \delta}(x)} \cup \overline{B_{r + \xi + \delta}(\bar x)}) \subset \overline{B_r(T^x \cup T^\partial)},
% \]
% where the second inclusion is by Remark~\ref{twocubes}, and the last inclusion is by Lemma~\ref{cube}.
% \end{proof}
% %\input{pictures/Suv}

% % \begin{lemma}
% % Let $r > 0$. Let $\Gamma \subset \mathbb{R}^n$ be a closed connected set of a finite length, and let $(ax]$ be a one-sided tangent to $\Gamma$ at $x$.
% % Let $Q$ be a cusp with the axis $(ax]$ satisfying $(\Gamma \cap \overline{B_\varepsilon(x)}) \subset (\Int Q \cup \{x\})$ for any sufficiently small $\varepsilon > 0$.
% % Then for any sufficiently small $\oordball_x \Gamma$-nice $\varepsilon > 0$ there exist connected sets $T^x \ni x$ and $T^Q \supset \Gamma \cap Q_\varepsilon$ such that $\H(T^x \cup T^Q) = o(\varepsilon)$ and $\overline{B_r(\Gamma \cap \overline{B_\varepsilon(x)})} \subset \overline{B_r(Q_{\leq \varepsilon})} \subset \overline{B_r(T^x \cup T^Q)}$.
% % \label{cuspfortangent}
% % \end{lemma}
% % \begin{proof}
% % Let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$ and let $\St(P)$ be a Steiner tree on the set $P \defeq \{\bar x\} \cup ( \Gamma \cap Q_\varepsilon )$.
% % Note that $\sharp P \leq \oordball_x \Gamma + 1$ and $P \subset Q_\varepsilon$.
% % Let $\xi \defeq \diam Q_\varepsilon$.
% % By the definition of a cusp, $\xi = o(\varepsilon)$ and $\H(P) = o(\varepsilon)$.

% % The claim follows from Lemma~\ref{cube} by taking $T^x \defeq S(x, \delta)$ and $T^Q\defeq S(\bar x, \xi + \delta) \cup \St(P)$, where $\delta = o(\varepsilon)$ is from Remark~\ref{twocubes}. Indeed,
% % \[
% % Q_{\leq \varepsilon} \subset \conv(\{x\}, Q_\varepsilon) = \bigcup_{z \in Q_\varepsilon} [xz],
% % \]
% % so
% % \[
% % \overline{B_r(Q_{\leq \varepsilon})} \subset \bigcup_{z \in Q_\varepsilon} \overline{B_r([xz])} \subset (\overline{B_{r + \delta}(x)} \cup \overline{B_{r + \xi + \delta}(\bar x)}) \subset \overline{B_r(T^x \cup T^Q)},
% % \]
% % where the second inclusion is by Remark~\ref{twocubes}, and the last inclusion is by Lemma~\ref{cube}.
% % \end{proof}

% \begin{corollary}
% \label{cor:tang-comp}
% Let $\Sigma$ be a minimizer for a compact set $M \subset \mathbb{R}^n$ and $r > 0$, and let $x \in \Sigma$.
% \begin{enumerate} 
% \item \label{tang-comp:comp}
% For every one-sided tangent $(ax]$ of $\Sigma$ at $x$ there exists exactly one connected component $\Sigma_1$ of $\Sigma \setminus \{x\}$ to which $(ax]$ is tangent.
% Moreover, $\oordball_x \Sigma_1 = 1$, and for any $(\Sigma_1, x)$-nice $\varepsilon > 0$ the equality $\H(\Sigma_1 \cap \overline{B_\varepsilon(x)}) = \varepsilon + o(\varepsilon)$ holds.
% \item \label{tang-comp:ang} The angle between any two one-sided tangents of $\Sigma$ at $x$ is at least $2\pi/3$.
% In particular, there are at most three one-sided tangents at any point of $\Sigma$.
% \end{enumerate}
% \end{corollary}
% \begin{proof}\leavevmode
% \begin{enumerate}
% \item Let $W$ be the closure of the union of all connected components of $\Sigma \setminus \{x\}$ to which $(ax]$ is tangent.
% Let $\varepsilon > 0$ be $(W, x)$-nice, let $T^x$ and $T^\partial$ be the sets from Lemma~\ref{cuspfortangent} applied to $\Gamma = W$ and let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$.
% Then the set 
% \[
% \Sigma \setminus (W \cap \overline{B_\varepsilon(x)}) \cup T^x \cup T^\partial \cup [x\bar x]
% \]
% is connected and has the energy not larger than $\Sigma$. Then it cannot be shorter than $\Sigma$, so $\H(W \cap \overline{B_\varepsilon(x)}) \leq \varepsilon + o(\varepsilon)$.
% In view of Remark~\ref{ord_pos} and Remark~\ref{geq_ord}, equalities $\H(W \cap \overline{B_\varepsilon(x)}) = \varepsilon + o(\varepsilon)$ and $\oordball_x W = 1$ hold.
% The claim of the item follows immediately.

% \item Let one-sided tangents $(a_1x]$ and $(a_2x]$ of $\Sigma$ at $x$ be such that $\angle ((a_1x], (a_2x]) < 2 \pi / 3$.
% Denote by $\Sigma_1$ and $\Sigma_2$ the closures of connected components of $\Sigma \setminus \{x\}$ which have one-sided tangents $(a_1x]$ and $(a_2x]$, respectively.
% Let $\varepsilon > 0$ be $(\Sigma, x)$-nice.
% \alextodo{здесь враньё из-за того, что $(\Sigma,x)$-nice не обязан быть $(\Sigma_1,x)$-nice}
% Denote $\bar x_1 \defeq (a_1x] \cap \partial B_\varepsilon(x)$ and $\bar x_2 \defeq (a_2x] \cap  \partial B_\varepsilon(x)$. Let $T^x_1 = T^x_2 = T^x$, $T^\partial_1$ and $T^\partial_2$ be the sets from Lemma~\ref{cuspfortangent} applied to $\Gamma = \Sigma_1$ and to $\Gamma = \Sigma_2$, and let $\St(\bar x_1, \bar x_2, x)$ be a Steiner tree on the set $\{\bar x_1, \bar x_2, x\}$. Then the set
% \[
% \Sigma \setminus ((\Sigma_1 \cup \Sigma_2) \cap \overline{B_\varepsilon(x)}) \cup T^\partial_1 \cup T^\partial_2 \cup T^x \cup \St(\bar x_1, \bar x_2, x)
% \]
% is connected and has the energy not larger than $\Sigma$. Additionally, by Proposition~\ref{angles4}, it is shorter that $\Sigma$. It is not possible, since $\Sigma$ is a minimizer, so our assumption is false.
% \end{enumerate}
% \end{proof}

% \begin{corollary}
% Let $(ax]$ be a one-sided tangent of $\Sigma$ at $x$.
% \begin{enumerate} 
% \item 
% Let $Q$ be a cusp with the axis $(ax]$ satisfying $(\Sigma \cap \overline{B_\varepsilon(x)}) \subset (\Int Q \cup \{x\})$ for any sufficiently small $\varepsilon > 0$.
% Then for any sufficiently small $\oordball_x \Sigma$-nice $\varepsilon > 0$ the inequalities $\H(\Sigma \cap Q_{\leq \varepsilon}) \leq \varepsilon + o(\varepsilon)$ and $\oordball_x( \Sigma \cap Q_{\leq \varepsilon} ) \leq 1$ hold.
% \label{len0-cusp}
% \item There exists exactly one closed connected component $\Sigma_1$ of $\Sigma \setminus \{x\}$ to which $(ax]$ is tangent.
% Moreover, $\oordball_x \Sigma_1 = 1$, and for any sufficiently small $\oordball_x \Sigma_1$-nice $\varepsilon > 0$ the equality $\H(\Sigma_1 \cap \overline{B_\varepsilon(x)}) = \varepsilon + o(\varepsilon)$ holds.
% \label{len0-comp}
% \end{enumerate}
% \label{len0}
% \end{corollary}
% \begin{proof}\leavevmode
% \begin{enumerate}
% \item Let $T^x$ and $T^Q$ be the sets from Lemma~\ref{cuspfortangent} and let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$. Then the set 
% \[
% \Sigma \setminus Q_{\leq \varepsilon} \cup T^Q \cup T^x \cup [x\bar x]
% \]
% is connected and has the energy not larger than $\Sigma$. Then it cannot be shorter than $\Sigma$, so $\H(\Sigma \cap Q_{\leq \varepsilon})\leq \varepsilon+o(\varepsilon)$.
% %The upper bound follows from the inequality $\oordball_x \Sigma > 0$.
% By Remark~\ref{geq_ord}, the inequality $\oordball_x (\Sigma \cap Q_{\leq \varepsilon}) \leq 1$ follows.

% \item
% Let $\Sigma_1$ be any closed connected component of $\Sigma \setminus \{x\}$ to which $(ax]$ is tangent.
% If there is another such component $\Sigma_2$, define $W \defeq \Sigma_1 \cup \Sigma_2$; otherwise, define $W \defeq \Sigma_1$.
% By Lemma~\ref{con}, there exists a cusp $Q$ with the axis $(ax]$ such that for any sufficiently small $\varepsilon > 0$ the inclusion $( W \cap \overline{B_\varepsilon(x)} ) \subset (\Int Q \cup \{x\})$ holds.
% It follows from item~\ref{len0-cusp} that $\H(W \cap Q_{\leq \varepsilon}) \leq \varepsilon + o(\varepsilon)$ and $\oordball_x(W \cap Q_{\leq \varepsilon}) \leq 1$.
% Then, in view of Remarks~\ref{ord_pos} and~\ref{geq_ord}, $\oordball_x(W \cap Q_{\leq \varepsilon}) = 1$ and $\H(W \cap Q_{\leq \varepsilon}) = \varepsilon + o(\varepsilon)$.

% We see that $\Sigma_2$ cannot exist, since otherwise we could use the same arguments for $\Sigma_1$ and $\Sigma_2$ separately and get $\H(\Sigma_1 \cap Q_{\leq \varepsilon}) = \H(\Sigma_2 \cap Q_{\leq \varepsilon}) = \H(W \cap Q_{\leq \varepsilon}) = \varepsilon + o(\varepsilon)$, which is not possible.
% \end{enumerate}
% \end{proof}

% \begin{lemma}
% If $\Sigma$ has two one-sided tangents at a point $x \in \Sigma$, then the angle between them is at least $2\pi/3$. %In particular they can not coincide.
% In particular, $\Sigma$ has at most three one-sided tangents at any point.
% \label{angles2}
% \end{lemma} 
% \begin{proof}
% Let one-sided tangents $(a_1x]$ and $(a_2x]$ be tangent to closed connected components $\Sigma_1$ and $\Sigma_2$ of $\Sigma \setminus \{x\}$, respectively. %By Lemma~\ref{con}, %что компонента связности $W_i$ содержится в псевдоконусе
% %(не умаляя общности $\varepsilon_0 \leq \varepsilon_1$),
% For $i \in \{1, 2\}$, let $Q_i$ be a cusp with the axis $(a_ix]$ from Lemma~\ref{con} applied to $\Gamma = \Sigma_i$.
% % Define the closures of intersections of connected components with $B_\varepsilon(x)$ by $W_1$ and $W_2$ \textcolor{red}{хочется это предложение заменить/дополнить формулами}.

% Let $\varepsilon > 0$ be sufficiently small and $\oordball_x \Sigma$-nice.
% Note that $(\Sigma_i \cap \overline{B_\varepsilon(x)}) \subset (\Int Q_i \cup \{x\})$ and $\H(\Sigma_i \cap \overline{B_\varepsilon(x)})\geq \varepsilon$ for $i \in \{1,2\}$.
% \alextodo{здесь и в предыдущем следствии мб есть враньё из-за того, что $\oordball_x \Sigma$-nice не обязан быть $\oordball_x \Sigma_1$-nice}

% Assume that $\angle ( (a_1x], (a_2x] ) < 2 \pi / 3 $. Denote $\bar x_1 \defeq (a_1x] \cap \partial B_\varepsilon(x)$ and $\bar x_2 \defeq (a_2x] \cap  \partial B_\varepsilon(x)$. Let $T^{Q_1}$, $T^{Q_2}$ and $T^x$ be the sets from Lemma~\ref{cuspfortangent}, and let $\St(\bar x_1, \bar x_2, x)$ be a Steiner tree on the set $\{\bar x_1, \bar x_2, x\}$. Then the set
% \[
% \Sigma \setminus ((\Sigma_1 \cup \Sigma_2) \cap \overline{B_\varepsilon(x)}) \cup T^{Q_1}\cup T^{Q_2}\cup T^x \cup \St(\bar x_1, \bar x_2, x)
% \]
% is connected and has the energy not larger than $\Sigma$. Additionally, by Proposition~\ref{angles4}, it is shorter that $\Sigma$. It is not possible, since $\Sigma$ is a minimizer, so our assumption is false.
% \end{proof}

%\begin{corollary}
%В условиях замечания~\ref{star} найдется $\varepsilon>0$ такое, что $B_\varepsilon(x) \cap \Sigma$ является дугой (либо лежащей в одном псевдоконусе, либо в объединении двух псевдоконусов с осями, образующими прямую).
%\end{corollary}
%Следующее утверждение показывает регулярность $\Sigma$ в окрестности любой точки из $x$ из $\Sigma \setminus \E_\Sigma$.

%\begin{proposition}
%For an arbitrary point $x\in \S_\Sigma \sqcup \X_\Sigma$ there exists such $\varepsilon=\varepsilon(x)>0$ that set $ \Sigma \cap B_\varepsilon (x) $ consists of $ \oord_x \Sigma $ line segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with pairwise angles between them at least $ 2 \pi / 3 $.% Moreover, in the case of $ x \in S_ \Sigma $, set $ \overline{B_\varepsilon (x)} \cap \Sigma $ is a segment or a regular tripod centered at $ x $, and in the case of $ x \in \X_\Sigma $ --- a segment with an end at $ x $ and another one at $\partial B_\varepsilon(x)$, or the union of two segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with angle at least $ 2 \pi / 3 $ between them.

%ВОЗМОЖНО НАДО УБРАТЬ
%\label{discr_str}
%\end{proposition}

%\begin{proof}
%It is easy to see that for each $x \in \Sigma$ inequality $\oordball_x \Sigma \leq 2^{m}\sqrt{m} $ holds. Assume the contrary, then for sufficiently small $\varepsilon>0$ the co-area inequality entails $\H(\Sigma \cap \overline{B_\varepsilon (x)}) \geq (2^{m}\sqrt{m} +1) \varepsilon$. But then set $\Sigma' \defeq \Sigma \setminus B_\varepsilon(x) \cup S^{x, \varepsilon}$ is better than $\Sigma$: it is connected, its energy is not greater and its length is strictly less than of $\Sigma$. This gives a contradiction with the optimality of $\Sigma$.

%Now let $x \in \S_\Sigma \sqcup \X_\Sigma$ and let $\varepsilon>0$ be such that $\Sigma \cap \overline{B_\varepsilon(x)} \setminus \{x\} \subset \S_\Sigma$. Thus, there exists an infinite monotonically decreasing sequence $\varepsilon_i \rightarrow 0$ such that $\sharp (\partial B_{\varepsilon_i}(x) \cap \Sigma) = \oordball_x \Sigma \leq 2^{m}\sqrt{m}$ for every $i$. Without loss of generality let $\varepsilon_1<\varepsilon$. For numbers $l>k$ let us define set
%\[
%\Sigma_{k,l} \defeq \Sigma \cap \overline{{B}_{\varepsilon_k}(x)} \setminus B_{\varepsilon_l}(x).
%\]
%Note that $\Sigma_{k,l} \subset \S_\Sigma$ is a full Steiner forest and all its terminal vertices belong to $\partial B_{\varepsilon_k}(x) \cup \partial B_{\varepsilon_l}(x)$. Since $\Sigma_{k,l}$ has not more vertices than $2^{m}\sqrt{m}-2$, the number of its branching points is at most $2^{m+1}\sqrt{m}-2$ for each $l>k$ and $\Sigma_{k,l}$ consists of a finite number of line segments, less than $2^{m+2}\sqrt{m}$. Then there exists such a number $m>k$ that set $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ does not contain a branching points or a maximal segment not containing point $x$. So the number of segments in $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ is at most the number of segments of every set $\Sigma_{m,n}$, $n>m$ (which is less than $2^{m+2}\sqrt{m}$); in particular it is finite.    

%In view of Lemma~\ref{angles2} and Remark~\ref{3vectors} set $\Sigma \cap B_{\varepsilon_m}(x)$ should be either a segment with one end at point $x$ and another at $\partial B_{\varepsilon_m}(x)$, or union of two such segments with the angle at least $2\pi/3$ between them, or the union of three such segments with angles $2\pi/3$ between them (i.e. regular tripod with the center at $x$, belonging to the same plane). 
%\end{proof}
%\textcolor{red}

%\begin{remark}
%It is easy to see that if $x\in \S_\Sigma$, then there exists such $\varepsilon>0$ that $\Sigma \cap B_\varepsilon(x)$ is a segment or a tripod with the vertices at $\partial B_\varepsilon(x)$ and the center at $x$. If $x \in \X_\Sigma$, then there exists such $\varepsilon>0$ that $\Sigma \cap B_\varepsilon(x)$ is a union of one, two or three segments with one end at $x$ and the other end at $\partial B_\varepsilon(x)$ with the pairwise angles at least $2\pi/3$. \textcolor{red}{во второй главе была очень похожая ремарка, мб стоит оставить тут только новую инфу}
%\end{remark}

% \begin{remark}
% For any $u\in U(x, \varepsilon)$ the inequality $|x u|\leq r+\varepsilon$ holds.
% \label{ddist}
% \end{remark}

% \begin{remark}
% Let $x \in \Sigma$ be an energetic point. If $y(x)\in M$ corresponds to $x$, then $y(x) \in \overline{U(x,\varepsilon)}$ for any $\varepsilon > 0$.
% \label{rem_c}
% \end{remark}

% \begin{remark}
% Obviously, $y(\bar{x}) \in \overline{U(\bar{x},\varepsilon)}$, where $y(\bar{x})\in M$ is an arbitrary point, corresponding to $\bar{x}$.
% \label{rem_c}
% \end{remark}

% \begin{remark}
% A point $x \in \Sigma$ is non-energetic if and only if there exists $\varepsilon>0$ such that $U(x,\varepsilon)=\emptyset$.
% \end{remark}

\begin{remark}\label{rem_cC}
There exists $\gamma = o_\varepsilon(1)$ such that for any $u\in U(x,\varepsilon)$ the inequality $\angle ux y(x) \leq \gamma$ is satisfied for some corresponding point $y(x)$.
Let $\bar x \in \Sigma$ be an energetic point. For any $u\in \overline{U(\bar{x},\varepsilon)}$ there exists such a corresponding point $y(\bar x)$ and $\gamma=o_\varepsilon(1)$ that $\angle u\bar x y(\bar x) \leq \gamma$. Due to compactness of the set of corresponding points, one can choose the same $\gamma(\bar x, \varepsilon)$ for all $y(\bar x)$. \textcolor{red}{тут непонятно, кто из $\bar x$, $\varepsilon$ фиксирован, а кто нет}
\end{remark}

% \begin{proof}
% Let $x = (x_1, \dots, x_n)$. For any $\varepsilon > 0$ let $I^n_\varepsilon$ be the $n$-dimensional cube with the center at $x$ and sides of length $2\varepsilon$, parallel to the coordinate axes:
% \[
% I^n_\varepsilon \defeq [x_1 - \varepsilon, x_1 + \varepsilon] \times \dots \times [x_n - \varepsilon, x_n + \varepsilon].
% \]
% Let $V(\varepsilon)$ be the set of $2^n$ vertices of $I^n_\varepsilon$. Let $c' \defeq \frac{n\sqrt{n}}{r}$ and define the set
% \[
% S = S(x, \varepsilon) \defeq \bigcup_{v \in V(\varepsilon + c'\varepsilon^2)} [xv].
% \]
% Note that $S$ is connected, $x \in S$ and $\H(S) = c\varepsilon + o(\varepsilon)$, where $c = 2^n \sqrt{n}$.

% Let $y \in \overline{B_{r + \varepsilon}(x)}$. Note that $y \in \overline{B_{r + \varepsilon}(x)} \subset \overline{B_r(I^n_\varepsilon)}$. Let $z$ be the closest to $y$ point of $I^n_\varepsilon$. Due to symmetry, we can assume that $y_i \geq z_i \geq x_i$ for each $i$. Let the index $i$ belong to the set $J$ if $y_i - z_i \leq c'\varepsilon^2$, and to the set $K$ if $y_i - z_i > c'\varepsilon^2$. Denoting $|yz| = l \leq r$, we have
% \begin{equation}
%     l^2 = \sum_{i=1}^n(y_i-z_i)^2=\sum_{i\in K}(y_i-z_i)^2+o(\varepsilon^2).
%     \label{2z}
% \end{equation}

% Define $\hat{z} \defeq (x_1 + \varepsilon + c'\varepsilon^2, \dots, x_n + \varepsilon + c'\varepsilon^2) \in \mathbb{R}^n$. By the definition, $\hat{z} \in V(\varepsilon + c'\varepsilon^2) \subset S$. Note that $|\hat{z}_i - y_i| \leq \varepsilon + c'\varepsilon^2$ for $i \in J$, and $\hat{z}_i = z_i + c'\varepsilon^2$ for $i \in K$. It follows that
% \[
%  \sum_{i=1}^n (y_i-\hat{z_i})^2 \leq |J|\varepsilon^2 + o(\varepsilon^2) + \sum_{i\in K} (y_i-z_i-c'\varepsilon^2)^2 = |J|\varepsilon^2+l^2-2c'\varepsilon^2\sum_{i\in K}(y_i-z_i)+o(\varepsilon^2).
% \]
% The last equality follows from~\eqref{2z}. Equality~\eqref{2z} also implies that there exists $i \in K$ such that $(y_i - z_i)^2 \geq \frac{l^2}{n}+o(\varepsilon^2)$, so $y_i-z_i \geq \frac{l}{\sqrt{n}}+o(\varepsilon^2)$. %(\textcolor{red}{добавила в каком-то виде $o(\varepsilon^2)$}).
% Then
% \[
% \sum_{i=1}^n (y_i-\hat{z_i})^2\leq l^2+\varepsilon^2\left(|J|-2c' \frac{l}{\sqrt{n}}\right)+o(\varepsilon^2) \leq l^2 + \frac{r - 2l}{r} \varepsilon^2 n + o(\varepsilon^2).
% \]
% If $l > \frac{2r}{3}$, then
% \[
% l^2 + \frac{r - 2l}{r} \varepsilon^2 n + o(\varepsilon^2) \leq l^2 - \frac{n\varepsilon^2}{3} + o(\varepsilon^2) \leq l^2 \leq r^2,
% \]
% if $\varepsilon$ is sufficiently small.
% Otherwise, assuming $\varepsilon < \frac{r}{3\sqrt{n}}$, we have
% \[
% l^2 + \frac{r - 2l}{r} \varepsilon^2 n + o(\varepsilon^2) \leq \frac{4r^2}{9} + \frac{r^2}{9} + o(\varepsilon^2) \leq r^2,
% \]
% if $\varepsilon$ is small enough.
% Either way, $y\in \overline{B_r(S)}$, and the claim is proved.
% \end{proof}

% \begin{corollary}
% Let $x\in \Sigma$. Then $\oordball_{ x}\Sigma \leq 3$. Moreover, there exists $\rho = \rho(x) > 0$ such that
% \begin{enumerate} 
% \item if $\oordball_{x}\Sigma = 2$, then for any $(\Sigma, x)$-nice $\varepsilon < \rho$ the inequality $\angle AxB \geq 2\pi/3$ holds up to $o_\rho(1)$, where $\{A, B\} = \Sigma \cap \partial B_\varepsilon(x)$;
% \label{kapr}
% \item if $\oordball_{x}\Sigma = 3$, then for for any $(\Sigma, x)$-nice $\varepsilon < \rho$ the equation
% \[
% \vv{Ax} + \vv{Bx} + \vv{Cx} = 0
% \]
% holds up to $o_\rho(1)$, where $\{A,B,C\} = \Sigma \cap \partial B_\varepsilon(x)$.
% \label{kapr2}
% \end{enumerate}
% %НАДО ПРОВЕРИТЬ ЧТО МЫ ВЕЗДЕ ГОВОРИМ О КС: ВРОДЕ ДОКАЗАТЕЛЬСТВО НЕ ЧУВСТВИТЕЛЬНО К ЧУЖИМ КУСКАМ СИГМА В ШАРИКАХ 
% %МОЖЕТ ЧТО-ТО ИЗ УТВ НЕВЕРНО (НО ВСЕ ЧТО ИСПОЛЬЗУЕМ ВРОДЕ ОК)
% \label{kaprrr}
% \end{corollary}
% \begin{proof}
% Assume that any of the claims of the corollary is false, then there exists an arbitrarily small $(\Sigma, x)$-nice $\varepsilon > 0$ and such $A, B \in \Sigma \cap \partial B_\varepsilon(x)$ that $\angle AxB$ is less than $2\pi/3$ by a constant which does not depend on $\varepsilon$.
% In view of Remark~\ref{geq_ord}, the inequality $\H(\Sigma \cap B_\varepsilon(x))\geq \oordball_x \Sigma \cdot \varepsilon$ holds.
% Then the set
% \[
% \Sigma \setminus B_\varepsilon(x) \cup \St(A,x,B) \cup S^*(x,\varepsilon) \cup \left( \bigcup_{C \in ( \Sigma \cap \partial B_\varepsilon(x) ) \setminus \{ A, B \}} [xC] \right),
% \]
% where $\St(A,x,B)$ is a Steiner tree on the set $\{ A, x, B\}$ and $S^*(x,\varepsilon)$ is defined in Corollary~\ref{main_c}, is connected and has the energy not greater than $\Sigma$.
% In view of Proposition~\ref{angles4}, it is also shorter than $\Sigma$, which contradicts the optimality of $\Sigma$.
% \end{proof}
% \begin{proof}
% \leavevmode\textcolor{blue}{сказать бы тут ещё пару слов про не больше 3}
% \begin{enumerate}
%  \item In view of Remark~\ref{geq_ord}, the inequality $\H(\Sigma \cap B_\varepsilon(x))\geq 2\varepsilon$ holds.
%  Assume that $\angle AxB$ is less than $2\pi/3$ by a constant which does not depend on $\varepsilon$. Then the set
%  \[
%     \Sigma \setminus B_\varepsilon(x) \cup \St(A,x,B) \cup S^*(x,\varepsilon),
%  \]
%  where $\St(A,x,B)$ is a Steiner tree on the set $\{ A, x, B\}$ and $S^*(x,\varepsilon)$ is defined in Corollary~\ref{main_c}, is connected and has the energy not greater than $\Sigma$. In view of Proposition~\ref{angles4}, it is also shorter than $\Sigma$, which contradicts the optimality of $\Sigma$.
%  \item In view of Remark~\ref{geq_ord}, the inequality $\H(\Sigma \cap B_\varepsilon(x))\geq 3\varepsilon$ holds.
%  Assume that at least one of the three pairwise angles is less than $2\pi/3$ by a constant which does not depend on $\varepsilon$. Without loss of generality, let $\angle AxB$ be such an angle. Then the set
%  \[
%     \Sigma \setminus B_\varepsilon(x) \cup \St(A,x,B) \cup [xC]\cup S^*(x, \varepsilon),
%  \]
%  contradicts the optimality of $\Sigma$ by the same arguments as in item~\ref{kapr}.
% \end{enumerate}
% \end{proof}
%\begin{corollary}
%Let $x\in \G_\Sigma$. Then $\oordball_x\Sigma = \oord_x\Sigma$. Доказательство: разбор случаев. Проверить!  Проверила, легко доказать пока не получилось
%\end{corollary}
%\begin{proof}
%Assume the contrary: $\oord_x\Sigma <\oordball_x\Sigma\leq 3$. Thus there exists connected component $\Sigma\setminus x$ with $\oordball$ equal to $2$ or to $3$. So there are following cases:
%\begin{itemize}
%\item $\Sigma_1$ is unique connected component of $\Sigma\setminus \{x\}$ and $\oordball_x\Sigma_1= 3$.
%\item  $\Sigma_1$ is unique connected component of $\Sigma\setminus \{x\}$ and $\oordball_x\Sigma_1= 2$.
%\item $\Sigma_1$, $\Sigma_2$ are  connected components of $\Sigma\setminus \{x\}$, $\oordball_x\Sigma_1= 2$, $\oord_x\Sigma_1=1$ and $\oordball_x\Sigma_2=1=\oord_x\Sigma_2$.
%\end{itemize}
%\end{proof}

% \begin{corollary}
% \label{cor:tang-comp}
% Let $\Sigma$ be a minimizer for a compact set $M \subset \mathbb{R}^n$ and $r > 0$, and let $x \in \Sigma$.
% \begin{enumerate} 
% \item \label{tang-comp:comp}
% For every one-sided tangent $(ax]$ of $\Sigma$ at $x$ there exists exactly one connected component $\Sigma_1$ of $\Sigma \setminus \{x\}$ to which $(ax]$ is tangent.
% Moreover, $\oordball_x \Sigma_1 = 1$, and for any $(\Sigma_1, x)$-nice $\varepsilon > 0$ the equality $\H(\Sigma_1 \cap \overline{B_\varepsilon(x)}) = \varepsilon + o(\varepsilon)$ holds.
% \item \label{tang-comp:ang} The angle between any two one-sided tangents of $\Sigma$ at $x$ is at least $2\pi/3$.
% In particular, there are at most three one-sided tangents at any point of $\Sigma$.
% \end{enumerate}
% \end{corollary}
% \alextodo{всё, кроме утв. про длину компоненты, следует сразу из пред. следствия; утв. про длину проще вывести из пункта 1 след. леммы}

% \begin{lemma}
% For any $x\in \Sigma$ the following statements hold:
% \begin{enumerate}
% \item For any sufficiently small $\varepsilon > 0$ the equality $\H(\Sigma \cap B_\varepsilon(x)) = \oordball_x\Sigma \cdot \varepsilon +o(\varepsilon)$ holds.
% \alextodo{тут и в док-ве добавить замыкание к шару?}
% %\item There exists $\oordball_x\Sigma$ rays $(B_ix]$ such that for every $\delta>0$ there exists such $\varepsilon_1>0$  that for each $\varepsilon<\varepsilon_1$ such that
% %\[
% %\sharp (\partial B_\varepsilon(x)\cap \Sigma) =\oordball_x\Sigma
% %\]
% %the inequality 
% %\[
% %\angle A_ixB_i<\delta
% %\]
% %holds, where $\{A_i\}_{i=1}^{\oordball_x\Sigma} \defeq \partial B_\varepsilon(x)\cap \Sigma$.
% \label{three}
% \item % $\Sigma$ has $\oordball$ tangent rays at $x$ and 
% Every closed connected component $\Sigma_1$ of $\Sigma \setminus \{x\}$ has a unique one-sided tangent at $x$.
% Thus, by Corollary~\ref{cor:tang-comp}, $\oord_x \Sigma_1 = \oordball_x \Sigma_1 = 1$ and $\H(\Sigma_1 \cap \overline{B_\varepsilon(x)}) = \varepsilon + o(\varepsilon)$ for any sufficiently small $\varepsilon > 0$,
% \alextodo{вынести объяснение в док-во и ссылаться там на~\ref{two}, чтобы доказать для любого малого $\varepsilon$}
% and the pairwise angles between one-sided tangents of $\Sigma$ at $x$ are at least $2\pi/3$.
% \label{four}
% \item The equality $\oord_x\Sigma = \oordball_x \Sigma$ holds, and, in view of Corollary~\ref{kaprrr}, $1 \leq \oord_x \Sigma \leq 3$.
% \alextodo{переписать / убрать док-во, в соотв. с изменённым пред. пунктом}
% \label{ordord-item3}
% \end{enumerate}
% \label{ordord}
% \end{lemma}
% \begin{proof}
% Let us start by proving two auxiliary statements:
% \begin{enumerate}[(a)]
% \item \textit{For any $c > 0$ there exists $\rho > 0$ such that for any $\oordball_x\Sigma$-nice $\varepsilon < \rho$ the inequality $\H(\Sigma \cap B_\varepsilon(x)) < (\oordball_x\Sigma + c ) \cdot \varepsilon$ holds.
% Moreover, in view of Remark~\ref{geq_ord},
% \[
% \oordball_x\Sigma \cdot \varepsilon\leq \H(\Sigma \cap B_\varepsilon(x)) < (\oordball_x\Sigma + c ) \cdot \varepsilon.
% \]}
% Indeed, assume the contrary, i.e. that there exists $c > 0$ and a sequence of $\oordball_x\Sigma$-nice $\varepsilon_k$ such that $\varepsilon_k \rightarrow 0$ and $\H( \Sigma \cap B_{\varepsilon_k}(x) ) \geq (\oordball_x\Sigma +c) \cdot \varepsilon_k$ for every $k$.
% Then, for a sufficiently small $\varepsilon_k$, the set 
% \[
% \Sigma \setminus B_{\varepsilon_k}(x) \cup \left( \bigcup_{A\in \Sigma \cap \partial B_{\varepsilon_k}(x)} [Ax] \right) \cup S^*(x, \varepsilon_k),
% \]
% where $S^*(x, \varepsilon_k)$ is defined in Corollary~\ref{main_c}, is connected, has the energy not greater than $\Sigma$ and is shorter than $\Sigma$, which is not possible.
% \label{one}
% \item \textit{For any $c > 0$ there exists $\rho > 0$ such that for any $\oordball_x \Sigma$-nice $\varepsilon < \rho$ one can find an $\oordball_x \Sigma$-nice $\delta$ satisfying $(1 - c) \cdot \varepsilon \leq \delta < \varepsilon$.
% }

% Indeed, assume the contrary, then there exists $c > 0$ and a sequence of $\oordball_x \Sigma$-nice $\varepsilon_k$ such that $\varepsilon_k \rightarrow 0$ and $\sharp ( \Sigma \cap \partial B_\delta(x) ) \geq \oordball_x\Sigma + 1$ for any $(1 - c) \cdot \varepsilon_k \leq \delta < \varepsilon_k$. Let $\delta_k \leq (1 - c) \cdot \varepsilon_k$ be the supremum of $\oordball_x \Sigma$-nice $\delta < \varepsilon_k$. Then, due to coarea inequality,
% \[
% \H \left( \Sigma \cap B_{\varepsilon_k}(x) \right) \geq \oordball_x\Sigma \cdot \delta_k + ( \oordball_x \Sigma + 1 ) \cdot (\varepsilon_k - \delta_k) \geq ( \oordball_x \Sigma + c ) \cdot \varepsilon_k,
% \]
% which contradicts~\ref{one}.
% \label{two}
% \end{enumerate}

% Now we turn to the claims of the Lemma.

% \begin{enumerate}
% \item Assume the contrary, i.e. that there exist a constant $c_1 > 0$ and a sequence $\xi_k \rightarrow 0$ such that $\H( \Sigma \cap B_{\xi_k}(x) ) \geq (\oordball_x \Sigma + c_1) \cdot \xi_k$.
% Then, due to~\ref{one}, we can assume that $\sharp (\Sigma \cap \partial B_{\xi_k}(x)) \geq \oordball_x \Sigma + 1$ for each $k$.
% Let $\varepsilon_k \geq \xi_k$ be the infimum of $\oordball_x \Sigma$-nice $\varepsilon > \xi_k$.
% Then, due to coarea inequality,
% \[
% \H(\Sigma \cap B_{\varepsilon_k}(x)) \geq (\oordball_x\Sigma + c_1) \cdot \xi_k + ( \oordball_x\Sigma + 1 ) \cdot (\varepsilon_k - \xi_k) \geq (\oordball_x\Sigma + \min(c_1, 1)) \cdot \varepsilon_k.
% \]
% This contradicts~\ref{one}, because for $c \defeq \min(c_1, 1) / 2$ and a sufficiently small $\varepsilon_k$ we must have
% \[
% \H(\Sigma \cap B_{\varepsilon_k}(x)) \leq (\oordball_x\Sigma + c) \cdot \varepsilon_k.
% \]
% \item There exists a sequence of $\oordball_x \Sigma$-nice $\varepsilon_k$ such that $\varepsilon_k \rightarrow 0$ and $\varepsilon_{k + 1} \leq \frac{\varepsilon_k}{2}$ for each $k$.

% In view of item~\ref{three},
% \begin{equation}\label{eq:krays}
% \H(\Sigma \cap ( \overline{B_{\varepsilon_k}(x)\setminus B_{\varepsilon_{k + 1}}(x)} ) ) = \oordball_x\Sigma \cdot (\varepsilon_k-\varepsilon_{k + 1}) + o(\varepsilon_k).
% \end{equation}
% Let $t \defeq \oordball_x \Sigma$, and let $\{ A^k_i\}_{i=1}^t \defeq \Sigma \cap \partial B_{\varepsilon_k}(x) $.
% Then, due to~\eqref{eq:krays}, up to a renumeration of $A^k_i$ for each fixed $k$, we have $\angle A^k_ixA^{k + 1}_i=o_{\varepsilon_k}(1)$ for $1 \leq i \leq t$.
% Then there exist $\{A^\infty_i\}_{i=1}^t$ such that $(A^k_ix] \rightarrow (A^\infty_ix]$ for each $1 \leq i \leq t$.

% In view of item~\ref{tang-comp:comp} of Corollary~\ref{cor:tang-comp}, to show that $(A^\infty_1 x], \dots, (A^\infty_t x]$ are $t$ distinct one-sided tangents each tangent to its own closed connected component of $\Sigma \setminus \{x\}$, it is sufficient to show that for any $z\in \Sigma$ we have
% \[
% \min_{1 \leq i \leq t}\angle zxA^\infty_i=o_{|zx|}(1).
% \]
% Suppose it is not so, i.e. there exists $\gamma > 0$ and a sequence of points $z_k \in \Sigma$ such that $|z_kx| \rightarrow 0$ and
% \[
% \gamma_k \defeq \min_{1 \leq i \leq t} \angle z_kxA^\infty_i \geq \gamma
% \]
% for each $k$.
% Let $\varepsilon_k$ be the infimum of $\oordball_x \Sigma$-nice $\varepsilon \geq |z_kx|$.
% In view of~\ref{two}, for any $c > 0$ and a sufficiently big $k$ one can find an $\oordball_x \Sigma$-nice $\delta_k$ such that $(1 - c) \cdot \varepsilon_k \leq \delta_k < |z_kx| \leq \varepsilon_k$.
% Then, due to item~\ref{three},
% \[
% t \cdot \varepsilon_k + o(\varepsilon_k) = \H( \Sigma \cap B_{\varepsilon_k}(x) ) \geq \H( \Sigma \cap B_{\delta_k}(x) ) + \dist( \Sigma \cap \partial B_{\delta_k}(x), z_k) \geq
% \]
% \[
% \geq t \cdot \delta_k + o(\delta_k) + \sin \gamma_k \cdot \delta_k \geq (1 - c) \cdot (t + \sin \gamma) \cdot \varepsilon_k + o(\varepsilon_k),
% \]
% which is not possible when $1 - c > \frac{t}{t + \sin \gamma}$.

% % Let $\varepsilon_1, \varepsilon_2>0$ be such that $\sharp (\partial B_{\varepsilon_k}(x)\cap \Sigma)=\oordball_x \Sigma$ for $k\in \{1;2\}$ and $0.2<\varepsilon_2/\varepsilon_1<0.8$ (such $\varepsilon_1, \varepsilon_2<\varepsilon$ exist for any $\varepsilon>0$ due to~\ref{two}). Then 
% % \[
% % \H(\Sigma \cap B_{\varepsilon_1,\varepsilon_2}(x) ) = \oordball_x\Sigma \cdot (\varepsilon_1-\varepsilon_2)
% % \]
% % up to $o(\varepsilon_1)$, where $ B_{\varepsilon_1,\varepsilon_2}(x)\defeq \overline{B_{\varepsilon_1}(x)\setminus B_{\varepsilon_2}(x)}$.
% % Let \[\{A^k_i\}_{i=1}^{\oordball_x\Sigma}\defeq \partial B_{\varepsilon_k}(x)\cap \Sigma\] for $k\in \{1;2\}$.
% % Thus, up to renumeration, $\angle A^1_ixA^2_i=o_{\varepsilon_1}(1)$ for $i\in 1, \ldots, \oordball_x\Sigma$. Iterate this for decreasing sequence of $\varepsilon_1$ (for example by halving $\varepsilon_1$ in each step) we get that there exists such $\{A^\infty_i\}_{i=1}^{\oordball_x\Sigma}$ that $(A^k_ix] \rightarrow (A^\infty_kx]$ for every $i\in 1,\ldots\oordball_x\Sigma$.
% % Let $z\in \Sigma \cap B_{\varepsilon_k}(x)$. It is sufficiently to show that $\min_{i\in 1,\ldots\oordball_x\Sigma}\angle zxA^\infty_i=o_{\varepsilon_k}(1)$, id est that $\min_{i\in 1,\ldots\oordball_x\Sigma}\angle zxA^k_i=o_{\varepsilon_k}(1)$. It is true, as
% % \[
% %  \oordball_x\Sigma \varepsilon_k+o(\varepsilon_k) =\H(\Sigma \cap B_{\varepsilon_k}(x)\geq \oordball_x\Sigma \varepsilon_k + \cos (\frac{\angle A_kxz}{2})\varepsilon_{k+1}\geq  \oordball_x\Sigma \varepsilon_k + 0.2\cos (\frac{\angle A_kxz}{2})\varepsilon_k.
% % \]
% % the statement of item. \textcolor{blue}{я сломался :( нам же надо объяснить, что у любой нестабилизирующейся последовательности $x_k \rightarrow x$ из одной компоненты будет один и тот же предел $(x_kx] \rightarrow (ax]$. чёт мы тут этого не объяснили}
% % % %Я ХЗ МОЖЕТ МОЖНО БЫЛО НАПИСАТЬ ПРОЩЕ И ПОНЯТНЕЕ(((
% % \textcolor{red}{мне кажется тут надо подробнее}
% \item By Remark~\ref{ord_comp}, the number of closed connected components of $\Sigma \setminus \{x\}$ is finite, and, if $\Sigma_1$ is one of them, then $\oord_x \Sigma_1 > 0$.
% Due to item~\ref{four}, $\Sigma_1$ has a one-sided tangent, so, by item~\ref{tang-comp:comp} of Corollary~\ref{cor:tang-comp}, $\oordball_x \Sigma_1 = 1$, and, therefore, $\oord_x \Sigma_1 = \oordball_x \Sigma_1$.
% Since the number of components is finite, the same is true for $\Sigma$.
% % Assume the contrary, then there exists a connected component of $\Sigma\setminus \{x\}$ such that for its closure $\Sigma'$ we have $\oordball_x\Sigma' > \oord_x \Sigma'$. Due to Remark~\ref{ord_pos}, $\oord_x \Sigma' \geq 1$, so $\oordball_x \Sigma' \geq 2$. But, due to item~\ref{four}, the set $\Sigma'$ has a tangent line at $x$. Thus, for a sufficiently small $\varepsilon>0$, on the one hand, due to Corollary~\ref{len0}, $\H(B_\varepsilon(x)\cap \Sigma') =  \varepsilon+o(\varepsilon)$, and, on the other hand, due to coarea inequality, $\H(B_\varepsilon(x)\cap \Sigma'\geq \varepsilon$. So we get a contradiction. 
% \end{enumerate}
% \end{proof}

%\begin{remark}
%For every connected component $\Sigma \setminus x$ there exists unique one-sided tangent $(ax]$
%\label{uniqq}
%\end{remark}

% \[
% |x'y(x)| = |\vv{x'x} + \vv{xy(x)}| = \sqrt{\varepsilon^4 + r^2 - 2\varepsilon^2 \langle \vv{xy(x)}, \vv{h} \rangle } \leq \sqrt{r^2 + \varepsilon^4} = r + o(\varepsilon^3)
% \]

% \begin{lemma}
% Let $x\in \Sigma$ be an energetic point with $\oord_x\Sigma \leq 2$. For $\gamma > 0$ define
% %\[
% %K(x, \gamma) \defeq \left\{ \vv{v} \in \mathbb{R}^n \, \Big| \, |\vv{v}| = 1 \text{ and } \angle\left( \vv{v}, \vv{xy(x)} \right) \leq \gamma \text{ for some corresponding point } y(x) \right\},
% %\]
% % $K(x, \gamma)$ be a set of unit vectors $\vv{xk}$ starting at $x$ such that there exists a corresponding point $y(x)$ with $\angle (\vv{xy(x)},\vv{xk})\leq \gamma$.
% %\[
% %N(x, \gamma) \defeq \conv K(x, \gamma) = \left\{ \vv{n} \in \mathbb{R}^n \, \bigg| \, \vv{n} = \sum_{i=1}^m a_i \vv{v_i} \text{ for some } m > 0,\, v_i \in K(x, \gamma),\, a_i > 0,\, \sum_{i=1}^m a_i = 1 \right\}.
% %\]
% \textcolor{red}{
% \[N(x,\gamma)\defeq \left\{ \vv{v} \in \mathbb{R}^n \, \Big| \, |\vv{v}| = 1 \text{ and } \angle\left( \vv{v}, \sum_{i=1}^m a_i\vv{xy(x)} \right) \leq \gamma\right\}\]  for some corresponding to $x$ points $y_1(x) \ldots y_m(x)$ and positive coefficients $a_1, \ldots a_m$ with $\sum a_i \leq 1$.}
% % Also, let $N(x, \gamma) \defeq \conv K(x, \gamma)$, i.e. for any vector $\vv{n}\in N$ there exists such a set of positive coefficients $a_1, \ldots a_m$ that $\vv{xn}=\sum a_i\vv{xk_i}$ for $\vv{xk_i}\in K(\gamma,x)$ and $\sum a_i \leq 1$.%$m\leq 2n$,
% \begin{enumerate}
% \item If $\oord_x\Sigma=1$, then there exists $\gamma=o_\varepsilon(1)$ such that for any sufficiently small $\varepsilon > 0$ satisfying ${\sharp ( \Sigma \cap \partial B_\varepsilon(x) ) = 1}$ one has $\frac{\vv{Cx} }{\varepsilon} \in N(x, \gamma)$, where $\{ C \} \defeq \Sigma \cap \partial B_\varepsilon(x)$.
% \item If $\oord_x\Sigma=2$, then there exists $\gamma=o_\varepsilon(1)$ such that for every sufficiently small $\varepsilon > 0$ satisfying $\sharp ( \Sigma \cap \partial B_\varepsilon(x) ) = 2$ one has $\frac{\vv{Ax}+\vv{Dx} }{|\vv{Ax} + \vv{Dx}|} \in N(x, \gamma)$, where $\{ A, D \} \defeq \Sigma \cap \partial B_\varepsilon(x)$.
% \end{enumerate}
% \label{napr}
% \end{lemma}
% \begin{proof}\leavevmode
% \begin{enumerate}
% \item Assume the contrary, then there exists a constant $\gamma > 0$ and an arbitrarily small $\varepsilon > 0$ such that $\sharp (\Sigma \cap \partial B_\varepsilon(x) ) = 1$, and, if $\{ C \} \defeq \Sigma \cap \partial B_\varepsilon(x)$, then there exists a hyperspace separating $\vv{Cx}$ from $N(x, \gamma)$, i.e. a unit vector $\vv{h} \in \mathbb{R}^n$ such that $\langle \vv{Cx},\vv{h} \rangle = \rho^+ > 0$ and  $\langle \vv{n} ,\vv{h} \rangle \leq -\rho^- < 0$ for any $\vv{n} \in N(x, \gamma)$. Let $W \defeq \Sigma \cap \overline{B_\varepsilon(x)}$. Let
% \[
% H \defeq \{ z \in \mathbb{R}^n \, \big |\, \langle \vv{Cz}, \vv{h} \rangle = 0 \}, \quad H^+ \defeq \{ z \in \mathbb{R}^n \, \big |\, \langle \vv{Cz}, \vv{h} \rangle > 0 \}, \quad H^- \defeq \{ z \in \mathbb{R}^n \, \big |\, \langle \vv{Cz}, \vv{h} \rangle < 0 \},
% \]
% i.e. $H$ is the hyperspace orthogonal to $\vv{h}$ and containing $C$, and $H^+$, $H^-$ are the corresponding halfspaces. Let
% \[
% W' \defeq \{ z - \max( 0, \langle \vv{Cz}, \vv{h} \rangle ) \cdot \vv{h} \, \big |\,  z \in W \},
% \]
% i.e. $W'$ is the set obtained from $W$ by orthogonally projecting $W \cap H^+$ on $H$, and leaving $W \setminus H^+$ in place. Note that $\H(W') < \H(W)$ because $W$ is connected, $x \in W \cap H^+$ and $C \in W \cap H$.

% The set $\Sigma \setminus W \cup W'$ is connected and is shorter than $\Sigma$. We will obtain a contradiction by showing that it also has the energy not greater than $\Sigma$, i.e. that $U(x, \varepsilon) \subset \overline{ B_r( W' ) }$.

% Let $u\in U(x,\varepsilon)$, and let $z\in W$ be such that $|zu|\leq r$. Note that $\angle( \vv{zu}, \vv{xu} ) = o_\varepsilon(1)$ because $|zu|, |ux| \geq r - \varepsilon$ and $|zx| \leq \varepsilon$. By Remark~\ref{rem_cC}, $\angle( \vv{xu}, \vv{xy(x)} ) = o_\varepsilon(1)$ for some corresponding point $y(x)$. Then $\angle ( \vv{zu}, \vv{xy(x)} ) = o_\varepsilon(1)$, i.e. $\frac{\vv{zu}}{|zu|} \in N(x, \gamma)$ if $\varepsilon$ is sufficiently small.

% Let $z' \defeq z - \max( 0, \langle \vv{Cz}, \vv{h} \rangle ) \cdot \vv h \in W'$. If $z'=z$, then $|uz'| = |uz| \leq r$. Otherwise, note that
% \[
% |uz'|^2=\langle \vv{uz} - \langle \vv{Cz}, \vv{h} \rangle \cdot \vv h,\vv{uz} -  \langle \vv{Cz}, \vv{h} \rangle \cdot \vv h \rangle = |uz|^2 + \langle \vv{Cz}, \vv{h} \rangle^2 - 2 \cdot \langle \vv{Cz}, \vv{h} \rangle \cdot \langle \vv{uz},\vv h \rangle = 
% \]
% \[
% = |uz|^2 + \langle \vv{Cz}, \vv{h} \rangle \cdot \left( \langle \vv{Cz}, \vv{h} \rangle - 2 \cdot \rho^- \right).
% \]
% Then, in view of $0 < \langle \vv{Cz}, \vv{h} \rangle \leq \varepsilon$, we have $|uz'|^2 \leq |uz|^2 \leq r^2$ if $\varepsilon$ is sufficiently small. Either way, $U(x, \varepsilon) \subset \overline{ B_r( W' ) }$.


% % Let $k \defeq \langle \vv{Cx},\vv{h} \rangle$. Note that $0 < k < \varepsilon$. Let $x' \defeq x - k \cdot \vv{h}$ be a projection of $x$ on the hyperspace orthogonal to $\vv{h}$ and containing $C$. The set $\Sigma \setminus B_\varepsilon(x) \cup [x'C]$ is connected and is shorter than $\Sigma$. All that is left to obtain a contradiction is to show that this set has the energy not greater than $\Sigma$.

% % Let $u\in U(x,\varepsilon)$. By Remark~\ref{rem_cC}, $\vv{xu} \subset N(x, \gamma)$. Let $z\in [xC]$ \textcolor{blue}{я опять сломался :( почему $[xC]$, у нас же энергетическая точка} be such that $|zu|\leq r$. Then for $k_z\defeq \frac{k|Cz|}{|Cx|}<k$ and $z'= z+k_z\vv h$  the inequality
% % \[
% % |uz'|^2=\langle \vv{uz}+k_1\vv h,\vv{uz}+k_1\vv h \rangle = |uz|^2+k_1^2h^2+2k_1 \langle \vv{uz},\vv h \rangle < |uz|^2
% % \]
% % holds for a sufficiently small $\varepsilon_1$.
% \item Assume the contrary, then there exists a constant $\gamma > 0$ and an arbitrarily small $\varepsilon > 0$ such that $\sharp (\Sigma \cap \partial B_\varepsilon(x) ) = 2$, and, if $\{A, D\} \defeq \Sigma \cap \partial B_\varepsilon(x)$, then there exists a hyperspace separating $\vv{Ax}+\vv{Dx}$ from $N(x, \gamma)$, i.e., a unit vector $\vv{h}$ such that $\langle \vv{Ax}+\vv{Dx},\vv h \rangle = \rho^+ > 0$ and  $\langle \vv n,\vv h \rangle \leq -\rho^- < 0$ for any $\vv n \in N(x, \gamma)$. Let $W \defeq \Sigma \cap \overline{B_\varepsilon(x)}$. Let
% \[
% E \defeq \{ z \in \mathbb{R}^n \, \big |\, |Az| + |Dz| = 2 \varepsilon \},
% \]
% In other words, $E$ is the prolate spheroid with focal points $A$ and $D$, i.e. the set of points with the sum of the distances to $A$ and $D$ equal to $2\varepsilon$. Let
% \[
% W' \defeq \{ z - \max( 0, \langle \vv{Cz}, \vv{h} \rangle ) \cdot \vv{h} \, \big |\,  z \in W \},
% \]
% i.e. $W'$ is the set obtained from $W$ by orthogonally projecting $W \cap H^+$ on $H$, and leaving $W \setminus H^+$ in place. Note that $\H(W') < \H(W)$ because $W$ is connected, $x \in W \cap H^+$ and $C \in W \cap H$.

% Then the set $\Sigma \setminus ([Ax]\cup [Dx])\cup [Ax']\cup [Dx']$, where $x'\defeq x+k\vv{h}$, is better than $\Sigma$: it is shorter and its energy is not greater. Let us consider the ellipsoid consisting of all the points $v$ such that $|Av|+|Dv|=|Ax|+|Dx|=2\varepsilon$. Then, for a sufficiently small $k>0$, $x'$ lies inside it, and hence $|Ax'|+|Dx'|<|Ax|+|Dx|$. The energy doesn't increase similar to the previous item as $\dist(u,z+k_1\vv{h})\leq \dist (u,z)$ for $u\in U(x,\varepsilon)$, $z\in[Ax]\cup[Dx]$ and $0<k_1\leq k$.

% % Assume the contrary, then there exists a hyperspace $H\ni x$ separating $x+\vv{Ax}+\vv{Dx}$ from $N$ \textcolor{red}{$x + N$?}. Let $h$ be a perpendicular to $H$ such that $\langle \vv{Ax}+\vv{Dx},\vv h \rangle > 0$ and  $\langle \vv n,\vv h \rangle < 0$ for every $\vv n \in N$. Then the set $\Sigma \setminus ([Ax]\cup [Dx])\cup [Ax']\cup [Dx']$, where $x'\defeq x+k\vv{h}$, is better than $\Sigma$: it is shorter and its energy is not greater. Let us consider the ellipsoid consisting of all the points $v$ such that $|Av|+|Dv|=|Ax|+|Dx|=2\varepsilon$. Then, for a sufficiently small $k>0$, $x'$ lies inside it, and hence $|Ax'|+|Dx'|<|Ax|+|Dx|$. The energy doesn't increase similar to the previous item as $\dist(u,z+k_1\vv{h})\leq \dist (u,z)$ for $u\in U(x,\varepsilon)$, $z\in[Ax]\cup[Dx]$ and $0<k_1\leq k$.
% \end{enumerate}
% \end{proof}
% \begin{remark}
% In view of Corollary~\ref{ordord} we can exchange $\oordball$ by $\oord$ in the statement of Lemma~\ref{napr}. \textcolor{blue}{дальше всегда пишем $\oord$}
% \end{remark}

% \begin{proposition}\label{discr_str}
% For an arbitrary point $x\in S_\Sigma \sqcup X_\Sigma$ there exists such $\varepsilon=\varepsilon(x)>0$ that set $ \Sigma \cap B_\varepsilon (x) $ consists of $ \oord_x \Sigma $ line segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with pairwise angles between them at least $ 2 \pi / 3 $. Moreover, in the case of $ x \in S_ \Sigma $, set $ \overline{B_\varepsilon (x)} \cap \Sigma $ is a segment or a regular tripod centered at $ x $, and in the case of $ x \in X_\Sigma $ --- a segment with an end at $ x $ and another one at $\partial B_\varepsilon(x)$, or the union of two segments with one end at $ x $ and another one at $\partial B_\varepsilon(x)$, with angle at least $ 2 \pi / 3 $ between them.
% \end{proposition}
% \begin{proof}
% It is easy to see that for each $x \in \Sigma$ inequality $\oordball_x \Sigma \leq 6$ holds. Assume the contrary, then for sufficiently small $\varepsilon>0$ the co-area inequality entails $\H(\Sigma \cap \overline{B_\varepsilon (x)}) \geq 7 \varepsilon$. But then set $\Sigma' \defeq \Sigma \setminus B_\varepsilon(x) \cup \partial B_\varepsilon(x)$ is better than $\Sigma$: it is connected, its energy is not greater and its length is strictly less than of $\Sigma$. This gives a contradiction with the optimality of $\Sigma$.

% Now let $x \in S_\Sigma \sqcup X_\Sigma$ and let $\varepsilon>0$ be such that $\Sigma \cap \overline{B_\varepsilon(x)} \setminus \{x\} \subset S_\Sigma$. Thus, there exists an infinite monotonically decreasing sequence $\varepsilon_i \rightarrow 0$ such that $\sharp (\partial B_{\varepsilon_i}(x) \cap \Sigma) = \oordball_x \Sigma \leq 6$ for every $i$. Without loss of generality let $\varepsilon_1<\varepsilon$. For numbers $l>k$ let us define set
% \[
% \Sigma_{k,l} \defeq \Sigma \cap \overline{{B}_{\varepsilon_k}(x)} \setminus B_{\varepsilon_l}(x).
% \]
% Note that $\Sigma_{k,l} \subset S_\Sigma$ is a Steiner forest and all its vertices belong to $\partial B_{\varepsilon_k}(x) \cup \partial B_{\varepsilon_l}(x)$. Since $\Sigma_{k,l}$ has not more vertices than $13$, the number of its branching points is at most $11$ for each $l>k$ and $\Sigma_{k,l}$ consists of a finite number of line segments, less than $25$. Then there exists such a number $m>k$ that set $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ does not contain a branching points or a maximal segment not containing point $x$. So the number of segments in $\Sigma \cap \overline{B_{\varepsilon_m}(x)}$ is at most the number of segments of every set $\Sigma_{m,n}$, $n>m$ (which is not greater than $24$); in particular it is finite.    

% In view of Lemma~\ref{angles2} set $\Sigma \cap B_{\varepsilon_m}(x)$ should be either a segment with one end at point $x$ and another at $\partial B_{\varepsilon_m}(x)$, or union of two such segments with the angle at least $2\pi/3$ between them, or the union of three such segments with angles $2\pi/3$ between them (i.e. regular tripod with the center at $x$). 
% \end{proof}


Let $Q_1$ and $Q_5$ be such cusps with vertices at $L_1$ and $L_5$ and axes almost parallel to $o_rho(\bar x)$ that 

Let $S$ be the point of intersection $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. Let $A'$ be an area bounded by $[L_1,L_5]$, $\breve{L_1S}, $\breve{L_5S}$ where the arcs are the arcs of circumferences $\partial B_r(y(L_1))$ and $\partial B_r(y(L_3))$. And let $A$ be the union of $A'$ and its reflection regarding to $L_1L_5$. Thus $A$ is a union of two cusps $Q_1\in \mathbb{Q_{|L_1S|}}^{L_5,L_1}$ and $Q_5\in \mathbb{Q_{|L_5S|}}^{L_1,L_5}$. Then sets $S^{Q_1}$ and $S^{Q_5}$ defined at the proof of lemma~\ref{angles2} are such that $\H(S^{Q_1})=o(|L_1S|)$, $\overline{B_r(Q_1)}\subset \overline{B_r(S^{Q_1})}$
URURU


Let us construct a 


Now look at the set $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$, where $S^{[L_1L_5]}$ is defined in the proof of lemma~\ref{angles2}.



  
 Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).



Предположим противное, то есть (ввиду Леммы~\ref{alm} п.~\ref{__2} для $c= \bar c/ 10$) что для сколь угодно малого $\rho > 0$ существует такая ломаная $L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\rho}$, что все углы $\angle((L_iL_{i+1}),(ix))> \bar{c}/2$ при $i=1,2,3,4$. 
Будем считать $(ix)$ осью абсцисс, а $\bar{c}$ достаточно малым. Не умаляя общности, точкам $L_1$, $L_3$, $L_5$ соответствуют верхние точки множества $M$, а точкам $L_2, L_4$ --- нижние: ввиду пункта~\ref{1145} доказательства Леммы~\ref{Losiu} и неравенства $\angle L_{i-1}L_{i}L_{i+1} \leq \pi-\bar{c}$, $i=2,3,4$ двум подряд идущим точкам не могут соответствовать одновременно верхние или нижние точки.
 Заметим теперь, что отношения между отрезками ломаной линейные (то есть отношение оценивается сверху и снизу константой, зависящей от $\bar{c}$), и замена ломаной на отрезки $L_1-L_2-L_4-L_5$ уменьшит длину на величину, линейно зависящую от $[L_1L_2]$:
 поскольку $L_3 \notin B_r(y(L_1))$ выполняется 
 \[
 |Pr_{(y(L_1)L_1)}[L_2L_3]|<|Pr_{(y(L_1)L_1)}[L_1L_2]|+o(|L_1L_3|).
 \label{1111}
 \]
  Поскольку 
  \[
  |\angle (y(L_1)L_1), (ix])-\pi/2| =o_\rho(1)
  \]
 выполняется 
 \[
 |L_2L_3|_y<|L_1L_2|_y+o(|L_1L_2|+|L_2L_3|),
 \]
 где $|\cdot |_y$ означает длину проекции на прямую, перпендикулярную $(ix)$. Тогда
 \[
 |L_2L_3|\sin \frac{ \bar{c}}{2}<|L_1L_2|+o(|L_1L_2|+|L_2L_3|),
 \]
 то есть
 \[
 |L_2L_3|< \frac{1}{\sin \frac{ \bar{c}}{2}}|L_1L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
%Тогда для достаточно малого $\rho$ выполняется

 Аналогично, поскольку  $L_3 \notin B_r(y(L_1))$ и $|\angle (y(L_3)L_3), (ix])-\pi/2| =o_\rho(1)$ выполняется
  \[
 [L_2L_1]<\frac{1}{\sin \frac{ \bar{c}}{2}}|L_3L_2|+o(|L_1L_2|+|L_2L_3|). 
 \]
 В таком случае
 \[
\sin\frac{ \bar{c}}{2}- \frac{o(|L_1L_2|+|L_2L_3|)}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|+|L_2L_3|)}{|L_1L_2|},
 \]
 а значит, для достаточно малого $\rho$ верно
 \[
\frac{\bar c}{3} < \sin \frac{ \bar{c}}{2}- \frac{o(|L_2L_3|(1+\frac{1}{\sin\frac{ \bar{c}}{2}}|L_1L_2|+o_\rho(1)))}{|L_3L_2|}\leq  \frac{|L_2L_3|}{|L_1L_2|}\leq \frac{1}{\sin \frac{ \bar{c}}{2}}+\frac{o(|L_1L_2|(1+ \frac{1}{\sin \frac{ \bar{c}}{2}}+o_\rho(1)))}{|L_1L_2|}< \frac{3}{\bar{c}}.
 \]
 
  %\[[L_2L_3]_y>|L_1L_2|_y-|L_1L_3| o_{\varepsilon(c)}(1)\]
 %|L_1L_2|-\bar{\varepsilon}^2,\]
  %где нижний индекс $y$ означает проекцию на ось абсцисс. То есть $|L_2L_3|>\sin c |L_1L_2|-o_{\bar{\varepsilon}}(1)|L_1L_3|$.
% И наоборот, $|L_1L_2|>\sin \bar{c} |L_2L_3|-o_{\bar{\varepsilon}}(1)|L_1L_3|$. 
 %Из этого очевидным образом следует существование $c_1, c_2>0$ таких, что $c_2|L_2L_3|\geq |L_1L_2| \geq c_1|L_1L_3|$.   
 Аналогично и для остальных $L_i$. 
 
 Замена ломаной $L_1-L_2-L_3-L_4-L_5$ на $L_1-L_2-L_4-L_5$ уменьшит ее длину не меньше, чем на величину, линейно зависящую от $|L_1L_2|$, поскольку $\angle L_2L_3L_4 \leq \pi-\bar{c}$ (а значит $\cos \angle L_2L_3L_4 \geq  -\cos \bar{c}$):
 \begin{multline*}
 |L_2L_3|+|L_3L_4|-|L_2L_4|=\frac{(|L_2L_3|+|L_3L_4|)^2-|L_2L_4|^2}{|L_2L_3|+|L_3L_4|+|L_2L_4|}>\\
 > \frac{2|L_2L_3||L_3L_4| (1+ \cos \angle L_2L_3L_4)}{2(|L_2L_3|+|L_3L_4|)}\geq
 \frac{|L_3L_4|(1- \cos \bar{c})}{ \left (1+\frac{|L_3L_4|}{|L_2L_3|} \right)}\geq  \frac{(\frac{\bar{c}}{3})^3}{(1+\frac{3}{\bar{c}})}|L_1L_2|.
\end{multline*}
 
 
 
% \[
% |L_2L_3|+|L_3L_4|-|L_2L_4|\geq  |L_2L_3|(1+\frac{c}{3}-\frac{1}{\sin c})>|L_2L_3|(1+\frac 2 c),
 %\]
 %поскольку 
 %\[
 %|L_2L_4|=\sin \angle L_2L_3L_4 \frac{|L_2L_3|}{\sin L_2L_4 L_3}\leq  \frac{|L_2L_3|}{\sin L_2L_4 L_3} \leq  \frac{|L_2L_3|}{\sin (\pi-c)}= \frac{|L_2L_3|}{\sin c}.
 %\]
 %ой ОЙОЙ ТУТ НЕ ТАК
 
% \begin{multline*}
 %|L_2L_3|+|L_3L_4|-\sqrt{ |L_2L_3|^2+|L_3L_4|^2+2 %|L_2L_3||L_3L_4|\cos (2c) }\geq \\
%|L_1L_2| \left(\sin c+\sin^2 c-\sqrt{\frac{1}{\sin^2 c}+\frac{1}{\sin^4 c}+2\frac{\cos (2c)}{\sin^3 c}})+o_{\varepsilon(c)}(1|L_1L_2| \right),
% \end{multline*}
%Таким образом замена уменьшает длину множества на величину, линейно зависящую от $|L_1L_2|$.
%\input{pictures/dvapo}
%Обозначим точки $L_6 \defeq [L_1y(L_3)] \cap \partial B_r(y(L_3))$ и $L_7 \defeq [L_5y(L_3)] %\cap \partial B_r(y(L_3))$ где $y(L_3)$ произвольная соответствующая $L_3$ точка. Тогда %$$B_r([L_1L_6]) \cup B_r([L_5L_7]) \supset B_r([L_1L_3]) \cup B_r([L_3L_5]).$$ и %$\H([L_1L_6]) \cup B_r([L_5L_7]))=o_{[L_1L_2]}(1)$ (это следует из теоремы Пифагора и  %пункта~\ref{1145} доказательства Леммы~\ref{Losiu}). Тогда можно заменить ломаную  %$L_1-L_2-L_3-L_4-L_5$ на $L_6-L_1-L_2-L_4-L_5-L_7$ и получить противоречие с оптимальностью %$\Sigma$ (см. рис~\ref{fig:dvapo}).
%А значит
%\[
%\H([L_1L_2]\cup [L_2L_4]\cup[L_4L_5]\cup S^{[L_1L_5]})\leq \H(L_1-L_2-L_3-L_4-L_5)-|L_2L_3|(1+\frac 2 c)+o(|L_1L_5|)<\H(L_1-L_2-L_3-L_4-L_5).
%\]
Тогда множество $ \Sigma \setminus ([L_2L_3] \cup [L_3L_4]) \cup [L_2L_4]\cup S^{[L_1L_5]}$ лучше $\Sigma$: является связным (поскольку все внутренние точки исходной ломаной --- степени два), обладает меньшей длиной и не большей энергией. Противоречие с оптимальностью $\Sigma$ (см. рис~\ref{fig:dvapo}).
%ПОМЕНЯТЬ РИСУНОК ИЛИ ВЕРНУТЬ ЗАКОМЕНЧЕННОЕ



\[ 
\H(Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))) \geq \cos (\angle z_0x_0a_0) |z_0 x_0|\geq 
\]
Herewith $\angle ((ax], (a_0x_0])=o_{\rho_2}(1)$, а значит, при достаточно малом $\rho_2$, все односторонние касательные к $\sigma \cap B_{\rho_0}(x_0)$ имеют угол с $(a_0x_0]$, больший $1/20$.
Тогда
\[
\H(\sigma \cap B_{\rho_0}(x_0)) \geq \frac{Pr_{(a_0x_0]}(\sigma \cap B_{\rho_0}(x_0))}{\cos \frac{1}{10}}\geq \frac{\cos (\angle  z_0x_0a_0)}{\cos \frac{1}{10}}|z_0 x_0|=\frac{\cos (o_{\rho_0}(1))}{\cos \frac{1}{10}}\rho_0.
\]
С другой стороны, поскольку ребро $(a_0x_0]$ направлено в обе стороны, выполняется $\H(\sigma \cap B_{\rho_0}(x_0))=\rho_0+o_{\rho_0}(1)$. Противоречие для достаточно малого $\rho_0$.


Не умаляя общности будем считать, что ребро $(ax]$ направлено в одну сторону, поскольку в противном случае применим пункт~\ref{A} (см замечание~\ref{remA}).
Пусть $\varepsilon>0$ такое, что $\sharp (\partial B_\varepsilon(x)\cap \Sigma)=\oordball_x\Sigma \leq 3$. И пусть $s \in \partial B_\varepsilon(x)$ такая, что путь из $s$ в $x$ лежит в $\overline{B_\varepsilon(x)}$.

Рассмотрим величину поворота пути: $|\turn(\breve{sx})|<2\pi$. Аналогично рассуждениям в предыдущем пункте заметим, что конечность величины поворота и наличие в компоненте связности энергетических точек только одного ребра, причем направленного в одну сторону, влечет конечность числа точек ветвления на пути из $s$ в $x$. Таким образом можно выбрать $\varepsilon>0$ таким, что $\breve{sx}$ не содержит точек ветвления.

Тогда ввиду Леммы~\ref{dug_ok}  $\breve{sx}$  содержится внутри некоторого псевдоконуса.

%Пусть инъективная функция $f: [0;1] \rightarrow \R^2$ параметризует $\breve{[sx]}$. Множество $\breve{[sx]} \cap G_\Sigma$ содержится в псевдоконусе $Q_{\rho}^{a,x}$. Будем также считать, что это псевдоконус имеет следующий вид: $Q^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left( Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) \right)$ для некоторых сходящихся к нулю монотонных последовательностей неотрицательных чисел $\{s_k\}$ и $\{\rho_k\}$, где $\rho_1=\varepsilon$ (см Лемму~\ref{con}). Будем считать выбранные последовательности минимальными по включению. Пусть точки $c,d \in [0;1]$ такие, что $f([c,d])\cap G_\Sigma=f(c) \cup f(d)$. Тогда, ввиду отсутствия на дуге $\breve{[sx]}$ точек ветвления, выполняется $f([c,d])=[f(c),f(d)]$. В таком случае, если $f(c) \in Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k}}(x) $, $f(d) \in Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+1}}(x) $, то выполняется $[f(c);f(d)] \subset  Q(\rho_{k-1},s_{k-1},x,a) \setminus B_{\rho_{k+1}}(x)$. А значит, 
%\[
%\breve{[sx]}=f([0;1]) \subset \bar{Q}^{a,x}_{\varepsilon} \defeq \bigcup_{k=1}^{\infty} \left(Q(\rho_k,s_k,x,a) \setminus B_{\rho_{k+2}}(x) \right).
%\]
%Тогда к $\breve{[sx]}$ применим пункт~\ref{A}.
%МОЖЕТ НАДО ВЕРНУТЬ
%\end{proof}

усть $\Sigma'$ --- замыкание компоненты связности $\Sigma \setminus \{x\}$ и пусть $\Sigma'$ содержит бесконечную последовательность энергетических точек ребра $(ax]$, сходящуюся к $x$. Пусть кроме того $\Sigma' \cap \overline{B_{\rho}(x)}$ не содержит иных энергетических точек для некоторого $\rho>0$. Тогда $\Sigma' \cap \overline{B_{\rho}(x)}$ содержит конечное число точек ветвления.  
%То есть найдется такое $\rho_1>0$, что множество $\overline{B_{\rho_1}(x)} \cap \Sigma'$ является дугой. 
Кроме того найдется такое $\rho_1>0$ и псевдоконус $Q_1 \in Q^{a,x}_{\rho_1}$, что $\Sigma' \cap \overline{B_{\rho_1}(x)}\subset Q_1$. %При этом прямые, содержащие односторонние касательные к $\Sigma $ в энергетической точке $\bar x$ ребра $(ix]$, стремятся к $(ix)$ при $\bar x \rightarrow x$, $i=a,b$.


Для любой точки $\bar{x} \in G_\Sigma \cap  \Sigma' \cap U \setminus \{ x\}$ касательные лучи к $\bar x$ параллельны ближайшему к ней энергетическому ребру $(ix]$ с точностью до $\alpha/100$.

Докажем утверждение шага от противного: пусть, не умаляя общности, точка $x^a_1 \subset Q^{a,x}_\rho \cap U \cap \Sigma' \cap X_\Sigma$ имеет порядок два. 
Пусть $[x^a_1;t]$ --- максимальный по включению  отрезок, содержащийся на пути из $x^a_1$ в $x$. Тогда, по предположению и ввиду следствия~\ref{sm_an},
\[
\alpha/100< \angle((ax),(x^a_1t)) \leq \pi/6+\alpha/100.  
\]
Несложно заметить, что $\angle ((x^a_1t],(ax])= \angle((ax),(x^a_1t))$ (а не $\pi-\angle((ax),(x^a_1x))$) поскольку в противном случае любой путь, начинающийся с $x^a_1-s$, где $[x^a_1s]$ --- второй максимальный отрезок инцидентный $x$, находится внутри области, ограниченной путем из $x^a_1$ в $x$ и двумя пустыми шарами с радиусом $r$ и с центрами в точке, соответствующей $x^a_1$, и в точке сгущения точек, соответствующих энергетическим точкам ребра $(ax]$. В таком случае такой путь не может содержать энергетических точек ребра $(bx]$, а значит концевыми точками для него могут быть только энергетические точки ребра $(ax]$ степени $1$, ввиду леммы~\ref{alm} принадлежащие $X_\Sigma$. Но путь, начинающийся с $x^a_1-s$ и в точках ветвления продолжающийся не тем отрезком, который является почти перпендикулярным $(ax]$, 
%(нетрудно заметить, что всегда найдется два направления, имеющих с ребром угол, не больший $\pi/6+\alpha/100$), 
не будет содержать энергетических точек ребра $(ax]$ степени $1$ (а также точек $\partial U$, точки $x$ и энергетических точек ребра $(bx]$ степени $1$), а значит никогда не закончится.

The point $y$ belongs to $M$ and corresponds to $x$.   
\item Let hyper-plane $\xi$ be orthogonal to $(xy)$. Then it contains the energetic ray $(zx]$ of $\Sigma$ with a vertex at $x$. So it is an energetic hyper-plane.
\item Let us define an \textit{orientation} (clockwise or counterclockwise) of energetic ray $(zx]$ and energetic hyperplane $\xi$ such way that the orientated angle in this direction from $(zx]$ to $(yx]$ is equal to $\pi/2$.
 \label{orientation}

It is easy to notice that then the orientated angle in this direction from $\xi$ to another energetic hyper-plane (if it exists) at $x$, is not less than $\pi$.

\item Let $x \in E_\Sigma$. Then there exists one or two energetic hyper-plane with vertex at $x$ (sometimes we will subscribe a vertex to a hyper-place).
\label{netri}
\item
One energetic hyper-plane $\xi$ can have two orientations (we say that it is orientated in the both directions or two-orientated) if there exist two different limit points of $y_k$, where $y_k$ corresponds to $x_k$. Otherwise it is one-orientated.
\item if there is two-orientated energetic ray at $x$, then the containing it energetic hyper-plane is also two-orientated. But not vice versa. 
\item In the case of two-orientated $\xi$ there is no other energetic hyper-plane at point $x$.
\end{enumerate}


% \begin{lemma}
% Let $r>0$ and let $x \in \mathbb{R}^n$. Then for every $m\leq n$
% and sufficiently small $\delta>0$ for the cube $I^m=[-\delta;\delta]^m$ there exists such sets $S_0$, $S_1$,\ldots $S_{2^m}$ that $\overline{B_{r}(I^m)} \subset \overline {B_r(\bigcup_{i=1}^{2^n} S_i)}$ and
% \begin{itemize}
% \item each vertex of $I^m$ belong to a set $\bigcup_{i=1}^{2^n} S_i$;
% \item $S_i$ is connected for every $i\in 0,1,\ldots 2^m$, set $\bigcup_{i=0}^{2^m} S_i$ is also connected;
% \item $\H(\bigcup_{i=1}^{2^m} S_i)=o(\delta)$, $\H(S_0)=c(m)\delta$, where $c(m)\leq 2^{m}\sqrt{m}$ and $(0,\ldots,0) \in S_0$.
% \end{itemize}
% \label{cube}
% \end{lemma}
% \begin{proof}

% Let us construct sets $S_i$ is connected for every $i\in 0,1,\ldots 2^m$ by the following way: for each vertex $A_i$ of $I^m$ let $S_i$ be a union of $n$ segments with length $c(n)\delta^2$, incident to $A^i$, collinear to coordinate axis, lying outside of the $\Int I^m$, where \[c(n)\defeq \frac{n\sqrt{n}}{2r}.\]

% Let $y \in \overline{B_{r}(I^m)}$ and let $z \in I^m$ be the nearest to it point from $I^m$. If $|yz|< r$ we can apply the result for smaller $\frac{|yz|}{r}\delta$, so it is sufficiently to check the statement in case $|yz|=r$. 
% So $\sum_{i=1}^n (y_i-z_i)^2=r^2$. Let $I$ be the set of such indices 
% that $z_i=y_i\in(-\delta,\delta)$ for $i\in I$. Then for the rest indices (denote set of them by $J$) $z_i$ is equal to $\pm \delta$. Thus \[\sum_{i\in J} (y_i-z_i)^2=r.\]
% Now let $\hat{z}$ be the nearest to $y$ point from $\overline{\bigcup_{i=0}^{2^n} S_i}$. Let, without less of generality
% $y_i\geq 0$ for every $i$ and $y_i\geq z_i$ for every $i\in J$. Then $\hat{z_i}= \delta$ for $i\in I$.
% Let also $J_1$, $J_2$ be such set of indices that $J=J_1 \sqcup J_2$ and
% \begin{itemize}
%     \item Iff $i\in J_1$ then $y_i \in [\delta, \delta+c\delta^2]$; $z_i=\delta$, $\hat{z_i} = y_i$. In this case $y_i - \hat{z_i}=0$ and $c\delta^2 \geq y_i - z_i\geq 0$.
%     \item Iff $i\in J_2$ then $y_i > \delta+c\delta^2$; $z_i=\delta$, $\hat{z_i} = \delta+c\delta^2$. 
%     \item Iff $i \in I$ then $z_i=y_i \in [0;\delta[$, $\hat{z_i}=\delta$ and $0<\hat{z_i}-y_i\leq \delta$.
% \end{itemize}
% Then
% \begin{equation}
%     r^2=\sum_{i=1}^n(y_i-z_i)^2=\sum_{i\in J_1}(y_i-z_i)^2+\sum_{i\in J_2}(y_i-z_i)^2=\sum_{i\in J_2}(y_i-z_i)^2+o(\delta^2).
%     \label{2z}
% \end{equation}
% And
% \begin{equation}
%  \sum_{i=1}^n (y_i-\hat{z_i})^2=\sum_{i\in I} (y_i-\hat{z_i})^2+ \sum_{i\in J_2} (y_i-\hat{z_i})^2\leq |I|\delta^2+\sum_{i\in J_2} (y_i-z_i-c\delta^2)^2=|I|\delta^2+r^2+o(\delta^2)-2c\delta^2\sum_{i\in J_2}(y_i-\delta).  
%  \label{3z}
% \end{equation}
% The last equality follows from~\eqref{2z}. First equality of~\eqref{2z} also implies existence of such $i\in J_2$ that $(y_i-z_i)^2\geq \frac{r^2}{n}$ and thus $y_i-\delta \geq \frac{r}{\sqrt{n}}$. 
% Then~\eqref{3z} implies
% \[
% \sum_{i=1}^n (y_i-\hat{z_i})^2\leq r^2+\delta^2(|I|-2c \frac{r}{\sqrt{n}})+o(\delta^2)\leq r.
% \]

% %The set $S_0$ has just to connect all vertices of $I^m$. For example it can be %$(2^m-1)$ edges of the cube, forming a tree on its vertices. Thus $\H(S_0)=2^m\delta$.% Or $S_0$ can be
% Let set $S_0$ be a union of $2^{m}$ segments connecting the center with vertices of the cube. Thus $\H(S_0)=2^m\sqrt m \delta$.  

% So $y\in \overline{B_r(\bigcup_{i=0}^{2^n} S_i)}$ and the statement is proved.
% \end{proof}

% At first we need the following statements: \textcolor{blue}{убрать вложенность и выделить эти 2 утверждения в отдельную лемму, поправить и корректно ввести все обозначения в этой лемме}
% \begin{enumerate}
% \item For a given $r>0$ and an arbitrary segment $[uv]$ of a sufficiently small length $\varepsilon>0$ there exists such a set $S^{uv}$ that  $|\H(S^{uv})|=o(\varepsilon)$ and $\overline {B_r([uv])} \subset \overline{B_r(S^{uv})}$. Moreover, $S^{uv}=S^u \cup S^v$, where $u\in S^u$, $v \in S^v$, $S^u$ and $S^v$ are both connected.  
% \label{segment}
% \begin{proof}
% Due to Pythagorean theorem, \textcolor{blue}{добавь корень, перепиши чуть подробнее мб со словами} there exists such $\delta=o(\varepsilon)$ that for every $z\in \overline{B_r([uv])}$ the inequality 
% \[
% \dist (z, \{u\}\cup \{v\})\leq r+\delta
% \]
% holds.
% Thus the statement follows by taking $S^u$ ($S^v$) equal to $S$ from Lemma~\ref{cube} for the $n$-dimensional cube with the center at $u$ (at $v$) and sides of length $2\delta$.
% \end{proof}
% \item For a sufficiently small $\varepsilon > 0$ and an arbitrary cusp $Q\in \mathbb{Q}_\varepsilon^{a,x}$ there exists such a connected set $T^Q$ that $|\H(T^Q)|=\varepsilon+o(\varepsilon)$, $\overline{B_r(Q)} \subset \overline{B_r(T^Q)}$ and $T^Q \supset ((ax] \cap B_\varepsilon(x))$.
% % (see Fig.~\ref{TQ}).
% %For an arbitrary cusp $Q\in Q_\varepsilon^{a,x}$ there exists such a set $S^Q$ that $|\H(S^Q)|=o(\varepsilon)$ and $\overline{B_r(Q)} \subset \overline{B_r(S^Q)}$. Moreover, $S^Q=S_1 \cup S_2$, where $\overline{B_r(S_1)} \supset \overline{B_{o(\varepsilon)}((ax]\cap \partial B_\varepsilon(x))} \supset \overline{B_r(\partial Q \cap \partial B_\varepsilon(x))}$, $x \in S_2$ and both $S^1$ and $S^2$ are connected.% (see Fig.~\ref{TQ}).
% \begin{proof}
% Let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$. Let $\rho$ be the maximum of $\delta$ from item~\ref{segment} on the closed set of segments $[xz]$ where $z\in Q \cap \partial B_\varepsilon (x)$. Thus $\rho=o(\varepsilon)$. 
% Let $\xi$ be the maximum of $\rho$ and the diameter of the set $Q \cap \partial B_\varepsilon (x)$. Then $\xi =o(\varepsilon)$ too. \textcolor{blue}{поправить определение $\xi$, чтобы всё стало хорошо; написать поподробнее, какими свойствами cusp'а мы пользуемся}

% Thus the statement follows by taking $T^Q\defeq [x\bar x] \cup S^Q \cup S^x$, where $S^Q$ ($S^x$) is defined in Lemma~\ref{cube} for the $n$-dimensional cube with the center at $\bar x$ ($x$) and sides of length $4\xi$.

% %Let $\bar x \in (ax] \cap \Int Q^{a,x}_\varepsilon$ and let $\delta=o(\varepsilon)$ be such that $B_\delta(\bar x) \supset  (Q_\varepsilon^{a,x} \cap H_{\bar x, (ax]})$ where $H^+_{\bar x, (ax]}$ is a half-space, cut off from ${x}$ by hyper-plane $H_{\bar x, (ax]}\ni \bar x$  perpendicular to $(ax)$. In view of the definition of a cusp $\diam (Q_\varepsilon^{a,x} \cap H_{\bar x, (ax]})=o(\varepsilon)$ and $\conv (\overline{B_\delta(\bar x)}, \{x\}) \supset Q^{a,x}_\varepsilon$. 

% %Now let $T(Q^{a,x}_\varepsilon)$ be a union of $[\bar x; x]\cup S^{\bar x, \delta+c\varepsilon^2} \cup S^{x,c\varepsilon^2}$, where $c(n)$ is defined in Lemma~\ref{cube} and $S^{\cdot,\cdot}$ in Corollary~\ref{ball} .

% %Clearly, $T^{Q}$ meets all requirements. %is connected, $\H(T^Q)=\varepsilon+o(\varepsilon)$

% \end{proof}
% % \item For a cusp $Q\in Q_\varepsilon^{a,x}$ there exists such connected set $T^Q$ that $|\H(T^Q)|=\varepsilon+o(\varepsilon)$, $\overline{B_r(Q)} \subset \overline{B_r(T^Q)}$ and $T \supset ((\partial Q \cap \partial B_\varepsilon(x)) \cup \{x\})$ (see Fig.~\ref{TQ}).
%  %\begin{proof}
%  %In the notations of the previous item let us define $Z \defeq (ax] \cap \partial B_\varepsilon(x)$. Then set 
%  %\[
%  %T^Q \defeq S^Q \cup [Zx].
%  %\]
%  %\end{proof}
% %meets all requirements.
% \end{enumerate}

%\begin{figure}
%\center{\includegraphics[width=0.4%\caption{Construction of sets $S^Q$, $T^Q$.}
%\label{TQ}
%\end{figure}

% \textcolor{blue}{сослаться на следствие, а это док-во закоментить}

% \textcolor{blue}{кажется, для связности нам нужно ещё дотянуться до всех точек $W \cap \partial Q$ (и так во всех смежных утверждениях)}

% First, assume that two connected components $\Sigma_1$ and $\Sigma_2$ of $\Sigma \setminus \{x\}$ have the same one-sided tangent $(ax]$. In view of Lemma~\ref{con}, for any sufficiently small $\varepsilon > 0$ and $W \defeq \Sigma_1 \cup \Sigma_2 \cap \overline{B_\varepsilon(x)}$ there exists such a cusp $Q \in  \mathbb{Q}_\varepsilon^{a,x}$ that $W \subset Q$ and $W \cap \partial Q \subset \partial B_\varepsilon(x) \cup \{x\}$. Note that $\H(W) \geq 2\varepsilon$.

% Let $\bar x \defeq (ax] \cap \partial B_\varepsilon(x)$ and let $T^x$ and $T^Q$ be the sets from Lemma~\ref{smallsets}, item~\ref{cuspfortangent}. The set 
% \[
% \Sigma \setminus W \cup T^x \cup T^Q \cup [x\bar x],
% \]
% is connected, and has the energy not larger than $\Sigma$. It also has the length shorter than $\Sigma$ because $\H(W) \geq 2\varepsilon$ and $\H(T^x \cup T^Q \cup [x\bar x]) = \varepsilon + o(\varepsilon)$. This is not possible, since $\Sigma$ is a minimizer, so our assumption is false.


% \item For every $\gamma>0$ define $\rho(\gamma)>0$ as supremum of such numbers that for every energetic point $\bar x \in B_{\rho(\gamma)}(x)\cap \Sigma_1$ and for every corresponding point $y(\bar x)$ there exists such a point $y(x)$ corresponding to $x$ that $\angle ((y(\bar{x})\bar x],(y(x)x])\leq \gamma/2$. Thus we define sets $N(x_1,\delta)=\{\pm \vv{v}|\angle( \vv{v}, \vv{z})\leq \delta, \vv{z}\in N(x_1)\}$ and
% \[
% N_1(\gamma,x,\Sigma_1)\defeq \bigcup_{\bar x \in B_{\rho(\gamma)}(x)\cap \Sigma_1\cap \G_\Sigma\setminus \{x\}} N(\frac{\gamma}{2}, \bar x).
% \]
% Clearly that $ N_1(\gamma,x,\Sigma_1)\subset N(\gamma,x)$, is not empty and the vectors of $ N_1(\gamma,x,\Sigma_1)$ are perpendicular to $(ax]$ up to $\gamma$.
% For every $\bar x\in B_{\rho(\gamma)}(x) \cap \Sigma_1\cap \G_\Sigma \setminus \{x\}$, by Lemma~\ref{napr}, $\vv{s(\bar x)}$ belongs to $N(\gamma,x)$ and is perpendicular to $(ax)$ up to $\gamma$.

% \item Note that $(x_kx] \rightarrow (ax]$. On the one hand, $\Sigma \cap B_r(y) = \emptyset$, so $\angle yxx_k \geq \pi/2-o_{|x_kx|}(1)$, and $\angle yxa \geq \pi/2$. On the other hand, $\Sigma \cap B_r(y(x_k)) = \emptyset$, so $\angle y(x_k)x_kx \geq \pi/2-o_{|x_kx|}(1)$. Considering the sum of angles in triangle $\triangle x_kxy(x_k)$, we have $\angle y(x_k)xx_k \leq \pi/2+o_{|x_kx|}(1)$, so $\angle yxa \leq \pi/2$.
% Therefore, $\angle yxa=\pi/2$.
% \item Assume the contrary, then there exist $\gamma > 0$ and a sequence $\{ x_k\} \subset \Sigma_1 \setminus \{x\}$, $x_k \rightarrow x$ such that $\vv{s(x_k)}$ is not $\gamma$-orthogonal to $\vv{ax}$ for each $k$. Each $x_k$ is an energetic point because $\vv{s(x_k)} \neq \vv{0}$. By Lemma~\ref{napr}, $\vv{s(x_k)} \in N(x_k)$, so there exist corresponding points $y_i(x_k)$ and $\alpha_{k,i} \geq 0$ for $1 \leq i \leq n$ such that $\vv{s(x_k)} = \sum_i \alpha_{k,i} \cdot \vv{x_ky_i(x_k)}$. After, if necessary, replacing $\{x_k\}$ by a subsequence, we can assume that $y_i(x_k) \rightarrow y_i(x)$ for each $i$. Then, in view of item~\ref{almost-orthogonal:item3}, for a sufficiently big $k$ each $\vv{x_ky_i(x_k)}$ is $\gamma$-orthogonal to $\vv{ax}$. But then $\vv{s(x_k)}$ is also $\gamma$-orthogonal to $\vv{ax}$ as their linear combination, which contradicts our assumption.

% \textcolor{blue}{следующее рассуждение короче, но там есть проблемка: не все $\vv{xy(x)}$ ортогональны $\vv{ax}$; нужно, чтобы $y(x)$ была предельной}

% \textcolor{blue}{If $\bar x$ is a non-energetic point, then $\vv{s(\bar x)} = \vv{0}$ and the statement of the item is true. Otherwise, consider any corresponding point $y(\bar x)$. Note that $y(\bar x) \in U(x, |\bar xx|)$, so, by Remark~\ref{rem_cC}, $\angle y(\bar x)xy(x) = o_{|\bar xx|}(1)$ for some corresponding point $y(x)$. Thus, in view of item~\ref{almost-orthogonal:item3}, $\vv{xy(\bar x)}$ is $o_{|\bar xx|}(1)$-orthogonal to $\vv{ax}$. Then the same is true for any vector in $N(\bar x)$, which, by Lemma~\ref{napr}, contains $\vv{s(\bar x)}$.}

%\begin{proposition}
%Let $x\in \E_\Sigma$, let $\Sigma_1$ be a closed connected component of $\Sigma \setminus x$ containing a sequence of energetic points converging to $x$. Then we can define a set $N_1(\gamma,x,\Sigma_1)\subset N(\gamma,x)$ by a following way: let $\rho(\gamma)$ be such that for every energetic point $\bar x \in B_{\rho(\gamma)}(x)\cap \Sigma_1$ and for every corresponding point $y(\bar x)$ there exists such a point $y(x)$ corresponding to $x$ that $\angle ((y(\bar{x})\bar x],(y(x)x])\leq \gamma/2$. Thus we define  a set 
%\[
%N_1(\gamma,x,\Sigma_1)\defeq \bigcup_{\bar x \in B_{\rho(\gamma)}(x)\cap \Sigma_1\cap \G_\Sigma} N(\frac{\gamma}{2}, \bar x).
%\]
%If $(ax]$ is a tangent line to $\Sigma_1$ at $x$, then vectors of $ N_1(\gamma,x,\Sigma_1)$ are perpendicular to $(ax]$ up to $\gamma$.
%\end{proposition}

%О, а вот тут надо новое писать
%\begin{remark}
%For every $x\in \Sigma$ the inequality $\oord_x\Sigma \leq \oordball_x\Sigma\leq 2\pi<7$ holds due to coarea inequality. Otherwise the set $\Sigma \setminus B_\varepsilon(x) \cup \partial B_\varepsilon(x)$ for sufficiently small $\varepsilon >0$ is better than $\Sigma$: it has not greater energy and strictly less length than $\Sigma$, and is still connected, so we have a contradiction with optimality of $\Sigma$.
%\end{remark}

% \begin{definition}
% The \textit{arc} $ \breve {[ax]} \subset \Sigma $ ($\breve {]ax]}$ or $\breve {]ax[}$) 
%  is the continuous injective image of the closed (semi-closed or open, respectively) interval. If inclusion and exclusion of the ends of the arc don't matter we will write $\breve{ax}$. \textcolor{red}{кажется, мы никогда не пользуемся этим обозначением, а дугой называем не только часть сигмы (см. определение cusp'а). предлагаю просто убрать это определение, и везде пояснять, что дуга это инъективный образ отрезка (мы и так это почти везде делаем).}

% \end{definition}

%может есть термин
%\begin{definition}
%By \textit{n-arc} in $\mathbb{R}^n$ we understand such a set that its projection on every axis of an orthonormal basis is a segment. 
%\end{definition}


==> parts/unproved.tex <==
\section{Unproved}

\begin{lemma}
Let $x \in \E_\Sigma$ be a non-isolated energetic point. Let $\Sigma_0$ be a closed connected component of $\Sigma \setminus \{x\}$. Let $\varepsilon>0$ with $\sharp ( \Sigma \cap \partial B_\varepsilon(x) ) = \oord_x\Sigma$ and $\sharp ( \Sigma_0 \cap \partial B_\varepsilon(x) ) = 1$ be sufficiently small. Let $F\in \Sigma_0\cap B_{\varepsilon}(x)$ be a branching point and let $\Sigma_1\ni F$ be such a closed connected component of $\Sigma \setminus F$ that $\eta \defeq \dist (\Sigma_1, \partial B_{\varepsilon}(x) \cup \{x\})>0$.

Then there exists such $\gamma=o_\varepsilon(1)$ and such finite graph $G$ that
\begin{enumerate}
    \item all vertices $V(G)$ belong to $\Sigma_1$;
    \item for every edge and both its vertices the angle between the edge and a one-sided tangent \alextodo{уточнить, какая именно касательная} at the vertex is not greater than $10\gamma$;\label{second}
    \item for every two vertices the path between them in $\Sigma$ and in $G$ contains the same set of vertices;\alextodo{тут уже используется, что $G$~--- дерево}
    \item for every vertex $v \in V(G)$ its degree as a vertex of the graph is equal to its order as a point of $\Sigma_1$: $\deg_G v = \oord_{v} \Sigma_1$.  
%$T$ doesn't contain loops; ОТСУТСТВИЕ ЦИКЛОВ ИЛИ ЧТО-ТО ДРУГОЕ
%    \item all leaves of $T$ are terminal points of of $\Sigma_0$ and all branching points of $T$ are the branching points of $\Sigma_0$.          МОЖНО ПРО ЛЮБЫЕ СТЕПЕНИ
\end{enumerate}
\label{tree}
\end{lemma}
\begin{remark}
$G$ is a finite tree. Moreover, if $A,B,C,D$ are such vertices of $G$ that $D$ belongs to every path from $i$ to $j\neq i$ where $i,j \in \{A,B,C\}$, then $D\in V(G)$. 
\end{remark}
\begin{proof}
Fix $\gamma,c=o_\varepsilon(1)$.
For $\bar x \in \Sigma_0$ define its \textit{comfort zone} as such $\delta(\bar x)>0$ that there exists $\bar \delta = \bar \delta(\bar x) \in [8\delta(\bar x),9\delta(\bar x)]$ with both $\delta(\bar x)$ and $\bar \delta(\bar x)$ satisfying
\begin{enumerate}[(a)]
    \item $\oord_{\bar x}\Sigma_1=\sharp(B_{\delta(\bar x)}(\bar x)\cap \Sigma_1)=\sharp(B_{\bar \delta(\bar x)}(\bar x)\cap \Sigma_1)$;\alextodo{хочется здесь и в подобных местах требовать что каждая компонента границу в одном месте пересекает}
    \item for every positive $\delta'\leq \bar \delta$ there exists such connected $S=S(\bar x, \delta')\ni \bar{x}$ that $F_M(\Sigma \setminus B_{\delta'}(\bar x)\cup S) \leq F_M(\Sigma)$ and $\H(S)\leq c\delta'$;МОЖНО СИЛЬНЕЕ AS $F_M(\Sigma \setminus B_{\delta'}(\bar x)\cup S) =o(\delta')$\label{ququ}
    \item for every positive $\delta'\leq \bar \delta$ and for every $t\in \Sigma_1\cap B_{\delta'}(\bar x)\setminus \{ \bar x\}$ the inequality $\angle t\bar x a_i\leq \gamma$ holds for some $i \in \{1, \dots, \oord_{\bar x}\Sigma_1\}$, where $[\bar x, a_i)$ are one-sided tangents of $\Sigma_1$ at $\bar x$.
\end{enumerate}

As $\Sigma_1$ is a compact set, there exists a minimal by inclusion finite collection $\{x_i\}_{i\in I}\subset \Sigma_1$ such that $\Sigma_1 \subset \bigcup_{i \in I} B_{\delta(x_i)}(x_i)$.
Define a graph $T$ on the set of vertices $V(T) \defeq \{x_i\}_{i \in I}$ as follows: let $(x_a, x_b) \in E(T)$, i.e. let $x_a$ and $x_b$ be adjacent, if and only if there is no other $x_i$ on the path $\Sigma_1(x_a, x_b)$.\alextodo{ввести это обозначение}
Note that if $x_a$, $x_b$ and $x_c$ are such points of $\Sigma_1$ that each path in $\Sigma_1$ from $x_i$ to $x_j$ (where different indices $i,j$ belong to $\{a,b,c\}$) contains the same branching point $F\notin \{x_a,x_b,x_c\}$, then there is such an index $l\in I$ that $F=x_l$. Note that $T$ is tree and all leaves of $T$ has an order $1$ in the set $\Sigma_1$.\alextodo{это дублирует ремарку?}
\textbf{Note that all conditions on $G$ except~\ref{second} hold for $T$ by the construction}.

\textcolor{blue}{%
For $j \in I$ denote $S_j := \Sigma_1 \cap B_{\delta(x_j)}(x_j)$; $S_j$ is connected, otherwise the condition on $\oord$ would not hold.
Note the following.
\begin{enumerate}[(I)]
    \item For each $j \in I$ there exists a point $s_j \in S_j$ such that $s_j \notin \bigcup_{i \in I \setminus \{j\}} S_i$ since the collection $\{x_i\}_{i \in I}$ is minimal by inclusion.
    \item For any $j \in I$ with $\oord_{x_j} \Sigma_1 = 1$ we have $x_j \notin \bigcup_{i \in I \setminus \{j\}} S_i$ because it is true for $s_j$ and all sets $S_i$ are connected.
    \item For any $j \in I$ with $\oord_{x_j} \Sigma_1 = 3$ we have $x_j \notin \bigcup_{i \in I \setminus \{j\}} S_i$.
    Indeed, if $x_j \in S_i$ for some $i \in I \setminus \{j\}$, then two connected components of $\Sigma_1 \setminus \{x_j\}$ which do not contain $x_i$ would both contain a leaf of $T$.
    But then they would both intersect $B_{\delta(x_i)}(x_i)$, which again violates the condition on $\oord$.
    \item For any $(x_i, x_j) \in E(T)$ we have $\Sigma_1(x_i, x_j) \subset (S_i \cup S_j)$. 
    Indeed, suppose the opposite, then, since $\Sigma_1(x_i, x_j) \subset \bigcup_{k \in I} S_k$, there exists a point $Q \in \Sigma_1(x_i, x_j) \setminus (S_i \cup S_j)$, $Q \in S_k$ for some $k \in I$.
    But $S_k$ is connected, so, without loss of generality, $x_i \in S_k$.
    Then $\oord_{x_i} \Sigma_1 \neq 1, 3$, so $\oord_{x_i} \Sigma_1 = 2$.
    But then $x_k \in \Sigma_1(x_i, s_i) \subset S_i$.
    It follows that $\delta(x_i) > |x_is_i| > |x_ks_i| > \delta(x_k)$ and $\delta(x_k) > |x_kQ| > |x_iQ| > \delta(x_i)$, which is a contradiction.\alextodo{надо тут картинку бахнуть}
    \item In particular, for any $(x_i, x_j) \in E(T)$ we have $|x_ix_j| < \delta(x_i) + \delta(x_j)$, so either $x_i \in B_{2\delta(x_j)}(x_j)$, or $x_j \in B_{2\delta(x_i)}(x_i)$.\label{cond:doublerad}
\end{enumerate}%
%
As long as condition~\ref{second} is not satisfied, we will modify $T$ by deleting some vertices and changing the set of edges, so that all the other conditions still hold, and, additionally,~\ref{cond:doublerad} also continues to be true.
Since the number of vertices is finite, this process will stop sooner or later.
}

Let us call the vertex $U\in V(T)$ \textit{bad} if the second condition does not hold at $U$ for one of its incident edges, i.e. if $\angle (t_U, [UV]) > 10 \gamma$, where $t_U$ is the nearest \alextodo{надо пояснять, что значит nearest} tangent ray of $\Sigma$ at $U$, and $[UV]\in E(T)$. Note that, if this is the case, then %$\delta(V)=o(\delta(U))$ (depends on ...), particularly,
$\delta(U) < \frac{\delta(V)}{8}$.
Let $U$ be an arbitrary bad vertex which is the first bad vertex on a path in $T$ from $F$ to $U$.
We will delete from $T$ the vertex $U$ and, possibly, some other vertices (and edges, incident to them) lying inside $B_{2\delta(V)}(V)$\alextodo{надо сказать, как перестраивается дерево}.
% in such a way that the first bad vertex become farer on the path from $F$ through $U$ in $\Sigma$.
Then, if there are still bad vertices in $T$, we will repeat the process.

\textcolor{blue}{%
%
}

We are going to show that then the algorithm stops, the following two conditions will hold for each edge $UV \in E(T)$:
\begin{enumerate}[(I)]
    \item $|UV| \leq 2( \delta(U) + \delta(V) )$;\alextodo{а это нужно где-то?}
    \item $\max( \angle(t_U, (UV)), \angle(t_V, (UV)) ) \leq 10\gamma$ for some tangent rays $t_U$, $t_V$ of $\Sigma$ at points $U$ and $V$, accordingly.\alextodo{а это ровно условие~\ref{second}}
\end{enumerate}

% Let us denote by \textit{case A} situation when vertex  $U$ belongs to the path from $F$ to $V$ and by \textit{case B} the opposite case. 
The following cases are possible:
\begin{enumerate}
   
    
    %There are two cases: \begin{enumerate}
        %\item 
%\textbf{        $U$ (and hence $Y$) belongs to the path from $F$ to $V$ in $\Sigma$.}

%Point $Y$ can not be ``bad'' vertex as $V$ was the first.
%радиус удвоился
        %\item \textbf{$V$ belongs to the path from $F$ to $U$ in $\Sigma$ (hence $V$ belongs to the path from $F$ to $Y$ in $\Sigma$).}
%Vertex $Y$ can be a ``bad'' vertex.
%радиус удвоился      
 %   \end{enumerate}
    \item \textbf{There exists $k>1$ and a set of consecutive adjacent vertices $\{A_i\}_{i=1}^{i=k} \subset V(T)\cap B_{2\delta(A_0)}(A_0)$ with $A_0\defeq V$, $A_1 \defeq U$ such that \alextodo{это условие всегда верно из-за того, что справа есть $i = 0$; может быть справа должно быть $\delta$, а не $2\delta$?}
    \[
    \left( \Sigma_{VU} \cap B_{\frac{3}{2} \delta(V)}(V) \right) \subset \bigcup_{i = 1}^k B_{2\delta(A_i)}(A_i)\cup B_{\delta(A_0)}(A_0),
    \]
    where $\Sigma_{UV}$ is a connected component of $\Sigma_1 \setminus V$ containing $U$.}
    Clearly, for every $i$ the inequality $\delta(A_i)\leq 3\delta(A_0)$ holds.
    %Then in \textit{case B} we can just 
    %delete from $V(T)$ all inner vertices and edges of path from $A_0$ to $A_k$ and all edges and vertices belonging to resulting connected components, which doesn't content $A_k$ or $A_0$ and add to $E(T)$ the edge $[A_0A_k]$. %любой другой i тоже ок, может надо другой
    There are two possible cases. %in \textit{Case A}:
    \begin{enumerate}
        \item \textbf{For every $j\leq k$ and every one-sided tangent $t_{A_j}$ of $\Sigma_1$ at $A_j$ the inequality $\angle ( t_{A_j},t_{A_0})\geq 9\gamma$ holds.}
        
        Due to construction conditions\alextodo{можно и конкретно сослаться}, we have $\angle (t_{A_0},[A_0A_{j}])\leq \gamma$.
        
        Then in every ball $B_{\delta(A_j)}(A_j)$ with $j\geq 1$ we have the inequality
        \[
        \H(\Sigma_1 \cap B_{\delta(A_j)}(A_j)) - \H(\Pr_{t_{A_0}} ( \Sigma_1 \cap B_{\delta(A_j)}(A_j) ) ) \geq 2\delta(A_j)(1 - \cos (8\gamma)) = 4\delta(A_j)\sin^2(4\gamma),
        \]
        where $\Pr_{t_{A_j}}(\cdot)$ is the orthogonal projection to the tangent line $t_{A_j}$.
        Note also that\alextodo{непонятно :(}
        \[
        \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))\geq \sum_{j=1}^k\frac{\H(\Sigma_1 \cap B_{\delta(A_j)}(A_j))}{4},
        \]
        where $\Sigma_{UV}$\alextodo{это уже определялось выше, может стоит обозначить за $\Sigma_2$ в начале случая и везде пользоваться?} is a connected component of $\Sigma \setminus V$  containing $U$ and
        \[
        B_{2\delta(A_0),\delta(A_0)}(A_0) := B_{2\delta(A_0)}(A_0)\setminus B_{\delta(A_0)}(A_0).
        \]
        Hence,\alextodo{вообще лучше наверное всё что внутри $\H$ обозначить буквой}
        \[
        \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0)) - \H( Pr_{t_{A_0}} ( \Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0) ) ) \geq \sin^2(4\gamma) \sum_{j = 1}^k \delta(A_j) \geq \frac{\delta(A_0)\sin^2(4\gamma)}{4}.
        \]
        %\[
        %\H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0))\geq
        %\]
        On the other hand,
        \[
        \H(\Sigma_{UV} \cap B_{2\delta(A_0)}(A_0)\setminus B_{\delta(A_0)}(A_0)) = \delta(A_0) + o(\delta(A_0)),
        \]
        and
        \[
        \H(\Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0)) - \H(Pr_{t_{A_0}} ( \Sigma_{UV} \cap B_{2\delta(A_0),\delta(A_0)}(A_0) ) ) \leq \delta(A_0) (1 - \cos\gamma) = 2\delta(A_0)\sin^2\frac{\gamma}{2}.
        \]
        So we got a contradiction for $\gamma < 0.2$.
        
        
        
        %thus $\angle (t_{A_0},t_{A_{j}})\geq 2\gamma$ for every $j\leq k$ and hence $\angle (t_{A_0},[A_{j-1}A_{j}])\geq \gamma$
      %  for every $j$. % On the other hand in \textit{case A} the inequality \[\angle (t_{A_j}[A_j,A_{j-1}]), \angle (t_{A_j}[A_j,A_{j-1}])\leq \gamma\] holds for $j>1$.
     %But this is impossible, otherwise we can pick $\bar A$ such that $|3/2\delta(A_0)-|A_0\bar A||=o(\delta(A_0))$ and delete in $\Sigma$ path between $A_0$ and $\bar A$ (we also delete all connected components doesn't contain $A_0$ or $\bar{A}$) and add the segment $[A_0\bar A]$ and a connected set $S\ni A_0$ from Lemma... instead of it. The resulting set is better than $\Sigma$ as the length of the deleted set was at least $\frac{3|\delta(A_0)|}{2\sin \gamma}+o(\delta(A_0))$ and the length of the added set is $\frac{3|\delta(A_0)|}{2}+o(\delta(A_0))$. 
       % So we get a contradiction.
%                \[
 %       \sharp (\Sigma \cap B_{|A_0A|(A_0)})=\oord_{A_0}(\Sigma).
  %      \]
   %     Thus
        
        \item \textbf{There exists such $1 < j \leq k$ that $\angle (t_{A_j},t_{A_0}) < 9\gamma$ for some one-sided tangent $t_{A_j}$ of $\Sigma_1$ at $A_j$.}     
        Due to construction,
        \[
        \angle (t_{A_j}, (A_0A_j)) < 10\gamma. 
        \]
        We delete from $V(T)$ all inner vertices of the path between $A_0$ and $A_j$ (and all edges and vertices belonging to resulting connected components, which do not contain $A_0$ or $A_j$) and add the edge $[A_0A_j]$ to $E(T)$.\alextodo{а почему удаление компонент ничего не портит?}
        
        Note that $|A_jA_0| \leq 2\delta(A_0)$. 
        %(the vertex $A_j$ was not ``bad'' as $U$ was the first bad one). %тут утроился угол 
    \end{enumerate}
    \alextodo{Я пока не понял (а) где мы пользуемся тем, что $U$ первая плохая на пути от $F$, (б) почему от удаления торчащих из середины удаляемого пути компонент ничего не ломается и (в) что происходит в случае 1а}
    \item \textbf{There exists such a point $Y \in V(T)$ that $U$ belongs to the path in $T$ from $V$ to $Y$, and $\delta(Y)+\frac{3}{2}\delta(V)>\dist(V,Y)\geq 2\delta(V) $.}
    Thus $2\delta(Y) \geq \delta(V)$ and $\angle(t_Y,(YV)) < \gamma < 10\gamma$ for some one-sided tangent $t_Y$ of $\Sigma_1$ at $Y$.
    \begin{enumerate}
    \item If $\angle(t_V, (YV)) < 10\gamma$ (note that it is true if $\delta(Y) \leq 8\delta(V)$), then we delete from $V(T)$ all inner vertices of the path between $Y$ and $V$ (and all edges and vertices belonging to resulting connected components, which do not contain $Y$ or $V$) and add the edge $[YV]$ to $E(T)$.
    
    \item Otherwise, we also delete from $T$ the same vertices and edges, also add the edge $[YV]$ to $E(T)$, and then repeat the algorithm for $V$ as $U$ and $Y$ as $V$ ($V := Y$ and $U := V$). 
    At each step we have three possible cases: case 1(b), 2(a) and 2(b) (it stops in the first two cases). When this process stops we will have two vertices that satisfy both conditions.
    \end{enumerate}
    %Note that in \textit{case A} point $Y$ can not be ``bad'' vertex as $U$ was the first, and in \textit{case B} it can but the first ``bad'' vertex is later than before the reconstruction of the tree.
\end{enumerate}
\end{proof}
\begin{lemma}
Let $x \in \E_\Sigma$ be a non-isolated energetic point. Let $\Sigma_0$ be a closed connected component of $\Sigma \setminus \{x\}$, and let $(ax]$ be its unique one-sided tangent at $x$. Let $\varepsilon>0$ with $\sharp ( \Sigma \cap \partial B_\varepsilon(x) ) = \oord_x\Sigma$ and $\sharp ( \Sigma_0 \cap \partial B_\varepsilon(x) ) = 1$ be sufficiently small. Let $P \subset \Sigma_0$ be the path from $\partial B_\varepsilon(x)$ to $x$ in $\Sigma_0$. Let $F$ be any branching point of $\Sigma_0$ such that $F \in \Int P$, and let $(bF]$ be the one one-sided tangent of $\Sigma_0$ at $F$ which is not a one-sided tangent of $P$ at $F$. Then $\vv{Fb}$ is $o_\varepsilon(1)$-orthogonal to $\vv[F]{ax}$.
\label{choice}
\end{lemma}
\begin{proof}
  %\item if $16\delta (A_{j+1})\geq 4\delta(A_i)\geq %\delta(A_{i-1})$ then angles between one-sided tangents of %$\Sigma$ at $A_i$ with $[A_{i-1}A_i]$ and $[A_iA_{i+1}]$ are %not greater then $\gamma$;
Let $(bF]$ be tangent to a closed connected component $\Sigma_1$ of $\Sigma_0 \setminus \{F\}$. Define $d(F) \defeq \dist(F, \partial B_\varepsilon(x))$ and $d(\bar x) \defeq \min( \dist( \bar x, \partial B_\varepsilon(x) ), 2 \cdot |\bar xF| )$ for $\bar x \in \Sigma_1 \setminus \{F\}$. Note that $\sharp ( \Sigma_0 \cap \partial B_\varepsilon(x) ) = 1$ implies that $d(\bar x) > 0$ for any $\bar x \in \Sigma_1$. Fix $\gamma=o_\varepsilon(1) > 0$. \textcolor{blue}{вообще она должна быть $o_\varepsilon(1)$, надо понять, какими утверждениями мы хотим пользоваться и сослаться на них тут}
%Let us construct the following tree with some points of $\Sigma_1$ as vertices.
%Let $\gamma=o_\varepsilon(1)$ be as in Lemma~\ref{napr}.% By the definition, any vector $\vv n \in N(x, \gamma)$ is perpendicular to $(ax)$ up to $\gamma$. \textcolor{blue}{надо это где-то объяснить!}

By item~\ref{four} of Lemma~\ref{ordord}, given any $\gamma > 0$, for each $\bar x \in \Sigma_1\textcolor{red}{\setminus \{F\}}$ \textcolor{blue}{почему без $F$? она же точно в коллекцию входит} there exists $0 < \delta(\bar x) < d(\bar x) / 2$ with $\sharp ( \Sigma_1 \cap \partial B_{\delta(\bar x)}(\bar x) ) = \oord_{\bar x}\Sigma_1$ such that, if $\Sigma_2$ is any closed connected component of $\Sigma_1 \setminus \{\bar x\}$ with the one-sided tangent $(\bar a\bar x]$ at $\bar x$, then the inequality $\angle s\bar x\bar a<\gamma$ holds for any $s \in  \Sigma_2 \cap \overline{B_{2\delta(\bar x)}(\bar x)}$.
Let $T$ be as in lemma~\ref{tree} for such connected component of $\Sigma \setminus F$ that doesn't contain 
$x$ or points from $\partial B_{\delta(x)}(x)$.

Consider the set of all leaves of $T$, excluding $F$. All these points are points of order $1$ in $\Sigma_1$. Thus, due to Proposition~\ref{prop:alm-orth} and Lemma~\ref{napr},  the edges of $T$ incident to them belongs to $N_1(2\gamma, x,\Sigma_1)$ and hence are perpendicular to $(ax)$ up to $2\gamma$. We want to show that every edge in $T$ is also perpendicular to $(ax)$ up to $2\gamma$. Assume the contrary. Then let us consider such a vertex $A$ of tree $T$ that the tree $T_1$ which is a closure of connected component of $T\setminus A$
has more than two vertices, vertex $A$ is a leaf of $T_1$, the edge $\vv{AB}$ incident to $A$, is such that $|\angle (AB),(ax)-\pi/2|>2\gamma$, and all other edges of $T_1$ are perpendicular to $(ax)$ up to $2\gamma$. There are two cases: if $B$ is of order $2$ then for a vertex $C$ adjacent to $B$ vector  $\vv{BC}$ is perpendicular to $(ax)$ up to $2\gamma$
and \[
\frac{\vv{AB}}{|AB|}+\frac{\vv{BC}}{|BC|}
\]
is also perpendicular to $(ax)$ up to $4\gamma$. Thus $\vv{AB}$ also should be perpendicular to $(ax)$ up to $4\gamma$, so we get a contradiction. If $B$ is of order $3$ then for vertices $C$,$D$ adjacent to $B$ the vectors $\vv{BC}$,$\vv{BD}$ and $\vv{BA}+\vv{BC}+\vv{BD}$ are perpendicular to $(ax)$ up to $2\gamma$, so we also get a contradiction. Therefore each edge of $T$, including the one incident to $F$, is perpendicular to $(ax)$ up to $2\gamma$. Then one of the three one-sided tangents $(bF]$ of $\Sigma_0$ at $F$ (the one that is not a one-sided tangent of $P$) is perpendicular to $(ax)$ up to $6\gamma=o_\varepsilon(1)$.  

%It is easy to see that this collection contains point $B$ and a sufficiently small partition of every path from $F$ to a leaf of the tree, i.e. the distance between the adjacent (in the order of the path) points $x_s$ and $x_t$ is less than $\varepsilon(x_s)+\varepsilon(x_t)$. \textcolor{blue}{тут явно надо подробнее (и, возможно, надо аккуратнее определять $\varepsilon(x)$)}

%If there is no point $B$ in the collection $\{x_i\}$ we will add point $B$ and a number $\varepsilon(B)$ in the collection too. 
%ТУТ возможно ЕСТЬ ОБМАН
%Починка обмана: Every path in $\Sigma_2$ from $B$ to a leaf of the tree is also a compact set with finite length, so we add in the collection points in such way that for every path collection contains sufficiently small partition (i.e. the distance between the adjacent (in the numeration of the path) points $x_s$ and $x_t$ are less than $\varepsilon(x_s)+\varepsilon(x_t)$ ). 

%After it we repeat the procedure for every path (there is finite number of such pathes) from $B$ to leaves such that each path was covered by finite union of balls with points on the path.

%Now we connect points $x_i$ by segments in the same order as these points are connected in $\Sigma_1$.% ТУТ СЛОЖНОСТЬ! ВДРУГ ОНИ БЫЛИ СОЕДИНЕНЫ ДЛИННЫМ ПУТЕМ ТО ЕСТЬ ОТРЕЗКИ ДЛИННЫЕ

%We have constructed a tree. Consider the set of all leaves of this tree, excluding $F$. All these points are points of order $1$ in $\Sigma_1$. Thus, due to Proposition~\ref{prop:alm-orth},  the edges of the tree incident to them \textcolor{red}{belongs to $N_1(2\gamma, x,\Sigma_1)$ and hence} are perpendicular to $(ax)$ up to $2\gamma$ \textcolor{blue}{а это откуда?}.
%\textcolor{red}{We want to prove by induction on the number of branching points, that edge of this tree, incident to $F$ is also  perpendicular to $(ax)$ up to $2\gamma$. At first let there is no branching points in this tree. Then the tree is a path $F-x_1-x_2-\ldots -x_N$ where $\vv{x_{N-1}x_N}\in N_1(2\gamma, x,\Sigma_1)$ and $\vv{x_{i-1}x_i}+\vv{x_ix_{i+1}}\in N_1(2\gamma, x,\Sigma_1)$ой кажется все же надо попросить чтобы длины были почти одинаковыми}


%Then, as the sum of unit vectors (collinear with the edges of the tree) incident to each vertex of the tree is perpendicular to $(ax)$ up to $2\gamma$, the segment incident to $F$ is also perpendicular to $(ax)$ up to $2\gamma$ (we can prove it by the induction on the number of branching points of the tree). \textcolor{red}{сложно и много скобок :( надо наверно это переписать предложениями покороче и без вложенностей. мб индукцию тоже стоит поподробнее}



% Let $\xi=o(\varepsilon)$ be a positive number. For $B$ let positive $\rho_1<\xi$  be such that $\sharp (\partial B_{\rho_1}(B)\cap \Sigma_1)=\oordball_B\Sigma_1=1$ and let $x_2\defeq \partial B_{\rho_1}(B)\cap \Sigma_1$. Then let positive $\rho_2\leq \rho_1$ be such that $\sharp (\partial B_{\rho_2}(x_1)\cap \Sigma_1)=\oordball_{x_2}\Sigma_1$. Then define $x_3$ if $\oordball_{x_2}\Sigma_1=2$ ( or $x_3$ and $x_4$ if $\oordball_{x_2}\Sigma_1=3$) as points of $\partial B_{\rho_2}(x_1)\cap \Sigma_1$ except the one point of  $\partial B_{\rho_2}(x_1)\cap \Sigma_1$ belonging to the path in $\Sigma_1$ from $x_1$ to $x_2$. 

%At every step we use the radius $\varepsilon_i$ not less that the half of supremum possible radius. If the process is infinite so we have a limite point $C=\lim_{k_i\rightarrow \infty} x_{k_i}$. Then there exists such $w>0$ that $\partial B_w(C)=\oordball_C \Sigma_1$. If $\oordball _C\Sigma=1$ then we delete all $x_{k_i}\in B_w(C)$, add in the collection $x_i$ point $x_{k_i}\defeq C$ and $\varepsilon_{k_i}\defeq w$ and finish this branch of algorithm. Otherwise, if  $\oordball _C\Sigma>1$ then we delete all $x_{k_i}\in B_w(C)$, add in the collection one or two points $x_{k_i}\defeq \partial B_w(C)\cap \Sigma_1$ except the one point of  $partial B_{w}(C)\cap Sigma_1$ belonging to the path in $\Sigma_1$ from $x_1$ to $C$.
%ТУТ НАДО ПРОВЕРИТЬ ЧТО ВСЕ КОРРЕКТНО С ТОЧКИ ЗРЕНИЯ СЧЕТНОСТИ.

%So, when algorithm stoped, we have constracted a (finite) Steiner tree such that  its vertices are points of $\Sigma_1$ and it edges are almost collinear to one-sided tangents of $\Sigma_1$ up to $o_\xi(1)=o(\varepsilon)$. Thus all its leaves, except $B$, are the terminal points of $\Sigma_1$. It means that all its terminal vectors (vectors collinear to edges inject to leaves and sum of vectors inject to vertices of degree two), except may be the one inject to $B$, are almost perpendicular to $(ix)$ up to $o_\rho(1)$. But then, as sum of terminal vectors of a steiner tree is equal to $0$, the edge, inject to $B$ is also almost perpendicular to $(ix)$. Then a one-sided tangent line to $\Sigma$ at point $B$ is almost perpendicular to $(ix)$ up to $o_\varepsilon(1)$.  
\end{proof}


%\begin{lemma}
%Пусть $\alpha$ -- подпространство, перпендикулярное всем $(xy(x))$ которые много встречаются в к с $\Sigma \setminus x$. Тогда $\Sigma'$ не может содержать ломанную из пяти звеньев, все внутренние точки которой степени 2, все отрезки которой имеют угол хотя бы $c=pi/{2^5}$ с $\alpha$. Доказательство: заменим два средних отрезка на один и извинимся.
%\label{no_poli}
%МОЭЕТ ЕСТЬ ЛИШНИЕ УСЛОВИЯ
%\end{lemma}


%\begin{lemma}вспомогательная

%определим N()\begin{itemize} 
    %\item Точки степени 1 из $B_\rho(x)$ не могут быть пределом энергетических, потому что с одной стороны к ним сходится последовательность точек из $N^\perp$ а с другой из $N$, тогда большая длина.
    %\item Точки из E более или менее лежат в $N^\perp$
    %\item Пусть есть конечное топ дерево все вершины которого кроме возможно одной -- из $\X_\Sigma$ из N(x, o). Тогда оставшаяся вершина тоже
    %\begin{proof}
    %Пусть точек ветвления 0. Тогда путь все внутренние вершины которого степени 2. Тогда ясно что сама точка не из E. И что входящий в нее отрезок -- из N
    
   % По индукции уберем точку ветвления соединенную с двумя концевыми. Возможно она соединена с помощью путей со звеньями в точках степени 2 из Х. Но тут нет никаких точек из Е и все ок, оставшийся отрезок входящий в эту точку -- из N
    %\end{proof}
    
    %\item Пусть есть топ дерево все вершины которого кроме возможно одной -- из $\X_\Sigma$ из N (x, o). Тогда оставшаяся вершина тоже
    
%\end{itemize}

%\end{lemma}
%\textcolor{red}{
%\begin{lemma}
%Let $x\in \Sigma$, let $\Sigma_1$ be a connected component of $\Sigma %\setminus x$ and let $\varepsilon>0$ be sufficiently small. let %$\Sigma'\cap B_\varepsilon(x)$ contains a polyline $L_1-L_2-L_3-L_4-L_5$ %such that of points of the polyline have order $2$ in $\Sigma$. Then %there exists such $j\in \{2,3,4\}$ that $\angle %L_{i-1}L_iL_{i+1}=\pi-o_{\varepsilon(1)}$.
%\label{no_poli}
%\end{lemma}
%\begin{proof}

%\end{proof}
%}


% \begin{theorem}
% The number of branching points in any minimizer $\Sigma$ is finite. \label{main}
% \end{theorem}
% \begin{proof}
% Assume the contrary. Then let $x$ be an arbitrary limit point of a sequence of branching points. Let $\varepsilon>0$ be sufficiently small and such that $\partial B_\varepsilon(x) \cap \Sigma =\oord_x\Sigma$. Due to item~\ref{four} of Corollary~\ref{ordord}, any connected component $\Sigma'$ of $\Sigma \setminus \{x\}$ has the unique one-sided tangent at $x$ and $\sharp ( \Sigma' \cap \partial B_\varepsilon(x) ) = 1$ \textcolor{blue}{опять же, про это нигде экспилицитно не написано}. Let $\Sigma'$ be a connected component of $\Sigma \setminus \{x\}$ such that the path $P$ in $\Sigma'$ from $\partial B_\varepsilon(x)$ to $x$ contains an infinite number of branching points. Let $(ax]$ be the unique one-sided tangent of $\Sigma'$ at $x$. Let $F$ be any of these branching points. By Lemma~\ref{choice}, one of the three one-sided tangents to $\Sigma'$ at $F$ (the one that is not a one-sided tangent of $P$) is perpendicular to $(ax)$ up to $o_\varepsilon(1)$.  
% % ТУТ ОБМАН МОЖЕТ ЛУЧШЕ НЕ О УГЛАХ А СРАЗУ ОБ ОТНОШЕНИИ К ПРОЕКЦИИ

% We want to prove that all one-sided tangents of $P$ (there are at most two one-sided tangents at each point) have angle at least $\pi/6 - o_\varepsilon(1)$ with $(ax)$. Let us consider a path $P'$ in $\Sigma'$ from $F$ to $X$, where $X$ is either equal to $x$, or is an arbitrary point of $P$. We will construct a finite partition of this path as in the proof of Lemma~\ref{choice}. In the notation of the lemma, we pick the finite subcovering of the balls $B_{\varepsilon(\bar x)}(\bar x)$ for points $\bar x \in P'$. Thus we have finite collections $\{x_k\}$ and $\{\varepsilon(x_k)\}$. $F$ and $X$ must belong to $\{x_k\}$ by the definition of $\varepsilon(\bar x)$.
% %It is easy to see that the first and the last points of the collection (in the order of the path) are $F$ and $X$.
% %$\{x_k\}$ contains both $F$ (as the first $x_1$) and $X$ (as the last one).

% % and numbers $\varepsilon(F)$ and $X$.
% %\begin{itemize}
% %\item let $x_1 \defeq F$. Let a positive $\xi=o(\rho)$. Let $\varepsilon_1$ be such that $\sharp(\partial B_{\varepsilon_1}(x_1)\cap \Sigma)=\oordball_{x_1}\Sigma$.
% %\item let $x_{k+1} \in \partial B_{\varepsilon_k}(x_k)\cap \Sigma$ and lay in the path from $x_k$ to $x$ in $\Sigma$. Let also positive $\varepsilon_{k+1}\leq \varepsilon_k$ be such that $\sharp(\partial B_{\varepsilon_{k+1}}(x_{k+1})\cap \Sigma)=\oordball_{x_{k+1}}\Sigma$.
% %\item If there is a point $A\neq X$ such that $A=\lim_{k \rightarrow infty} x_k$ then we will delete tails of sequences: let $\varepsilon<\xi$ be such that $\sharp(\partial B_{\varepsilon}(A)\cap \Sigma)=\oordball_{A}\Sigma$ then we will rename $x_l \defeq A$, $\varepsilon_l\defeq\varepsilon$ where $l$ was the first such number that all points $x_l, x_{l+1}, \ldots$ belong to $B_{\varepsilon}(A)$. After it we erase all values $x_k$, $\varepsilon_k$ for $k>l$.
% %\end{itemize}
% Note that for every $k$ the sum 
% \[
% \frac{\vv{x_{k-1}x_k}}{|x_{k-1}x_k|} + \frac{\vv{x_{k+1}x_k}}{|x_{k+1}x_k|} 
% \]
% is almost (up to $2\gamma=o_\varepsilon(1)$) perpendicular to $(ax)$) %\textcolor{red}{ Let there exists such $i$ that $((x_{i}x_{i+1}),(ax))<\pi/9$ and let $x_i$ be the first such vertex on the path from $F$ to $X$. 
% %But as $\frac{\vv{x_{i-1}x_i}}{|x_{i-1}i_k|} + \frac{\vv{x_{i+1}x_i}}{|x_{i+1}x_i|}$ is almost (up to $2\gamma=o_\varepsilon(1)$) perpendicular to $(ax)$)
% %the point $x_{i-1}$ can not be a branching point (otherwise $((x_{i}x_{i-1}),(ax))\geq \pi/6-o_\varepsilon(1)$) and can only be a point of order $2$ such that  $\pi/9<\angle ((x_{i-2}x_{i-1}),(ax))<\pi/8$. Let there exists such $j$ that $\pi/9<\angle ((x_{j}x_{j+1}),(ax))<\pi/8$. Thus, for sufficiently small $\varepsilon>0$, points $x_j$ and $x_{j+1}$ can not be branching points and can be only points of order $2$. Thus, for sufficiently small $\varepsilon>0$ the inequalities  $\pi/10<\angle ((x_{j}x_{j-1}),(ax)),\angle ((x_{j+1}x_{j+2}),(ax))<\pi/7$ hold. But then set
% %\[
% %\Sigma \setminus (\Sigma_{[x_{j-1}x_j]} \cup \Sigma_{[x_jx_{j+1}]}) \cup [x_{j-1}x_{j+1}]\cup S^*(x_{j-1},\varepsilon(x_{j-1}))\cup S^*(x_{j+1},\varepsilon(x_{j+1}))
% %\]
% %is better than $\Sigma$, so we get a contradiction. Therefore for every $x_i$ the inequality $((x_{i}x_{i+1}),(ax))\geq \pi/9$.
% %I.e. all one-sided tangents of $P$ at $X$ have the angle with $(ax)$ greater than $\pi/9$. As $X$ was arbitrary, it is true for any point of $P$. Similarly, the same is true for the path in $\Sigma'$ from $\partial B_\varepsilon(x)$ to $F$. Thus, on the one hand,
% %\[
% %\H(P)\geq \frac{1}{\cos(\pi/9)}Pr_{(ax)}(P)=\frac{1}{\cos(\pi/9)}\varepsilon \cos (o_\varepsilon(1))=\frac{1}{\cos(\pi/9)}\varepsilon\pm o(\varepsilon).
% %\]
% %where $Pr_{(ax]}(P)$ is the projection of $P$ to $(ax)$.
% %On the other hand, due to item~\ref{four} of Corollary~\ref{ordord}, and due to Corollary~\ref{len0}, $\H(\Sigma' \cap %B_\varepsilon(x))=\varepsilon+o(\varepsilon)$. 
% %We have a contradiction, so the assumption that the number of the branching points is infinite must be false. THE END
% %} 
% due to Lemma~\ref{choice} and item~\ref{kapr2} of Corollary~\ref{kaprrr} at branching points, and due to Lemma~\ref{napr} at points of order $2$.
% Thus the difference of unit vectors collinear to the one-sided tangents of $P'$ at $F$ and $X$ is $o_\varepsilon(1)$ perpendicular to $(ax)$, i.e. all one-sided tangents of $P$ at $X$ have the angle with $(ax)$ almost (up to $o_\varepsilon(1)$) equal to $\pi/6$. As $X$ was arbitrary, it is true for any point of $P$. Similarly, the same is true for the path in $\Sigma'$ from $\partial B_\varepsilon(x)$ to $F$. Thus, on the one hand,
% \[
% \H(P)\geq \frac{2}{\sqrt{3}}Pr_{(ax)}(P)=\frac{2}{\sqrt{3}}\varepsilon \cos (o_\varepsilon(1))=\frac{2}{\sqrt{3}}\varepsilon\pm o(\varepsilon).
% \]
% where $Pr_{(ax]}(P)$ is the projection of $P$ to $(ax)$.

% On the other hand, due to item~\ref{four} of Corollary~\ref{ordord}, and due to Corollary~\ref{len0}, $\H(\Sigma' \cap B_\varepsilon(x))=\varepsilon+o(\varepsilon)$. %(as $\H(\Sigma \cap B_\rho(x))=\oordball_x\Sigma +o(\rho)$).
% We have a contradiction, so the assumption that the number of the branching points is infinite must be false.
% \end{proof}

%\textcolor{red}{
\begin{proposition}
One-sided tangents of minimizer $\Sigma$ are continuous. 
\label{cont}
\end{proposition}
\begin{proof}
 Assume the contrary. Then there exists $x\in \Sigma$, connected component $\Sigma_1$ of $\Sigma \setminus x$,  a one-sided tangent $(ax]$ to $\Sigma_1$ at $x$, and a sequence of points $z_k\in \Sigma_1$ converging to $x$ such that one-sided tangents $(a_kz_k)$ doesn't converge to $(ax)$ (convergence of lines implies convergence of one-sided tangents due to Lemma~\ref{ordord} item~\ref{four}). Without loss of generality let there exists such $\pi/2>c>0$ that for every $z_k$ angle $\angle((ax),(a_kz_k))>c$, and let also sufficiently small $\varepsilon>0$ be such that $\sharp \partial B_\varepsilon(x) \cap \Sigma_1=1$ and $\{z_k\}_{k=1}^\infty \subset B_\varepsilon(x)$. Consider a path $P$ in $\Sigma_1$ from $z_1$ to $x$. Let $\gamma=o_\varepsilon(1)$. Let for every $x$ radius $\varepsilon(x_i)<\dist(\partial B_{\varepsilon}(x),P)$ be define as in Lemma~\ref{tree} and let $\{x_k\}_{k=1}^N\subset P$ and $\varepsilon(x_k)=\varepsilon(x_k,\gamma)$ be a finite collection such that $P\subset \cup_{k=1}^N B_{\varepsilon(x_k)}(x_k)$, $x_1=z_1$ and $x_N=x$. Note that for every $k$ the sum 
\[
\frac{\vv{x_{k-1}x_k}}{|x_{k-1}x_k|} + \frac{\vv{x_{k+1}x_k}}{|x_{k+1}x_k|} 
\]
is perpendicular to $(ax)$ up to $2\gamma$
thus
\[
\frac{\vv{x_{1}x_2}}{|x_{1}x_2|} - \frac{\vv{x_{N-1}x}}{|x_{N-1}x|} 
\]
is perpendicular to $(ax)$ up to $2\gamma$.
Therefore 
\[
\angle ((a_1x],(ax])\leq 4\gamma=o_\varepsilon(1),
\]
so we get a contradiction. 
\end{proof}
 \begin{corollary}
 The number of branching points is finite.
 \label{main}
 \end{corollary}
\begin{proof}
 Assume the contrary. Then there exists $x\in \E_\Sigma$, connected component $\Sigma_1$ of $\Sigma \setminus x$, one-sided tangent $(ax]$ to $\Sigma_1$ and an infinite sequence of branching points $\{x_i\}_{i=1}^{\infty}\subset \Sigma_1$ converging to $x$. But then, due to Lemma~\ref{choice} and Proposition~\ref{cont}, one-sided tangent $(ax]$ should be perpendicular to itself, so we get a contradiction.
\end{proof}
\subsection{vdrug prigoditsia}

\begin{lemma}
Let $x \in E_\Sigma$ and let there exist such a  cusp $Q\in \mathbb{Q}^{a,x}_\varepsilon$ that $Q^{a,x}_\varepsilon \cap \Sigma$ is an arc. Then for each $c>0$ there exists such $\varepsilon=\varepsilon(c)>0$ that every one-sided tangent at the points of set $Q^{a,x}_\varepsilon \cap B_{\varepsilon(c)}(x) \cap \Sigma$ has an angle not greater than $2c$ with a line $(ax)$.
\label{zapred}
\end{lemma}

\begin{proof}
Assume the contrary, id est there exists a sequence of points with one-sided tangents having an angle with $(ax)$ greater than $2c$, converging to $x$. Without loss of generality assume $c<\pi/2$. By item~\ref{__3} of Lemma~\ref{alm} for sufficiently small $\varepsilon$ this sequence consists only on the points of $X_\Sigma \sqcup S_\Sigma$. As there is no branching points, the direction of tangents doesn't change at points of $S_\Sigma$, that is there is a sequence of points from $ X_\Sigma $ converging to $ x $ such that at least one of the two segments incident to the point has an angle with $ (ax) $ greater than $ 2c $. Let $L_1$ be such a point and let $\varepsilon$ be chosen not greater than $\rho$ for $c/5$ in Lemma~\ref{alm}. By item~\ref{__2} of Lemma~\ref{alm} both segments incident to $L_1$ has an angle with $(ax)$ greater than $9/5c$. Then the segment lying on the path from $L_1$ to $x$ should end with point $L_2\in X_\Sigma $. But the segment leaving $ L_2 $ must have an angle with $ (ax) $ greater than $ 8/5c $ and end with point $ L_3 \in X_\Sigma $. Thus for any arbitrarily small $ \bar \varepsilon$ there exists a broken line $ L_1-L_2-L_3-L_4-L_5 \subset \Sigma \cap B_{\bar \varepsilon} (x) $ such that all angles $ \angle ((L_jL_{j + 1}), (ax))> c $ for $j = 1,2,3,4 $. This is a contradiction with Proposition~\ref{brrrr}.
\end{proof}
\begin{lemma}
For every $x\in E_\Sigma$ and  $c>0$ there exists such $\rho>0$, that for every $\bar x \in G_\Sigma \cap B_\rho(x)  \setminus \{x\}$ and for the $(ix]$, closest to $\bar x$ energetic ray of $x$, the following statements are true: 
\begin{enumerate}
\item if $\oord_{\bar x}\Sigma=1$, then $\bar x \in X_\Sigma$ and for the segment $[s\bar{x}] \subset \Sigma$ the following inequality is true:  \[\angle((s\bar{x})(ix))>\pi/2-c.\] 
In other words the segment $[s\bar x]$ is $o_\rho(1)-$almost perpendicular to $(ix)$.
If $(ix]$ is one-oriented energetic ray, then for point $y\defeq y(x)$, which is the limit of the points corresponding to the energetic points of the energetic ray $(ix]$ the following inequality is true:
 \[
 \angle ([s\bar{x}), [xy))<c;
 \]
\label{__1}
\item if $\bar x \in X_\Sigma$ and  $\oord_{\bar x} \Sigma=2$, then the angle of incidence is almost equal to the angle of reflection:
\[|\angle((s\bar{x}], (ix))-\angle( (ix),(t\bar{x}])|<c\mbox{, where } [s\bar{x}] \cup [t\bar{x}] \subset \Sigma;\]
\label{__2}
\item if $\bar {x} \in E_\Sigma$, then there exists such $\varepsilon>0$ that $B_\varepsilon(\bar x) \cap \Sigma$ is contained in the union of two cusps (and each cusp is not empty) with axes, almost parallel to $(ix)$, id est $|\angle((m\bar{x}],(ix))|<c$ and $|\angle((n\bar{x}],(ix))|<c$, where $\Sigma \cap B_\varepsilon(\bar x) \subset Q_\varepsilon^{m,\bar x}\cup Q^{n, \bar{x}}_\varepsilon$, for $ Q_\varepsilon^{m,\bar x} \in  \mathbb{Q}_\varepsilon^{m,\bar x}$, $ Q_\varepsilon^{n,\bar x} \in \mathbb{Q}_\varepsilon^{n,\bar x}$. 
\label{__3}
\end{enumerate}
\label{alm}
\end{lemma}
\begin{proof}
%окажем пункт~\ref{__1}. The points from set$S_\Sigma$ can not be of order $1$, otherwise their small neighbourhood can be deleted. 
%НАДО ВЫВЕСТИ ИЗ ПРЕДЫДУЩЕЙ
\begin{enumerate}
  

\item Lets prove that  
%для произвольного $x \in E_\Sigma$ найдется такое $\rho>0$, что для каждого $\bar x \in B_\rho(\Sigma)\setminus \{ %x\}$, 
 $\oord_{\bar x}\Sigma = 1$ implies $\bar x\in X_\Sigma$. 
\label{QQ}
Assume the contrary: let $\bar x \in E_\Sigma \cap B_\rho(x) \setminus x$. 
% Энергетическое ребро или ребра, к которым они сходятся, должны лежать на прямой, почти параллельной $(ix]$ ввиду %Следствия~\ref{alm_parr}.  
%\end{itemize}

In view of Lemma~\ref{ordball_} it is suffices to analyze the following cases:
\begin{itemize}
\item [(a)] Case $\oordball_{\bar x}\Sigma=2$.
Let $\{\varepsilon_l\}$ be a decreasing to $0$ sequence of such numbers that $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=2$ and $\varepsilon_1 < \min (\rho, \rho-|\bar x x|)$. Denote  $s^l, t^l \defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. 
We know from the item~\ref{WW} of Proposition~\ref{items} inequalities $\angle ((s^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ and $\angle ((t^l\bar x), (ix)) \leq \pi/3 +o_\rho(1)$ hold.%, то есть
%\begin{equation}
%s^l, t^l \in \Lambda((ix), \pi/3+o_\rho(1)).
%\label{LLL}
%\end{equation}
Then, due to the unit order of $\bar x$ there exists a converging to $\bar x$ sequence of such points $\{u_m\}\subset \Sigma$ that \[\angle\left((u_l\bar x),(ix)\right)=\frac{\pi}{2}.\] So we have a contradiction to the item~\ref{WWW} of Proposition~\ref{items}.


\item [(b)] Case $\oordball_{\bar x}\Sigma=1$. 

Let $\varepsilon_l>0$ be a decreasing to $0$ sequence of such numbers that $\sharp (\partial B_{\varepsilon_l}(\bar x) \cap \Sigma )=1$ and $s_l\defeq \partial B_{\varepsilon_l}(\bar x) \cap \Sigma$. Then in view of item~\ref{W} of Proposition~\ref{items} each line $(s_l\bar x)$ is almost perpendicular to $(ix)$:
\begin{equation}
\left|\angle \left((s_l\bar x), (ix)\right)-\frac{\pi}{2}\right| =o_\rho(1).
\label{99}
\end{equation}
Note that for every $\varepsilon_l$ holds
\begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)=\varepsilon_l+o_\rho(1)\varepsilon.
\label{100}
\end{equation}
Inequality $\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)\geq \varepsilon_l$ is true because of connectivity $\Sigma$ and inequality in the other side is true in view of Lemma~\ref{Losiu}: otherwise one could replace $\Sigma$ by $\Sigma \setminus B_{\varepsilon_l}(\bar x) \cup [\bar{x}s_l]\cup S$, where $S$ is defined at Lemma~\ref{Losiu} for $w=\bar x$, and get a contradiction with optimality of $\Sigma$. 

So, for sufficiently small $\rho$  \begin{equation}
\H(B_{\varepsilon_l}(\bar x)\cap \Sigma)<\varepsilon_l \left(1+\frac{1}{18}\right).
\label{101}
\end{equation}
Then we can say (add elements to $\{\varepsilon_l\}$ if it is necessarily) that
\begin{equation}
\frac{\varepsilon_l}{\varepsilon_{l+1}}\leq \frac{18}{17}.
\label{103}
\end{equation}
Otherwise there exists such $\varepsilon_l$ that $\sharp ( \partial B_{\bar{\varepsilon}}(\bar x)\cap \Sigma)\geq 2$ for every $\bar{\varepsilon} \in [\frac{17\varepsilon_l}{18},\varepsilon[$. Thus, by co-area inequality, 
\[
\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x)\right)\geq \H \left(\Sigma \cap B_{\frac{17\varepsilon_l}{18}}(\bar x)\right) +\H \left(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus  B_{\frac{17\varepsilon_l}{18}}(\bar x)\right)\geq \varepsilon_l \left (1+\frac{1}{18} \right),
\]
which contradicts to~\eqref{101}.
Note, as $\bar x$ has an energetic ray which is, in view of Corollary~\ref{alm_parr} $o_\rho(1)$-almost parallel to $(ix)$, there exists a sequence of energetic points $\{x_l\}$, converging to $\bar x$ such that $\angle ((x_l\bar x], (ix]) =o_\rho(1)+o_{|x_l\bar x|}(1)$.  The sequences $\{x_l\}$ and $\{ s_l \}$ with unit order $\oord_{\bar x}(\Sigma)=1$ imply the presence of also converging to $\bar x$ sequence of points $\{ u_l\}\subset \Sigma$ such that $\angle \left((u_l\bar x),(ix)\right) = \frac{\pi}{4}$. Consider an arbitrary element $u_m$ of this sequence. In view of inequality~\eqref{103} there exists such number $l$ that
\begin{equation}
0<\varepsilon_l-|\bar xu_m|\leq \frac{1}{18}\varepsilon_l.
\label{104}
\end{equation}
Note also, that by~\eqref{99} inequality
\[
\sharp (\partial B_{|\bar x u_m|}(\bar x)\cap \Sigma) \geq 2
\] 
holds.


%Можно также считать, что для произвольного $\delta \in [|\bar x u_m|,\varepsilon_l[$ выполняется $\sharp (\partial B_{\delta}(\bar x)\cap \Sigma) \geq 2$.

Let 
\[
k:=\max_{s \in \Sigma \cap \overline{B_{\varepsilon_l}}: \sharp (\Sigma \cap _{|s \bar x|}(\bar x))=1} \angle((ix),(\bar xs)),
\]
then $|k-\pi/2|=o_\rho(1)$.
Define also $K := \Lambda((p \bar x),k-\pi/2)$, where $(p\bar x) \perp (ix)$. $K$ contains an area of possible location of points $s_l$. 


%Кроме того, пусть $K \subset \Lambda((\bar x y(\bar x)), o_\rho(1))$ --- область возможного расположения точек $s_l$ (угол с вершиной в $\bar x$, раствором $o_\rho(1)$ и перпендикуляром к $(ix)$ в качестве биссектрисы), а 
Let $Q$ be a cusp or a union of two cusps with vertex at $\bar x$, containing all energetic points of  $B_{\varepsilon_l}(\bar x)$, then
\begin{equation}
d \defeq \dist(u_m, Q \cup K)\geq \frac{\sqrt{2}}{2}|\bar xu_m|-o_\rho(1)\varepsilon_l \geq (\frac{17}{18\sqrt 2}+o_\rho(1))\varepsilon_l,
%\label{105}
\end{equation}
where the last inequality follows from~\eqref{104}. 
%Ясно, что, ввиду единичного порядка $\bar x$ и определения компоненты связности $q$, выполняется $\H(q) \geq 2d$. В таком случае, ввиду неравенства коплощади для $\Sigma \setminus q$, верно
Then the length of the connected component of $\Sigma \setminus (Q \cup K)$, containing $u_m$, is greater or equal to $d$.
In view of co-area inequality, item~\ref{W} of Proposition~\ref{items} and inequality ~\eqref{101} inequality $\H(\Sigma \cap K \cap B_\varepsilon(\bar x)) \geq \frac{17}{18}\varepsilon$ holds.
On the other hand \[
\H(\Sigma \cap B_{\varepsilon_l}(\bar x)) \geq H(\Sigma \cap B_{\varepsilon_l}(\bar x)\cap K)+\H(\Sigma \cap B_{\varepsilon_l}(\bar x) \setminus (K \cup Q)) \geq \frac{17}{18}\varepsilon_l +d\geq
\varepsilon_l (\frac{17}{18}+\frac{17}{18\sqrt 2}-o_\rho(1))>\frac{19}{18}\varepsilon_l.
\]
So we get a contradiction to inequality~\eqref{101}.
\end{itemize}
\item% Let $\oord_{\bar x} \Sigma =2$ and $\bar x \in X_\Sigma$, и для некоторого $\varepsilon>0$ выполняется $\Sigma \cap \overline{B_{\varepsilon}(\bar x)}=[s\bar x] \sqcup [t\bar x]$. 
%\label{Q3}
The statement immediately follows from item~\ref{WWWW} of Proposition~\ref{items}.

\item% Докажем пункт~\ref{__3} Леммы.
%\begin{proof}
Because of items~\ref{BB} and~\ref{reb} Lemma~\ref{con} there exists $Q$ --- a cusp or a union of two cusps with vertex at $\bar x$ such that $G_\Sigma \cap B_{\varepsilon_0}(\bar x) \subset Q$ for sufficiently small $\varepsilon_0>0$. In view of Corollary~\ref{alm_parr} axes of these cusps are almost parallel to $(ix)$. If at least one energetic ray of $\bar x$ is two-orientated, the statement of the item is trivial because of Remark~\ref{star}. Similarly, the item is trivial if the rays are orientated to the different sides, id est for sufficiently small $\varepsilon_0>0$ points of $M$, corresponding to the energetic points from set $B_{\varepsilon_0}(\bar x) \setminus \bar{x}$ are locates at both parts of the plane divided by energetic rays of $\bar x$. %Thus we can assume that every energetic rays are one-sided
Let $(q_l\bar x]$ be a ray, not coinciding with any of cusps' axes. Then, because of the definition of cusps, there exists such $\varepsilon_1>0$, that $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\{\bar x\}$. We can also assume $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$, as  $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$ because of the item~\ref{QQ} of the proven Lemma, Remark~\ref{rem_ord} and Lemma~\ref{ordball_}. We will show that there exists such $\varepsilon_2>0$, that 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
\]
or 
\[
B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
\]

%Пусть $(q_1\bar x]$ --- луч, лежащий во внутреннем угле и не совпадающий ни с одним энергетическим ребром $\bar x$. Тогда, ввиду определения псевдоконуса найдется такое $\varepsilon_1>0$, что $(q_1\bar x] \cap Q \cap B_{\varepsilon_1}(\bar x)=\emptyset$. Поскольку ввиду пункта~\ref{QQ} доказываемой леммы, замечания~\ref{rem_ord} и леммы~\ref{ordball_}, выполняется $\oord_{\bar x} \Sigma =\oordball_{\bar x}\Sigma=2$, потребуем, чтобы $\varepsilon_1>0$ удовлетворяло условию $\sharp (\Sigma \cap \partial B_{\varepsilon_1}(\bar x))=2$. Покажем, что тогда найдется такое $\varepsilon_2>0$, что 
%\[
%B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x], 
%\]
%либо 
%найдется такое $\varepsilon_2>0$, что 
%\[
%B_{\bar \varepsilon_2}(\bar x) \cap (q\bar x] \cap \Sigma = \bar x. 
%\]
 Assume neither of the two cases come true. Then set $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ contains infinitely many points close to $\bar x$. Herewith each point of set $\Sigma \cap B_{\varepsilon_1}(\bar x) \cap (q\bar x]$ is not energetic and should be a center of a segment or a regular tripod.  
%, а множество $\Sigma \cap B_{\varepsilon}(\bar x) \setminus Q$ является штейнеровским лесом. 
By item~\ref{WWW} Proposition~\ref{items} ray $(qx]$ can not be perpendicular to $(ix]$. Let $L_1$ be an open area bounded by perpendicular to $(ix]$, passing through point $\bar x$, $(q_1\bar x]$ and $\partial B_{\varepsilon_1}(\bar x)$, not containing any energetic points. Then $S := \overline{L_1\cap \Sigma}$ is a Steiner forest, with all infinitely many terminal points, except at most three from set $\partial B_{\varepsilon_1} (\bar x) \cup \{ \bar x \}$, located at the perpendicular or at $(q\bar x]$. By Lemma~\ref{St_l} the perpendicular contains infinite number of terminal points of $ S$, thus there exists an infinite sequence of points $\{u_l\}$ such that $\angle((u_l,\bar x)(ix))=\pi/2$ for each $l$ which contradicts to item~\ref{WWW} of Proposition~\ref{items}. Ergo there exists such $\varepsilon_1>0$, that $\Sigma \cap (q_1\bar x] \cap \overline {B_{\varepsilon_1}(\bar x)}$ coincides with $\{\bar x\}$ or $(q_1\bar x] \cap B_{\varepsilon_1}(\bar x) $. We pick such $\varepsilon_1$ that also $\sharp(\partial B_{\varepsilon_1}(\bar x)\cap \Sigma)=2$ and $Q \cap B_{\varepsilon_1}(\bar x) \cap (q_1\bar x] = \emptyset$.

Let $(m\bar x]$ be an energetic ray of $\bar x$. Pick such decreasing to zero sequences $\{\bar{\varepsilon}_i \}$ and $\{ \gamma_i\}$, that 
\begin{itemize}
\item $Q \cap B_{\bar \varepsilon_i}(\bar x)$ is contained in the angle with bisector $(m\bar x]$ and size $2\gamma_i$;
\item the intersection of the borders of this angle (with bisector $(m\bar x]$ and size $2\gamma_i$) with set $\Sigma \cap \cap B_{\bar\varepsilon_{i+1}}(\bar x)$ coincides with point $\{ \bar x \}$ or with a boundary of a sector of $B_{\bar \varepsilon_{i+1}}(\bar x)$. 
\end{itemize}
Let $\gamma_1 \leq \pi/12$, $\bar \varepsilon_1 \defeq \varepsilon_1$.
If at some number (at most at one by Lemma~\ref{angles2}) the intersection is the segment, let $j$ be equal to this number. Otherwise let $j=0$.

Define the following cusp: \[
Q_1 \defeq Q^{m,\bar x}_{\overline{\varepsilon}_{j+1}}\defeq \bigcup_{i=j+1}^{\infty} \left(Q(m,\overline x, \gamma_i, \overline{\varepsilon_i}) \setminus B_{\overline{\varepsilon}_{i+1}}(\bar x)\right).
\]
If $\bar x$ has two energetic rays, similarly define the second cusp $Q_2$ with second energetic ray as the axis.

%$(a \bar x$ и $(b \bar x]$, то аналогично определим псевдоконус $Q^{b, \bar x}_{\bar \varepsilon_1}$
Thus an arbitrary connected component of $\Sigma \cap B_{\bar{\overline{\varepsilon_1}}}(\bar x)\setminus \{\bar x\}$ located inside the cusp $Q_1$ and $Q_2$ if it exists, or located outside of it. As $\bar x$ has an energetic ray, at least on of the components should lay inside, then it has a tangent line at point $\bar x$, which coincides to energetic ray and so $o_\rho(1)-$almost parallel to $(ix]$. Then by Lemma~\ref{angles2} another component can not lay in the same cusp. 
If there is only one cusp there could be one ray $(q \bar x]$, which doesn't intersect the cusp and $\varepsilon_1>0$ such that a connected component in $B_{\varepsilon_1}(\bar x)$ coincides with the segment $(qx]\cap B_{\varepsilon_1}(\bar x)$. 
Then we can choose an arbitrary cusp with $(qx]$ as an axis. Otherwise similarly construct the second cusp for the second energetic ray with decreasing sequence of radii $\{\varepsilon_k\}$.
Note that as $\bar x$ (due to item~1 of this lemma) can not have a unit order due to the item~3 from the proof of the Lemma~\ref{angles2}) set $\Sigma \cap B_{\bar \varepsilon}(\bar x)$ can not be located in the one cusp for any $\bar \varepsilon>0$. So by Lemma~\ref{angles2} there is certainly two cusps. Applying an item~\ref{WWWW} Proposition~\ref{items} we get that there is an infinite strictly decreasing to $0$ sequence $\varepsilon_k$ such that for $S_k,T_k\defeq \partial B_{\varepsilon_k}(\bar x)$ inequality $|(\angle S \bar x], (ix] - \angle (T \bar x], (ix]| = o_\rho(1)$ holds, so the axes of both cusps should be $o_\rho(1)$-almost parallel to $(ix]$, which is required for $\varepsilon$ equal to minimum of $\varepsilon_1$ and $\overline{\varepsilon_1}$.  
\end{enumerate}
 
% \begin{remark}
 %Заметим также, то угол между ребрами, содержащий соответствующую $x^i_k$ точку $y^i$, не может быть меньше $\pi$ (если покрытые $x^i_k$ точки есть в обеих полуплоскостях, то угол между ребрами составляет ровно $\pi$).
 %\label{rovno}
 
 %\end{remark}
 \end{proof}
%\subsection{unknown}
%НАДО ПРОВЕРИТЬ ЕСТЬ ЛИ У НАС с11 ЧТО МЫ ВООБЩЕ ДОКАЗАЛИ (ВОЗМОЖНО НЕ ПРОСТО НЕПРЕРЫВНОСТЬ ОДН КАСАТЕЛЬНОЙ, А ЕЩЕ И ЛИПШИЦЕВОСТЬ ГРАДИЕНТА)

%Лемма про долю точек с большой касательной
%(обобщение леммы про уменьшение наклона)

%Лемма про W -- для пространства 
%(

%Существует ли пример triple point не являющейся точкой 
